Conformally invariant fields out of Brownian loop soups

Consider a Brownian loop soup $\mathcal{L}_D^\theta$ with subcritical intensity $\theta \in (0,1/2]$ in some 2D bounded simply connected domain. We define and study the properties of a conformally invariant field $h_\theta$ naturally associated to $\mathcal{L}_D^\theta$. Informally, this field is a signed version of the local time of $\mathcal{L}_D^\theta$ to the power $1-\theta$. When $\theta=1/2$, $h_\theta$ is a Gaussian free field (GFF) in $D$. Our construction of $h_\theta$ relies on the multiplicative chaos $\mathcal{M}_\gamma$ associated with $\mathcal{L}_D^\theta$, as introduced in [ABJL23]. Assigning independent symmetric signs to each cluster, we restrict $\mathcal{M}_\gamma$ to positive clusters. We prove that, when $\theta=1/2$, the resulting measure $\mathcal{M}_\gamma^+$ corresponds to the exponential of $\gamma$ times a GFF. At this intensity, the GFF can be recovered by differentiating at $\gamma=0$ the measure $\mathcal{M}_\gamma^+$. When $\theta<1/2$, we show that $\mathcal{M}_\gamma^+$ has a nondegenerate fractional derivative at $\gamma=0$ defining a random generalised function $h_\theta$. We establish a result which is analoguous to the recent work [ALS23] in the GFF case ($\theta=1/2$), but for $h_\theta$ with $\theta \in (0,1/2]$. Relying on the companion article [JLQ23], we prove that each cluster of $\mathcal{L}_D^\theta$ possesses a nondegenerate Minkowski content in some non-explicit gauge function $r \mapsto r^2 |\log r|^{1-\theta+o(1)}$. We then prove that $h_\theta$ agrees a.s. with the sum of the Minkowski content of each cluster multiplied by its sign. We further extend the couplings between CLE$_4$, SLE$_4$ and the GFF to $h_\theta$ for $\theta\in(0,1/2]$. We show that the (non-nested) CLE$_\kappa$ loops form level lines for $h_\theta$ and that there exists a constant height gap between the values of the field on either side of the CLE loops.

==> subfiles/1D.tex <==
In this section, we study the analogue of the field $h_\theta$ in the one-dimensional case.
This is partly motivated by the recent connection between the 1D and 2D loop soup discovered in \cite{JLQ23a}.
As we will recall in Theorem \ref{T:1Disomorphism} below, the local time of the 1D loop soup is distributed as a (reflected) squared Bessel process of dimension $d=2\theta$.
When $\theta=1/2$, obtaining a Brownian motion (1D analogue of the GFF) from the loop soup then boils down to taking the square root of a (reflected) 1D squared Bessel process and then flipping each excursion independently of each other with equal probability.
What is the analogue of this procedure when $\theta \neq 1/2$? 
We will see that, surprisingly, taking the square root is not the right thing to do (although this might be very natural since the square root of a squared Bessel process is just a Bessel process) and that one has to take the power $1-\theta = 1-d/2$ instead. This power is exactly the one appearing in the Radon--Nikodym derivative of the Bessel process and its dual Bessel process of dimension $d^* = 4 -d = 2\theta^*$ where $\theta^* = 2-\theta$; see \eqref{E:Bessel_duality}. The purpose of this section is also to hint at the duality between the intensities $\theta$ and $2-\theta$ that might still hold in some sense in dimension two. See Section \ref{S:expansion_signed} for more details concerning the 2D case.

\subsubsection{Loop soup on $\R^+$}

Let us start by defining the loop soup on the half line $\R^+$. We follow \cite{Lupu18}.
For $x,y \in \R^+$, let $p(t,x,y)$ and $p_{\R^+}(t,x,y)$ be the heat kernels on $\R$ and $\R^+$:
\[
p(t,x,y) = \frac{1}{\sqrt{2\pi t}} e^{-(y-x)^2/(2t)}, \quad p_{\R^+}(t,x,y) = p(t,x,y) - p(t,x,-y)
\]
and let $\P_{\R^+}^{t,x,y}$ be the law of a Brownian bridge from $x$ to $y$ of duration $t$ in the half line $\R^+$. 
The Green function and the loop measure are respectively given by
\[
G_{\R^+}(x,y) = \int_0^\infty p_{\R^+}(t,x,y) \d t = 2 x \wedge y
\quad \text{and} \quad
\loopmeasure_{\R^+} = \int_0^\infty \frac{p_{\R^+}(t,x,x)}{t} \P_{\R^+}^{t,x,x} \d t.
\]
For $\theta >0$, the loop soup $\Lc_{\R^+}^\theta$ in $\R^+$ with parameter $\theta$ is distributed according to a Poisson Point Process with intensity $\theta \loopmeasure_{\R^+}$. Compared to the 2D case, the local time of $\Lc_{\R^+}^\theta$ is well defined pointwise and finite and we will denote it
\[
L_x(\Lc_{\R^+}^\theta) = \sum_{\wp \in \Lc_{\R^+}^\theta} L_x(\wp) = \sum_{\wp \in \Lc_{\R^+}^\theta} \int_0^{T(\wp)} \indic{\wp_t = x} \d t, \quad \quad x \in \R^+.
\]

\begin{theorem}[\cite{Lupu18}]\label{T:1Disomorphism}
Let $\theta>0$.
$(L_x(\Lc_{\R^+}^\theta))_{x \geq 0}$ has the law of a squared Bessel process of dimension $d=2\theta$, reflected at 0 when $\theta <1$.
\end{theorem}

Let $\Ps^d$ be the law under which $(R_x,x \geq 0)$ is a squared Bessel process of dimension $d=2\theta$, reflected at 0 when $\theta <1$.
The clusters of $\Lc_{\R^+}^\theta$ correspond to the excursions away from 0 of $R$. Therefore Theorem \ref{T:1Disomorphism} implies that when $\theta <1$ there are infinitely many clusters and when $\theta \geq 1$ there is only one cluster. Notice that the critical point is different from the two-dimensional case. However, we show in \cite[Theorem 1.9]{JLQ23a} that there is a phase transition at $\theta = 1$ in the percolative behaviour of large loops on the half-infinite cylinder $(0,\infty) \times \mathbb{S}^1$ (by conformal invariance, this translates to a phase transition in the percolative behaviour of large loops targeting a given point of some bounded 2D domain). See \cite[Section 1.3]{JLQ23a} for more details.


\subsubsection{Characterisation of Laguerre polynomials in terms of Bessel processes}

As already seen, the generalised Laguerre polynomials $\mathbf{L}_n^{(\theta-1)}$ have been used by Le Jan to renormalise the powers of the local time of the loop soup in dimension two. In this section, we show that these polynomials are also special in dimension one in the sense that they are the only polynomials leading to martingales. See Lemma \ref{L:1D_martingale} for a precise statement. 

For any $\theta>0$, the Wick powers of the local time $L_x(\Lc_{\R^+}^\theta)$ are defined by
\begin{equation}
\label{E:1D_power}
:L_x(\Lc_{\R^+}^\theta)^n:
\quad = \quad (2x)^n \mathbf{L}_n^{(\theta-1)} \Big( \frac{L_x(\Lc_{\R^+}^\theta)}{2x} \Big), \quad \quad x \geq 0, n \geq 1.
\end{equation}
In the special case $\theta = 1/2$ this corresponds to the even Wick powers of 1D Brownian motion.


\begin{lemma}\label{L:1D_martingale}
Let $\theta >0$ and $n \geq 1$. The process $ (:L_x(\Lc_{\R^+}^\theta)^n:)_{x \geq 0}$ is a martingale.
Moreover, $\mathbf{L}_n^{(\theta-1)}$ is the only monic polynomial such that \eqref{E:1D_power} is a martingale.
\end{lemma}

Let us stress that it is a well known fact that the Wick powers of 1D Brownian motion lead to martingales. However, it seems to be new when $\theta \neq 1/2$.

\begin{proof}
Because in this lemma the space $\R^+$ is thought of as time, we will change the notations $x$ and $y$ for the space variables by $s$ and $t$. We will denote by $(\Fc_t)_{t \geq 0}$ the natural filtration of the Bessel process.
Let $X_t = \sqrt{R_t}$ be a Bessel process of dimension $d=2\theta$. Recall that $X_t$ satisfies the stochastic differential equation
$
\d X_t = \frac{d-1}{2 X_t} \d t + \d B_t
$
where $(B_t)_{t \geq 0}$ is a 1D standard Brownian motion. A computation using It\^{o} formula leads to the following SDE for $: L_t(\Lc_{\R^+}^\theta)^n :$ (we write $\mathbf{L}_n$ instead of $\mathbf{L}_n^{(\theta-1)}$)
\begin{align*}
\d \left\{ (2t)^n \mathbf{L}_n^{(\theta-1)} \Big( \frac{X_t^2}{2t} \Big) \right\}
& = 2^nt^{n-1} X_t \mathbf{L}_n' \Big( \frac{X_t^2}{2t} \Big) \d B_t \\
& + 2^nt^{n-1} \left\{ n \mathbf{L}_n \Big( \frac{X_t^2}{2t} \Big) + \Big( \theta - \frac{X_t^2}{2t} \Big) \mathbf{L}_n' \Big( \frac{X_t^2}{2t} \Big) + \frac{X_t^2}{2t} \mathbf{L}_n'' \Big( \frac{X_t^2}{2t} \Big) \right\} \d t.
\end{align*}
Because $\mathbf{L}_n = \mathbf{L}_n^{(\theta-1)}$ satisfies $n \mathbf{L}_n(u) + (\theta - u) \mathbf{L}_n'(u) + u \mathbf{L}_n''(u) = 0$ (see e.g. (22.1.3) and (22.8.6) in \cite{special}), we see that the finite variation part vanishes. In other words, $(: L_t(\Lc_{\R^+}^\theta)^n :)_{t \geq 0}$ is a local martingale. A routine argument concludes that it is a martingale as desired.

The fact that $\mathbf{L}_n = \mathbf{L}_n^{(\theta-1)}$ is the only monic polynomial such that \eqref{E:1D_power} is a martingale follows from the fact that it is the only monic polynomial satisfying $n \mathbf{L}_n(u) + (\theta - u) \mathbf{L}_n'(u) + u \mathbf{L}_n''(u) = 0$.
\end{proof}



\subsubsection{Analogue of $h_\theta$ on $\R^+$ and renormalisation of its powers}


Assume that $\theta < 1$ (subcritical regime for 1D loop soups).
In this section we define the natural analogue $h_{\theta, \R^+}$ of $h_\theta$ on $\R^+$ and give a procedure to renormalise its ``odd'' powers. Let $R$ be a $2\theta$-dimensional squared Bessel process. Let $\Ec$ be the set of excursions of $R$ and, conditionally on $\Ec$, let $\sigma_e, e \in \Ec$ be i.i.d. spins taking values in $\{ \pm 1\}$ with equal probability. Define
\[
h_{\theta, \R^+}(x) := \sigma_{e_x} R_x^{1-\theta}, \quad \quad x \geq 0,
\]
where $e_x$ is the excursion containing $x$.


The following result computes the two-point function of the field $h_{\theta,\R^+}$ and shows that tilting the probability measure by $h_{\theta,\R^+}(x) h_{\theta,\R^+}(y)$ amounts to changing the dimension of the Bessel process to its dual $d^* = 4-d$. Equivalently, this changes the intensity of the loop soup to $\theta^* = 2-\theta$.

\begin{lemma}\label{L:2point1D}
Let $\theta \in (0,1)$.
For all $0 \leq x \leq y$, and all bounded measurable function $F$,
\begin{equation}
\label{E:two-point1D}
\Es^d \left[ h_{\theta, \R^+}(x) h_{\theta, \R^+}(y) F( (R_z)_{z \in [x,y]}) \right] = \frac{\Gamma(\theta^*)}{\Gamma(\theta)} G_{\R^+}(x,y)^{2(1-\theta)} \Es^{d^*} \left[ F( (R_z)_{z \in [x,y]}) \right]
\end{equation}
where $d^* = 4-d = 2 \theta^*$ and $\theta^* = 2-\theta$.
\end{lemma}



\begin{proof}
By independence of the signs on different clusters and then by Markov property, we have
\begin{align*}
\Es^d \left[ h_{\theta, \R^+}(x) h_{\theta, \R^+}(y) F( (R_z)_{z \in [x,y]}) \right]
& = \Es^d \left[ R_x^{1-\theta} R_y^{1-\theta} \indic{\forall z \in [x,y], R_z>0} F( (R_z)_{z \in [x,y]}) \right] \\
& = \Es^d \left[ R_x^{1-\theta} \Es^d_{R_x} \left[ R_{y-x}^{1-\theta} \indic{ \forall z \in [0,y-x], R_z >0 } F( (R_z)_{z \in [0,y-x]}) \right] \right].
\end{align*}
As already mentioned, the key observation is that the power $1-\theta$ is exactly the power one needs to take in order to obtain the dual Bessel process of dimension $d^* = 4-d$. More precisely, for any $t>0$ and starting point $r>0$, restricted to the event that $\{ \forall s \in [0,t], R_s >0 \}$, we have
\begin{equation}
\label{E:Bessel_duality}
\frac{\d \P_r^{d^*}}{\d \P_r^{d}} {}_{\big\vert_{\Fc_t}} = \left( \frac{R_t}{r} \right)^{1-d/2}
\end{equation}
where $(\Fc_s)_{s \geq 0}$ is the natural filtration associated to $(R_s)_{s \geq 0}$.
See \cite[Proposition 2.2]{LawlerBessel}.
This implies that the left hand side of \eqref{E:two-point1D} is equal to
\begin{align*}
\Es^d \left[ R_x^{2(1-\theta)} \Es^{d^*}_{R_x} \left[ \indic{ \forall z \in [0,y-x], R_z >0 } F( (R_z)_{z \in [0,y-x]}) \right] \right] = \Es^d \left[ R_x^{2(1-\theta)} \Es_{R_x}^{d^*} \left[ F( (R_z)_{z \in [0,y-x]}) \right] \right]
\end{align*}
since the dual Bessel process does not reach zero a.s. ($d^* \geq 2$).
Under $\Ps^d$, $R_x$ is Gamma$(\theta,2x)$-distributed ($\theta$ and $2x$ are respectively the shape and scale parameters). A computation with Gamma distributions shows that for any measurable function $f: [0,\infty) \to \R$,
\[
\Es^d \left[ R_x^{2(1-\theta)} f(R_x) \right]
= \Es^d \left[ R_x^{2(1-\theta)} \right] \Es^{d^*} \left[ f(R_x) \right]
= (2x)^{2(1-\theta)} \frac{\Gamma(2-\theta)}{\Gamma(\theta)} \Es^{d^*} \left[ f(R_x) \right].
\]
Wrapping things up and by Markov property, we have obtained that the left hand side of \eqref{E:two-point1D} is equal to
\begin{align*}
(2x)^{2(1-\theta)} \frac{\Gamma(2-\theta)}{\Gamma(\theta)} \Es^{d^*} \left[ \Es_{R_x}^{d^*} \left[ F( (R_z)_{z \in [0,y-x]}) \right] \right] 
= (2x)^{2(1-\theta)} \frac{\Gamma(2-\theta)}{\Gamma(\theta)} \Es^{d^*} \left[ F( (R_z)_{z \in [x,y]}) \right].
\end{align*}
Lemma \ref{L:2point1D} then follows from the fact that $G_{\R^+}(x,y) = 2x$.
\end{proof}

When $\theta \in (0,1)$, Lemma \ref{L:2point1D} suggests to define the ``odd'' powers (i.e. powers that are not integer powers of the local time) of $h_{\theta,\R^+}$ by
\begin{equation}
:h_{\theta,\R^+}(x) L_x(\Lc_{\R^+}^\theta)^n:
\quad = \quad (2x)^n h_{\theta,\R^+}(x) \mathbf{L}_n^{(\theta^*-1)} \Big( \frac{L_x(\Lc_{\R^+}^\theta)}{2x} \Big), \quad \quad x \geq 0, n \geq 1.
\end{equation}
When $\theta = 1/2$, this definition agrees with the definition \eqref{E:def_Wick_GFF} of odd Wick powers of 1D Brownian motion. This follows from the identity \eqref{E:Laguerre_Hermite} between odd Hermite polynomials and the Laguerre polynomials $\mathbf{L}_n^{(\theta^*-1)}$ where $\theta^* = 3/2$.
In the following lemma, we show that these renormalised powers define martingales. In view of Lemma \ref{L:1D_martingale}, we believe that this normalisation has the potential to work in 2D as well. See Section \ref{S:expansion_signed} for much more about the two-dimensional case.

\begin{lemma}\label{L:1D_martingale2}
Let $\theta \in (0,1)$. The processes
\[
(h_{\theta,\R^+}(x))_{x \geq 0}, \quad \quad  (:h_{\theta,\R^+}(x) L_x(\Lc_{\R^+}^\theta)^n:)_{x \geq 0}, \quad \quad, n \geq 1,
\]
are martingales.
\end{lemma}

\begin{proof}
Let $n \geq 0$ (the case $n=0$ corresponding to $h_{\theta,\R^+}$). As before, denote by $(\Fc_t)_{t \geq 0}$ the natural filtration associated to $R$. 
By independence of the spins on different excursions and then by the relation \eqref{E:Bessel_duality} between Bessel processes with dimensions $d=2\theta$ and $d^* = 4-d=2\theta^*$, we obtain that for any $0 \leq s < t$,
\begin{align*}
\Es^d \left[ :h_{\theta,\R^+}(t) L_t(\Lc_{\R^+}^\theta)^n: \Big\vert \Fc_s \right]
& = \sigma_{e_s} \Es^d \left[ R_t^{1-\theta} \indic{\forall u \in [s,t], R_u >0} (2t)^n \mathbf{L}_n^{(\theta^*-1)} \Big( \frac{L_t(\Lc_{\R^+}^\theta)}{2t} \Big) \Big\vert \Fc_s \right] \\
& = \sigma_{e_s} R_s^{1-\theta} \Es^{d^*} \left[ (2t)^n \mathbf{L}_n^{(\theta^*-1)} \Big( \frac{L_t(\Lc_{\R^+}^\theta)}{2t} \Big) \Big\vert \Fc_s \right].
\end{align*}
If $n=0$, this immediately gives the desired martingale property. If $n\geq 1$, we use Lemma \ref{L:1D_martingale} to conclude that
\[
\Expect{ :h_{\theta,\R^+}(t) L_t(\Lc_{\R^+}^\theta)^n: \Big\vert \Fc_s }
= \sigma_{e_s} R_s^{1-\theta} (2s)^n \mathbf{L}_n^{(\theta^*-1)} \Big( \frac{L_s(\Lc_{\R^+}^\theta)}{2s} \Big)
= ~:\!h_{\theta,\R^+}(s) L_s(\Lc_{\R^+}^\theta)^n\!:.
\]
The last equality follows by definition. This concludes the proof.
\end{proof}

==> subfiles/1D_old.tex <==
In this section, we study the analogue of the field $h_\theta$ in the one-dimensional case.
This is partly motivated by the recent connection between the 1D and 2D loop soup discovered in \cite{JLQ23a}.
As we will recall in Theorem \ref{T:1Disomorphism} below, the local time of the 1D loop soup is distributed as a (reflected) squared Bessel process of dimension $d=2\theta$.
When $\theta=1/2$, obtaining a Brownian motion (1D analogue of the GFF) from the loop soup then boils down to taking the square root of a (reflected) 1D squared Bessel process and then flipping each excursion independently of each other with equal probability.
What is the analogue of this procedure when $\theta \neq 1/2$? 
We will see that, surprisingly, taking the square root is not the right thing to do (although this might be very natural since the square root of a squared Bessel process is just a Bessel process) and that one has to take the power $1-\theta = 1-d/2$ instead. This power is exactly the one appearing in the Radon--Nikodym derivative of the Bessel process and its dual Bessel process of dimension $d^* = 4 -d = 2\theta^*$ where $\theta^* = 2-\theta$; see \eqref{E:Bessel_duality}. The purpose of this section is also to hint at the duality between the intensities $\theta$ and $2-\theta$ that might still hold in some sense in dimension two. See Section \ref{S:expansion_signed} for more details concerning the 2D case.

\subsubsection{Loop soup on $\R^+$}

Let us start by defining the loop soup on the half line $\R^+$. We follow \cite{Lupu18}.
For $x,y \in \R^+$, let $p(t,x,y)$ and $p_{\R^+}(t,x,y)$ be the heat kernels on $\R$ and $\R^+$:
\[
p(t,x,y) = \frac{1}{\sqrt{2\pi t}} e^{-(y-x)^2/(2t)}, \quad p_{\R^+}(t,x,y) = p(t,x,y) - p(t,x,-y)
\]
and let $\P_{\R^+}^{t,x,y}$ be the law of a Brownian bridge from $x$ to $y$ of duration $t$ in the half line $\R^+$. 
The Green function and the loop measure are respectively given by
\[
G_{\R^+}(x,y) = \int_0^\infty p_{\R^+}(t,x,y) \d t = 2 x \wedge y
\quad \text{and} \quad
\loopmeasure_{\R^+} = \int_0^\infty \frac{p_{\R^+}(t,x,x)}{t} \P_{\R^+}^{t,x,x} \d t.
\]
For $\theta >0$, the loop soup $\Lc_{\R^+}^\theta$ in $\R^+$ with parameter $\theta$ is distributed according to a Poisson Point Process with intensity $\theta \loopmeasure_{\R^+}$. Compared to the 2D case, the local time of $\Lc_{\R^+}^\theta$ is well defined pointwise and finite and we will denote it
\[
L_x(\Lc_{\R^+}^\theta) = \sum_{\wp \in \Lc_{\R^+}^\theta} L_x(\wp) = \sum_{\wp \in \Lc_{\R^+}^\theta} \int_0^{T(\wp)} \indic{\wp_t = x} \d t, \quad \quad x \in \R^+.
\]

\begin{theorem}[\cite{Lupu18}]\label{T:1Disomorphism}
Let $\theta>0$.
$(L_x(\Lc_{\R^+}^\theta))_{x \geq 0}$ has the law of a squared Bessel process of dimension $d=2\theta$, reflected at 0 when $\theta <1$.
\end{theorem}

Let $\Ps^d$ be the law under which $(R_x,x \geq 0)$ is a squared Bessel process of dimension $d=2\theta$, reflected at 0 when $\theta <1$.
The clusters of $\Lc_{\R^+}^\theta$ correspond to the excursions away from 0 of $R$. Therefore Theorem \ref{T:1Disomorphism} implies that when $\theta <1$ there are infinitely many clusters and when $\theta \geq 1$ there is only one cluster. Notice that the critical point is different from the two-dimensional case. However, we show in \cite[Theorem 1.9]{JLQ23a} that there is a phase transition at $\theta = 1$ in the percolative behaviour of large loops on the half-infinite cylinder $(0,\infty) \times \mathbb{S}^1$ (by conformal invariance, this translates to a phase transition in the percolative behaviour of large loops targeting a given point of some bounded 2D domain). See \cite[Section 1.3]{JLQ23a} for more details.


\subsubsection{Characterisation of Laguerre polynomials in terms of Bessel processes}

As already seen, the generalised Laguerre polynomials $\mathbf{L}_n^{(\theta-1)}$ have been used by Le Jan to renormalise the powers of the local time of the loop soup in dimension two. In this section, we show that these polynomials are also special in dimension one in the sense that they are the only polynomials leading to martingales. See Lemma \ref{L:1D_martingale} for a precise statement. 

For any $\theta>0$, the Wick powers of the local time $L_x(\Lc_{\R^+}^\theta)$ are defined by
\begin{equation}
\label{E:1D_power}
:L_x(\Lc_{\R^+}^\theta)^n:
\quad = \quad (2x)^n \mathbf{L}_n^{(\theta-1)} \Big( \frac{L_x(\Lc_{\R^+}^\theta)}{2x} \Big), \quad \quad x \geq 0, n \geq 1.
\end{equation}
In the special case $\theta = 1/2$ this corresponds to the even Wick powers of 1D Brownian motion.


\begin{lemma}\label{L:1D_martingale}
Let $\theta >0$ and $n \geq 1$. The process $ (:L_x(\Lc_{\R^+}^\theta)^n:)_{x \geq 0}$ is a martingale.
Moreover, $\mathbf{L}_n^{(\theta-1)}$ is the only monic polynomial such that \eqref{E:1D_power} is a martingale.
\end{lemma}

Let us stress that it is a well known fact that the Wick powers of 1D Brownian motion lead to martingales. However, it seems to be new when $\theta \neq 1/2$.

\begin{proof}
Because in this lemma the space $\R^+$ is thought of as time, we will change the notations $x$ and $y$ for the space variables by $s$ and $t$. We will denote by $(\Fc_t)_{t \geq 0}$ the natural filtration of the Bessel process.
Let $X_t = \sqrt{R_t}$ be a Bessel process of dimension $d=2\theta$. Recall that $X_t$ satisfies the stochastic differential equation
$
\d X_t = \frac{d-1}{2 X_t} \d t + \d B_t
$
where $(B_t)_{t \geq 0}$ is a 1D standard Brownian motion. A computation using It\^{o} formula leads to the following SDE for $: L_t(\Lc_{\R^+}^\theta)^n :$ (we write $\mathbf{L}_n$ instead of $\mathbf{L}_n^{(\theta-1)}$)
\begin{align*}
\d \left\{ (2t)^n \mathbf{L}_n^{(\theta-1)} \Big( \frac{X_t^2}{2t} \Big) \right\}
& = 2^nt^{n-1} X_t \mathbf{L}_n' \Big( \frac{X_t^2}{2t} \Big) \d B_t \\
& + 2^nt^{n-1} \left\{ n \mathbf{L}_n \Big( \frac{X_t^2}{2t} \Big) + \Big( \theta - \frac{X_t^2}{2t} \Big) \mathbf{L}_n' \Big( \frac{X_t^2}{2t} \Big) + \frac{X_t^2}{2t} \mathbf{L}_n'' \Big( \frac{X_t^2}{2t} \Big) \right\} \d t.
\end{align*}
Because $\mathbf{L}_n = \mathbf{L}_n^{(\theta-1)}$ satisfies $n \mathbf{L}_n(u) + (\theta - u) \mathbf{L}_n'(u) + u \mathbf{L}_n''(u) = 0$ (see e.g. (22.1.3) and (22.8.6) in \cite{special}), we see that the finite variation part vanishes. In other words, $(: L_t(\Lc_{\R^+}^\theta)^n :)_{t \geq 0}$ is a local martingale. A routine argument concludes that it is a martingale as desired.

The fact that $\mathbf{L}_n = \mathbf{L}_n^{(\theta-1)}$ is the only monic polynomial such that \eqref{E:1D_power} is a martingale follows from the fact that it is the only monic polynomial satisfying $n \mathbf{L}_n(u) + (\theta - u) \mathbf{L}_n'(u) + u \mathbf{L}_n''(u) = 0$.
\end{proof}



\subsubsection{Analogue of $h_\theta$ on $\R^+$ and renormalisation of its powers}


Assume that $\theta < 1$ (subcritical regime for 1D loop soups).
In this section we define the natural analogue $h_{\theta, \R^+}$ of $h_\theta$ on $\R^+$ and give a procedure to renormalise its ``odd'' powers. Let $R$ be a $2\theta$-dimensional squared Bessel process. Let $\Ec$ be the set of excursions of $R$ and, conditionally on $\Ec$, let $\sigma_e, e \in \Ec$ be i.i.d. spins taking values in $\{ \pm 1\}$ with equal probability. Define
\[
h_{\theta, \R^+}(x) := \sigma_{e_x} R_x^{1-\theta}, \quad \quad x \geq 0,
\]
where $e_x$ is the excursion containing $x$.


The following result computes the two-point function of the field $h_{\theta,\R^+}$ and shows that tilting the probability measure by $h_{\theta,\R^+}(x) h_{\theta,\R^+}(y)$ amounts to changing the dimension of the Bessel process to its dual $d^* = 4-d$. Equivalently, this changes the intensity of the loop soup to $\theta^* = 2-\theta$.

\begin{lemma}\label{L:2point1D}
Let $\theta \in (0,1)$.
For all $0 \leq x \leq y$, and all bounded measurable function $F$,
\begin{equation}
\label{E:two-point1D}
\Es^d \left[ h_{\theta, \R^+}(x) h_{\theta, \R^+}(y) F( (R_z)_{z \in [x,y]}) \right] = \frac{\Gamma(\theta^*)}{\Gamma(\theta)} G_{\R^+}(x,y)^{2(1-\theta)} \Es^{d^*} \left[ F( (R_z)_{z \in [x,y]}) \right]
\end{equation}
where $d^* = 4-d = 2 \theta^*$ and $\theta^* = 2-\theta$.
\end{lemma}



\begin{proof}
By independence of the signs on different clusters and then by Markov property, we have
\begin{align*}
\Es^d \left[ h_{\theta, \R^+}(x) h_{\theta, \R^+}(y) F( (R_z)_{z \in [x,y]}) \right]
& = \Es^d \left[ R_x^{1-\theta} R_y^{1-\theta} \indic{\forall z \in [x,y], R_z>0} F( (R_z)_{z \in [x,y]}) \right] \\
& = \Es^d \left[ R_x^{1-\theta} \Es^d_{R_x} \left[ R_{y-x}^{1-\theta} \indic{ \forall z \in [0,y-x], R_z >0 } F( (R_z)_{z \in [0,y-x]}) \right] \right].
\end{align*}
As already mentioned, the key observation is that the power $1-\theta$ is exactly the power one needs to take in order to obtain the dual Bessel process of dimension $d^* = 4-d$. More precisely, for any $t>0$ and starting point $r>0$, restricted to the event that $\{ \forall s \in [0,t], R_s >0 \}$, we have
\begin{equation}
\label{E:Bessel_duality}
\frac{\d \P_r^{d^*}}{\d \P_r^{d}} {}_{\big\vert_{\Fc_t}} = \left( \frac{R_t}{r} \right)^{1-d/2}
\end{equation}
where $(\Fc_s)_{s \geq 0}$ is the natural filtration associated to $(R_s)_{s \geq 0}$.
See \cite[Proposition 2.2]{LawlerBessel}.
This implies that the left hand side of \eqref{E:two-point1D} is equal to
\begin{align*}
\Es^d \left[ R_x^{2(1-\theta)} \Es^{d^*}_{R_x} \left[ \indic{ \forall z \in [0,y-x], R_z >0 } F( (R_z)_{z \in [0,y-x]}) \right] \right] = \Es^d \left[ R_x^{2(1-\theta)} \Es_{R_x}^{d^*} \left[ F( (R_z)_{z \in [0,y-x]}) \right] \right]
\end{align*}
since the dual Bessel process does not reach zero a.s. ($d^* \geq 2$).
Under $\Ps^d$, $R_x$ is Gamma$(\theta,2x)$-distributed ($\theta$ and $2x$ are respectively the shape and scale parameters). A computation with Gamma distributions shows that for any measurable function $f: [0,\infty) \to \R$,
\[
\Es^d \left[ R_x^{2(1-\theta)} f(R_x) \right]
= \Es^d \left[ R_x^{2(1-\theta)} \right] \Es^{d^*} \left[ f(R_x) \right]
= (2x)^{2(1-\theta)} \frac{\Gamma(2-\theta)}{\Gamma(\theta)} \Es^{d^*} \left[ f(R_x) \right].
\]
Wrapping things up and by Markov property, we have obtained that the left hand side of \eqref{E:two-point1D} is equal to
\begin{align*}
(2x)^{2(1-\theta)} \frac{\Gamma(2-\theta)}{\Gamma(\theta)} \Es^{d^*} \left[ \Es_{R_x}^{d^*} \left[ F( (R_z)_{z \in [0,y-x]}) \right] \right] 
= (2x)^{2(1-\theta)} \frac{\Gamma(2-\theta)}{\Gamma(\theta)} \Es^{d^*} \left[ F( (R_z)_{z \in [x,y]}) \right].
\end{align*}
Lemma \ref{L:2point1D} then follows from the fact that $G_{\R^+}(x,y) = 2x$.
\end{proof}

When $\theta \in (0,1)$, Lemma \ref{L:2point1D} suggests to define the ``odd'' powers (i.e. powers that are not integer powers of the local time) of $h_{\theta,\R^+}$ by
\begin{equation}
:h_{\theta,\R^+}(x) L_x(\Lc_{\R^+}^\theta)^n:
\quad = \quad (2x)^n h_{\theta,\R^+}(x) \mathbf{L}_n^{(\theta^*-1)} \Big( \frac{L_x(\Lc_{\R^+}^\theta)}{2x} \Big), \quad \quad x \geq 0, n \geq 1.
\end{equation}
When $\theta = 1/2$, this definition agrees with the definition \eqref{E:def_Wick_GFF} of odd Wick powers of 1D Brownian motion. This follows from the identity \eqref{E:Laguerre_Hermite} between odd Hermite polynomials and the Laguerre polynomials $\mathbf{L}_n^{(\theta^*-1)}$ where $\theta^* = 3/2$.
In the following lemma, we show that these renormalised powers define martingales. In view of Lemma \ref{L:1D_martingale}, we believe that this normalisation has the potential to work in 2D as well. See Section \ref{S:expansion_signed} for much more about the two-dimensional case.

\begin{lemma}\label{L:1D_martingale2}
Let $\theta \in (0,1)$. The processes
\[
(h_{\theta,\R^+}(x))_{x \geq 0}, \quad \quad  (:h_{\theta,\R^+}(x) L_x(\Lc_{\R^+}^\theta)^n:)_{x \geq 0}, \quad \quad, n \geq 1,
\]
are martingales.
\end{lemma}

\begin{proof}
Let $n \geq 0$ (the case $n=0$ corresponding to $h_{\theta,\R^+}$). As before, denote by $(\Fc_t)_{t \geq 0}$ the natural filtration associated to $R$. 
By independence of the spins on different excursions and then by the relation \eqref{E:Bessel_duality} between Bessel processes with dimensions $d=2\theta$ and $d^* = 4-d=2\theta^*$, we obtain that for any $0 \leq s < t$,
\begin{align*}
\Es^d \left[ :h_{\theta,\R^+}(t) L_t(\Lc_{\R^+}^\theta)^n: \Big\vert \Fc_s \right]
& = \sigma_{e_s} \Es^d \left[ R_t^{1-\theta} \indic{\forall u \in [s,t], R_u >0} (2t)^n \mathbf{L}_n^{(\theta^*-1)} \Big( \frac{L_t(\Lc_{\R^+}^\theta)}{2t} \Big) \Big\vert \Fc_s \right] \\
& = \sigma_{e_s} R_s^{1-\theta} \Es^{d^*} \left[ (2t)^n \mathbf{L}_n^{(\theta^*-1)} \Big( \frac{L_t(\Lc_{\R^+}^\theta)}{2t} \Big) \Big\vert \Fc_s \right].
\end{align*}
If $n=0$, this immediately gives the desired martingale property. If $n\geq 1$, we use Lemma \ref{L:1D_martingale} to conclude that
\[
\Expect{ :h_{\theta,\R^+}(t) L_t(\Lc_{\R^+}^\theta)^n: \Big\vert \Fc_s }
= \sigma_{e_s} R_s^{1-\theta} (2s)^n \mathbf{L}_n^{(\theta^*-1)} \Big( \frac{L_s(\Lc_{\R^+}^\theta)}{2s} \Big)
= ~:\!h_{\theta,\R^+}(s) L_s(\Lc_{\R^+}^\theta)^n\!:.
\]
The last equality follows by definition. This concludes the proof.
\end{proof}

==> subfiles/Wick_old.tex <==
\subsection{Main results}


The Wick powers of the GFF $h$, denoted by $:\!h^n\!:, n \geq 2$, give a precise meaning to $h^n$, $n \geq 2$. Because the GFF is only a generalised function, taking such powers is \textit{a priori} not a well defined operation. A non trivial fact is that it is actually possible to make sense of these powers via a renormalisation procedure. Contrary to the renormalisation of the exponential of the field, the renormalisation is not multiplicative but additive: one subtracts to $h(x)^n$ a polynomial in $h(x)$ with diverging coefficients and degree strictly smaller than $n$. See Section \ref{S:Wick_recall} for more details. 


The Wick renormalisation of the powers of the GFF $h$ provides another approach to the multiplicative chaos of the field. Indeed, by naively expanding the exponential around 0, one could hope to define the exponential of $\gamma$ times the GFF $h$ by
\begin{equation}
\label{E:expansion_Liouville}
:\!e^{\gamma h(x)} \d x\!:
\quad = \quad
\sum_{n \geq 0} \frac{\gamma^n}{n!} :\!h^n\!:.
\end{equation}
It is well known that this procedure works in the $L^2$-phase (see e.g. \cite[Section 2.3]{lacoin2017semiclassical}) in the sense that the above sum converges to a random measure that agrees with the exponential of the field. See Remark \ref{R:complex_L2} for why \eqref{E:expansion_Liouville} does not hold outside of the $L^2$-phase. Note that it is \textit{a priori} not obvious that the resulting sum is nonnegative; eventually this boils down to \eqref{E:Hermite_exp}.

In the Brownian loop soup setting, Le Jan \cite{LeJan2011Loops} gave a construction of the renormalised powers $:\!L_x^n\!:$ of the local time $:\!L_x\!:$ for any intensity $\theta$. This is closely related to the (self-)intersection local time of Brownian motion (see the lecture notes \cite{LeGall92} and the references therein). 
In Section \ref{S:expansion_unsigned}, we will give the precise relation between the multiplicative chaos $\Mc_\gamma$ of the loop soup and these intersection local times. When $\theta=1/2$, this question reduces to the aforementioned GFF setting and we directly obtain that
\begin{equation}
\label{E:expansion_unsigned_critical}
\Mc_{\gamma,\theta=1/2}( \d x) = 2\sum_{n \geq 0} \frac{2^n \gamma^{2n}}{(2n)!} (2\pi)^n :\!L_x^n\!: \d x \quad \quad \text{a.s.}
\end{equation}
In Theorem \ref{T:expansion_unsigned}, we show that such a relation also holds for any intensity $\theta>0$. However, the coefficients in the expansion are different and depend on $\theta$:
\begin{equation}
\label{E:expansion_unsigned_general}
\Mc_\gamma(\d x) = 2 \sum_{n \geq 0} \frac{\gamma^{2n}}{2^n} \frac{\Gamma(\theta)}{n! \Gamma(n + \theta)} (2\pi)^n :L_x^n: \d x \quad \quad \text{a.s.}
\end{equation}
See Theorem \ref{T:expansion_unsigned} for a precise statement.


\medskip

As already alluded to, when $\theta =1/2$, the Wick powers of the local time reduce to the even powers of the GFF. To define the odd powers, one has to take into account the sign of the field.
In Sections \ref{S:1D} and \ref{S:expansion_signed} we address the question of defining \emph{all} the powers of the field $h_\theta$ for any intensity $\theta \in (0,1/2)$.
We showed in \cite{JLQ23a} that the 1D and 2D loop soups are intimately related.
We will therefore start in Section \ref{S:1D} by building our intuition with the one-dimensional setting. This case is particularly appealing since for any $\theta$, there is an isomorphism relating the local time of the loop soup to a squared Bessel process of dimension $d=2\theta$, see \cite{Lupu18} and Theorem \ref{T:1Disomorphism} below.
In dimension 1, the analogue of the field $h_\theta$ and the local time are both well defined pointwise, so there is no need of normalising the powers to define them. However, we will show in Lemmas \ref{L:1D_martingale} and \ref{L:1D_martingale2} that there is a unique way of normalising the powers so that the resulting process is a martingale. When these powers are integer powers of the local time, this normalisation agrees with Le Jan's two-dimensional normalisation procedure (generalised Laguerre polynomials). 
%For ``odd'' powers (that take into account the sign of $h_\theta$), this normalisation reveals a notion of duality between loop soups with intensity $\theta$ and $\theta^* = 2-\theta$.

In Section \ref{S:expansion_signed}, we will come back to the 2D setting and state a precise conjecture about a renormalisation procedure that would define all the Wick powers of $h_\theta$; see Conjecture \ref{Conjecture1}. This procedure in particular reveals a surprising notion of \emph{duality} between the intensities $\theta$ and $\theta^* = 2-\theta$.
We then elaborate on this conjecture and show that it would imply the following expansion for the measure $\Mc_\gamma^+$: almost surely,
\[
\Mc_\gamma^+(\d x) = \Big( \sum_{k \geq 0} \frac{\gamma^{2k}}{2^k} \frac{\Gamma(\theta)}{k! \Gamma(k+\theta)} (2\pi)^k :L_x^k:
+ c_\mathrm{conj} \gamma^{2(1-\theta)} \frac{\gamma^{2k}}{2^k} \frac{\Gamma(\theta^*)}{k! \Gamma(k+\theta^*)} (2\pi)^k :h_\theta(x) L_x^k: \Big) \d x.
\]
See Section \ref{S:expansion_signed} for the definition of the different terms appearing in the above display.







\subsection{Renormalised powers of the GFF and of the occupation field of the loop soup}
\label{S:Wick_recall}


The purpose of this section is to recall the definition of the Wick powers of the GFF and of the local time of the loop soup. We start by working in the discrete setting where everything is well defined pointwise. Let $D_N \subset \frac1N \Z^2$ be a discrete approximation of $D$ as in \eqref{eq:DN}. Let $\Lc_{D_N}^\theta$ be a random walk loop soup in $D_N$ and denote by  $\ell_x$ the local time at $x$ (see \eqref{E:discrete_local_time}). Let $\varphi_N$ be a discrete GFF in $D_N$ whose covariance is given by the discrete Green function $G_N$. We will denote


To renormalise the powers of the GFF, the relevant polynomials are the Hermite polynomials $H_n, n \geq 0,$ which are the only monic\footnote{Monic means that the leading coefficient equals 1.} polynomials that are orthogonal w.r.t. the Gaussian measure $e^{-x^2/2} \d x$ and such that the degree of $H_n$ is $n$ for all $n \geq 0$. They can be explicitly written as
\begin{equation}
H_n (X) = \sum_{i=0}^{\floor{n/2}} (-1)^i \frac{n!}{i! (n-2i)!} \frac{X^{n-2i}}{2^i}.
\end{equation}
The $n$-th Wick power of the discrete GFF $\varphi_N$ is then defined by
\begin{equation}
\label{E:def_Wick_GFF}
:\varphi_N(x)^n:
\quad = \quad
G_N(x,x)^{n/2} H_n \left( \varphi_N(x)/ \sqrt{G_N(x,x)} \right).
\end{equation}



Regarding the local time of the loop soup with intensity $\theta$, the relevant polynomials are the generalised Laguerre polynomials $\mathbf{L}_n^{(\theta-1)}$, $n \geq 0,$ which are the only monic polynomials that are orthogonal w.r.t. the Gamma$(\theta)$-measure $x^{\theta-1} e^{-x} \indic{x >0} \d x$ (which is natural since for any given point $x$, $\ell_x$ is Gamma$(\theta)$-distributed) and such that the degree of $\mathbf{L}_n^{(\theta-1)}$ is $n$ for all $n$. Their explicit expression is given by
\begin{equation}
\label{E:Laguerre}
\mathbf{L}_n^{(\theta-1)}(X) = \sum_{i=0}^n (-1)^{n-i} \frac{\Gamma(n+\theta)}{(n-i)! \Gamma(\theta+i)} \frac{n!}{i!} X^i.
\end{equation}
The $n$-th Wick power of the local time $\ell_x$ is defined by
\[
:\ell_x^n: \quad = \quad G_N(x,x)^n \mathbf{L}_n^{(\theta-1)}(\ell_x/G_N(x,x)).
\]

The following result states that these renormalisations in the discrete possess nondegenerate scaling limits. We will view $\varphi_N, :\varphi_N^n:, \ell$ and $:\ell^n:$, $n \geq 1$, as random elements of $\R^{C_0(D)}$ by setting for all $f \in C_0(D)$,
\[
\scalar{ \varphi_N, f } = \frac{1}{N^2} \sum_{x \in D_N} \varphi_N(x) f(x)
\]
and similarly for the other objects. We will endow $\R^{C_0(D)}$ with the product topology.


\begin{theorem}\label{T:Wick_convergence}
For all $n \geq 1$, $(\varphi_N, :\varphi_N^2:, \dots, :\varphi_N^n:)$ converges in distribution as $N \to \infty$ to some nondegenerate $(\varphi,:\varphi^2:, \dots, :\varphi^n:)$ where $:\varphi^2:, \dots, :\varphi^n:$ are measurable w.r.t. the Gaussian free field $\varphi$.

For all $n \geq 1$, $(:\ell:, :\ell^2:, \dots, :\ell^n:)$ converges in distribution as $N \to \infty$ to some $(:L:,:L^2:, \dots, :L^n:)$ where $:L^2:, \dots, :L^n:$ are measurable w.r.t. the renormalised occupation field $:L:$. Moreover the convergence is joint with the loop soup.
\end{theorem}

\begin{proof}
This is a folklore result. A proof of the joint convergence of $( \varphi_N, :\varphi_N^2: )$ can be found in \cite[Appendix A]{ABJL21}. This proof generalises to any power. It also applies to the local time case since it relies on the computation of moments that are well understood in the loop soup setting \cite{LeJan2011Loops}.
\end{proof}





\subsection{Expansion of \texorpdfstring{$\Mc_\gamma$}{M gamma}}
\label{S:expansion_unsigned}


The main result of this section is the expansion \eqref{E:expansion_unsigned_general} of the measure $\Mc_\gamma$ that we now state precisely:


\begin{theorem}[Expansion of $\Mc_\gamma$]
\label{T:expansion_unsigned}
Let $\theta >0$ and $\gamma \in (0,\sqrt{2})$. For any bounded test function $f: D \to \R$,
\begin{equation}
\label{E:expansion_function}
2 \sum_{n =0}^{n_0} \frac{\gamma^{2n}}{2^n} \frac{\Gamma(\theta)}{n! \Gamma(n + \theta)} \int (2\pi)^n :L_x^n: f(x) \d x
\xrightarrow[n_0 \to \infty]{L^2} \scalar{ \Mc_\gamma, f }.
\end{equation}
\end{theorem}

Let us emphasise that, contrary to most of the current article, the above result is not restricted to the subcritical and critical regimes, but holds for any intensity $\theta >0$.

\begin{remark}\label{R:complex_L2}
By (the proof of) Theorem \ref{T:expansion_unsigned}, for any bounded test function $f$ and complex values of $\gamma$ with $|\gamma| < \sqrt{2}$, the left hand side of \eqref{E:expansion_function} converges in $L^2$. This gives a direct way of generalising the definition of $\Mc_\gamma$ to complex values of $\gamma$ by defining $\scalar{\Mc_\gamma,f}$ as the limit of the left hand side of \eqref{E:expansion_function}. As in the Gaussian case, when $\gamma \notin \R$, the resulting object should not be a (complex) measure but only a generalised function.
In the Gaussian setting, it is actually possible to define a complex multiplicative chaos for complex values of $\gamma$ in the eye-shaped domain 
\[
\gamma \in \mathrm{convex~hull} \left( \pm 2 \cup D(0,\sqrt{2}) \right).
\]
We refer to the introduction of \cite{lacoin2022universality} for more background on complex Gaussian multiplicative chaos.
In our non-Gaussian setting, making sense of $\Mc_\gamma$ for non real values of $\gamma$ outside of the $L^2$-regime $\{ |\gamma| < \sqrt{2} \}$ is a much more challenging question that we do not address in this article.

Note that since it should not be possible to define $\Mc_\gamma$ outside of the (closure of the -- to avoid talking about boundary cases that are not fully understood in the complex case) above eye-shaped domain, the radius of convergence of the left hand side of \eqref{E:expansion_unsigned_general} should be $\sqrt{2}$. In other words, the fact that Theorem \ref{T:expansion_unsigned} does not consider the regime $\gamma \in [\sqrt{2}, 2)$ is not a limitation of the proof.
\end{remark}


\begin{remark}
Extrapolating the above result to the case of one Brownian trajectory ($\theta \to 0$), it is likely that the Brownian multiplicative chaos measure associated to one trajectory (considered in \cite{bass1994, AidekonHuShi2018, jegoBMC, jegoRW, jegoCritical}) can be written as the sum of the $n$-th self intersection local time of the path (see the lecture notes \cite{LeGall92} and the references therein).
\end{remark}


\medskip


We now move on to the proof of Theorem \ref{T:expansion_unsigned}.
In the GFF case, the relation \eqref{E:expansion_Liouville} eventually boils down to the identity:
\begin{equation}
\label{E:Hermite_exp}
\sum_{n \geq 0} \frac{\gamma^n t^{n/2}}{n!} H_n(u/\sqrt{t}) = e^{\gamma u - \gamma^2 t/2}, \quad \quad t,u \in \R.
\end{equation}
Essentially, this identity guarantees that \eqref{E:expansion_Liouville} holds even at the discrete level.
In order to extend \eqref{E:expansion_unsigned_critical} to general intensities, one has to find a way of summing the Laguerre polynomials in such a way that the resulting sum is positive and behaves asymptotically like the exponential in \eqref{E:Hermite_exp}. This algebraic property is the content of the next lemma (see \eqref{E:expansion_unsigned_discrete} for the discrete version of \eqref{E:expansion_unsigned_general}). This identity does not seem to have been noticed before. Recall the definition \eqref{E:BesselI} of the modified Bessel function of the first kind $I_{\theta-1}$. Recall also its asymptotic behaviour (see \cite[9.7.1]{special}):
\begin{equation}
\label{E:BesselI_asymp}
I_{\theta-1}(u) \sim \frac{1}{\sqrt{2\pi u}} e^u, \quad \quad \text{as} \quad u \to \infty.
\end{equation}




\begin{lemma}\label{L:Laguerre_Bessel}
For all $t, u, \gamma >0$,
\begin{equation}
\label{E:Laguerre_Bessel}
\sum_{n \geq 0} \left( \frac{\gamma^2 t}{2} \right)^n \frac{1}{n! \Gamma(\theta+n)} \mathbf{L}_n^{(\theta-1)} \left( \frac{u^2}{2t} \right) = e^{-\gamma^2 t/2} \left( \frac{\gamma^2 ut}{4} \right)^{\frac{1-\theta}{2}} I_{\theta-1} \left( \gamma u \right).
\end{equation}
\end{lemma}

\begin{proof}
This is a direct computation using the explicit expressions \eqref{E:Laguerre} and \eqref{E:BesselI} of the Laguerre polynomials and of $I_{\theta-1}$.
\begin{comment}
Using the explicit expression \eqref{E:Laguerre} of the polynomials $\mathbf{L}_n^{(\theta-1)}$ and then exchanging the order of summation, we see that the left hand side of \eqref{E:Laguerre_Bessel} is equal to
\begin{align*}
\sum_{n \geq 0} \sum_{i=0}^n (-1)^{n-i} \left( \frac{\gamma^2 t}{2} \right)^n \frac{1}{(n-i)! i!\Gamma(\theta+i)} \left( \frac{u^2}{2t} \right)^i
= e^{-\gamma^2 t/2} \sum_{i \geq 0} \left( \frac{\gamma^2 u^2}{4} \right)^i \frac{1}{i!\Gamma(\theta+i)}.
\end{align*}
By definition \eqref{E:BesselI} of $I_{\theta-1}$ this agrees with the right hand side of \eqref{E:Laguerre_Bessel}.
\end{comment}
\end{proof}

Specifying Lemma \ref{L:Laguerre_Bessel} to $u = \sqrt{2 \times 2\pi \ell_x}$ and $t = 2\pi G_N(x,x)$, we obtain
\begin{equation}
\label{E:expansion_unsigned_discrete}
\Big( \frac{\gamma^2}{2} 2\pi \ell_x \Big)^{\frac{1-\theta}{2}} e^{-\frac{\gamma^2}{2} 2\pi G_N(x,x)} I_{\theta-1} \left( \gamma \sqrt{2 \times 2 \pi \ell_x} \right) = \sum_{n \geq 0} \frac{\gamma^{2n}}{2^n} \frac{1}{n! \Gamma(n + \theta)} (2\pi)^n :\ell_x^n: \quad \quad \text{a.s.}
\end{equation}
This is the discrete version of Theorem \ref{T:expansion_unsigned} that we are now ready to prove.

\begin{proof}[Proof of Theorem \ref{T:expansion_unsigned}]
Let $f: D \to \R$ be a bounded test function.
We start by showing that the left hand side of \eqref{E:expansion_function} converges in $L^2$. For $n_0 \geq 1$, we write
\[
S_{n_0} := \sum_{n=0}^{n_0} \frac{\gamma^{2n}}{2^n} \frac{\Gamma(\theta)}{n! \Gamma(n + \theta)} \int (2\pi)^n :L_x^n: f(x) \d x.
\]
Let $n_0 < n_1$ be two integers.
By the equation (4.6) in \cite{LeJan2011Loops} (beware that our normalisation of $:L_x^n:$ is $n!$ times Le Jan's normalisation), for all $n, m \geq 1$ and $z, w \in D$, we have
\begin{equation}
\label{E:covariance_Wick}
\Expect{ :L_z^n: : L_w^m: } = \indic{n=m} \frac{\Gamma(\theta+n)n!}{\Gamma(\theta)} G_D(z,w)^{2n}.
\end{equation}
Hence,
\begin{align*}
& \Expect{ \left( S_{n_1} - S_{n_0} \right)^2 } = \frac{1}{\Gamma(\theta)} \sum_{n = n_0}^{n_1} \frac{\gamma^{4n}}{2^{2n}} \frac{1}{n! \Gamma(n+\theta)} \int_{D \times D} (2\pi)^{2n} G_D(z,w)^{2n} ~\d z~\d w.
\end{align*}
We can moreover bound for all $n \geq 0$,
\[
\int_{D \times D} (2\pi)^{2n} G_D(z,w)^{2n} ~\d z~\d w
\leq C \int_0^1 r (\log r)^{2n} \d r = C 2^{-2n} n (2n-1)!
\]
which implies that
\begin{align*}
& \Expect{ \left( S_{n_1} - S_{n_0} \right)^2 }
\leq C \sum_{n = n_0}^{n_1} \frac{\gamma^{4n}}{2^{4n}} \frac{(2n)!}{n! \Gamma(n+\theta)}
\leq C \sum_{n \geq n_0} \sqrt{n} \frac{n!}{\Gamma(n+\theta)} \frac{\gamma^{4n}}{2^{2n}}.
\end{align*}
Since $\gamma < \sqrt{2}$, the above sum is finite and vanishes as $n_0 \to \infty$. This shows that $(S_{n_0}, n_0 \geq 1)$ is a Cauchy sequence in $L^2$ and in particular converges to a limiting random variable $S_\infty$. The main task actually consists in showing that $S_\infty$ agrees almost surely with $\frac12 \scalar{\Mc_\gamma, f}$.

We explain this identification now.
We want to take the limit of the relation \eqref{E:expansion_unsigned_discrete}. We start by considering the limit of the right hand side of \eqref{E:expansion_unsigned_discrete}. An analogous computation as the one we have just done in the continuum shows that
\[
\lim_{n_0 \to \infty} \limsup_{N \to \infty} \E \Big[ \Big( \sum_{n \geq n_0} \frac{\gamma^{2n}}{2^n} \frac{1}{n! \Gamma(n + \theta)} \frac{1}{N^2} \sum_{z \in D_N} f(z) (2\pi)^n :\ell_z^n: \Big)^2 \Big] = 0.
\]
This follows from the exact same computation that can be performed since \eqref{E:covariance_Wick} also holds in the discrete with the continuum Green function $G_D$ replaced by its discrete version $G_{D_N}$. These estimates about the tails of the sums in the discrete and in the continuum, in combination with Theorem \ref{T:Wick_convergence}, show that
\[
\sum_{n \geq 0} \frac{\gamma^{2n}}{2^n} \frac{1}{n! \Gamma(n + \theta)} \frac{1}{N^2} \sum_{z \in D_N} f(z) (2\pi)^n :\ell_z^n:
\xrightarrow[N \to \infty]{\mathrm{(d)}} S_\infty.
\]
Moreover, this convergence is joint with $\Lc_{D_N}^\theta \to \Lc_D^\theta$.

We now move to the convergence of the left hand side of \eqref{E:expansion_unsigned_discrete}.
Recall that $a = \gamma^2/2$.
By \cite[Theorem 1.12]{ABJL21},
\begin{equation}
\label{E:uniform_measure_discrete}
\frac{(\log N)^{1-\theta}}{N^{2-a}} \sum_{z \in D_N} \CR(z,D)^{-a} f(z) \indic{ 2 \pi \ell_z \geq a (\log N)^2 }
\end{equation}
converges in distribution as $N \to \infty$ to $c_* \scalar{ \Mc_\gamma, f }$ where $c_* = \frac{(2\sqrt{2})^a e^{a \gamma_{\text{EM}}}}{2 a^{1-\theta} \Gamma(\theta)}$ and $\gamma_{\text{EM}}$ is the Euler--Mascheroni constant. Moreover, the convergence is joint with $\Lc_{D_N}^\theta \to \Lc_D^\theta$.
We now argue that
\begin{align}
\label{E:compare0}
& \frac{1}{N^2} \sum_{z \in D_N} f(z) \left( \frac{\gamma^2}{2} 2\pi \ell_z \right)^{\frac{1-\theta}{2}} e^{-\frac{\gamma^2}{2} 2\pi G_N(z,z)} I_{\theta-1} \left( \gamma \sqrt{2 \times 2 \pi \ell_z} \right) \\
& - \frac{1}{c_* \Gamma(\theta)} \frac{(\log N)^{1-\theta}}{N^{2-a}} \sum_{z \in D_N} \CR(z,D)^{-a} f(z) \indic{ 2 \pi \ell_z \geq a (\log N)^2 }
\nonumber
\end{align}
goes to zero in $L^2$ as $N \to \infty$ (when $\gamma \in [\sqrt{2}, 2)$ this convergence should hold in $L^1$, but we do not need to consider this case here).
This type of arguments is now fairly routine in the multiplicative chaos literature. Indeed, it amounts to comparing two different types of approximations of the measure. One approximation is based on the uniform measure on the set of thick points. The other one basically consists in taking the exponential of the square root of the local time. See for instance \cite[Theorems 1.1 and 1.2]{jegoBMC} where a similar result is shown in the context of the local times of small circles of a given planar Brownian motion. Let us emphasise that the situation we are dealing with in this article is simpler than the one in \cite{jegoBMC} since we are only interested in the $L^2$-regime.

We are therefore not going to prove that \eqref{E:compare0} goes to zero in $L^2$. Instead, we are going to give some heuristics.
Using the asymptotic behaviour \eqref{E:BesselI_asymp} of $I_{\theta-1}$, we see that the first term in \eqref{E:compare0} is very close to
\begin{align*}
& \frac{1}{\sqrt{2\pi \gamma} 2^{1/4}} \frac{1}{N^2} \sum_{z \in D_N} f(z) (2\pi \ell_z)^{-1/4} \left( \frac{\gamma^2}{2} 2\pi \ell_z \right)^{\frac{1-\theta}{2}} e^{-\frac{\gamma^2}{2} 2\pi G_N(z,z)} e^{ \gamma \sqrt{2 \times 2 \pi \ell_z} }.
\end{align*}
By a Cameron-Martin type result, we also see that the shift $e^{ \gamma \sqrt{2 \times 2 \pi \ell_z} }$ makes $2\pi \ell_z / (\log N)^2$ very much concentrated around the value $a$. Hence, the power of $2\pi \ell_z$ in front of the exponential can be replaced by the same power of $a (\log N)^2$ and the first term of \eqref{E:compare0} is very close to
\[
\frac{1}{2\sqrt{\pi}} a^{1/2-\theta} \frac{(\log N)^{1/2-\theta}}{N^2} \sum_{z \in D_N} f(z) e^{-\frac{\gamma^2}{2} 2\pi G_N(z,z)} e^{ \gamma \sqrt{2 \times 2 \pi \ell_z} }.
\]
We are now back to the more familiar situation of comparing the uniform measure on the set of thick points and the exponential of the square root of the local time.

Overall, this shows that
\[
\frac{1}{N^2} \sum_{z \in D_N} f(z) \left( \frac{\gamma^2}{2} 2\pi \ell_z \right)^{\frac{1-\theta}{2}} e^{-\frac{\gamma^2}{2} 2\pi G_N(z,z)} I_{\theta-1} \left( \gamma \sqrt{2 \times 2 \pi \ell_z} \right)
\xrightarrow[N \to \infty]{\mathrm{(d)}} \frac{1}{\Gamma(\theta)} \scalar{\Mc_\gamma, f}
\]
jointly with the convergence $\Lc_{D_N}^\theta \to \Lc_D^\theta$.
Wrapping things up, and recalling that $2S_\infty$ denotes the $L^2$ limit of the left hand side of \eqref{E:expansion_function}, we have shown that
\[
\left( \scalar{ \Mc_\gamma, f }, \Lc_D^\theta \right)
\overset{\mathrm{(d)}}{=} \left( 2 S_\infty, \Lc_D^\theta \right).
\]
Because $\scalar{ \Mc_\gamma, f }$ and $2S_\infty$ are measurable w.r.t. $\Lc_D^\theta$, they must agree almost surely. This concludes the proof.
\end{proof}


\subsection{One-dimensional Brownian loop soup and Wick powers of Bessel processes}\label{S:1D}


\input{./subfiles/1D.tex}



\subsection{Wick powers involving \texorpdfstring{$h_\theta$}{h theta} and expansion of \texorpdfstring{$\Mc_\gamma^+$}{Mgamma+}}
\label{S:expansion_signed}


In this section we elaborate on Conjecture \ref{Conj:intro} by giving a much more precise conjecture (Conjecture \ref{Conjecture1} below) that would allow us to define \emph{all} the Wick powers of $h_\theta$. We will then show that this conjecture would have very strong implications concerning the asymptotic behaviour of the crossing probabilities studied in \cite{JLQ23a} and would also provide the expansion of the signed measure $\Mc_\gamma^+$; see \eqref{E:conj_crossing_probability} and \eqref{E:conj_expansion}.


Let us go back to the discrete setting first. Recall the definition \eqref{E:def_htheta_discrete} of $h_{\theta,N}$, the (conjecturally) analogue of $h_\theta$ in the discrete. We work on the cable graph so that $h_{\theta,N}$ is simply a discrete GFF.
The following lemma shows that the duality between $\theta$ and $\theta^* = 2-\theta$ that holds in the one-dimensional setting (Lemma \ref{L:2point1D}) also holds \emph{locally} in the two-dimensional setting when $\theta=1/2$; see also Remark \ref{rmk:isomorphism1/2}.

\begin{lemma}\label{L:duality_criticality}
Assume that $\theta=1/2$ and let $F : [0,\infty)^2 \to \R$ be a bounded measurable function. For all $x, y \in D_N$,
\begin{equation}
\label{E:duality_critical}
\Expect{ h_{\theta,N}(x) h_{\theta,N}(y) F(\ell_x(\Lc_{D_N}^\theta), \ell_y(\Lc_{D_N}^\theta)) }
= G_{D_N}(x,y) \Expect{ F(\ell_x(\Lc_{D_N}^{\theta^*}), \ell_y(\Lc_{D_N}^{\theta^*})) }
\end{equation}
where $\theta^* = 2-\theta = 3/2$.
\end{lemma}

The key ingredient in the proof of Lemma \ref{L:duality_criticality} is that the odd Hermite polynomials are related to the Laguerre polynomials $\mathbf{L}_n^{(\theta^*-1)}$ with $\theta^* = 3/2$. See \eqref{E:Laguerre_Hermite} below.

\begin{proof}
One could use the BFS-Dynkin isomorphism \eqref{E:BFS_Dynkin} to show this lemma. We will use another approach here that allows us to highlight some extra features of the Wick powers.
By density-type arguments, it is enough to prove \eqref{E:duality_critical} when $F(s,t) = P(s/G_{D_N}(x,x)) \times Q(t/G_{D_N}(y,y))$ is a product of two polynomials $P(\cdot/G_{D_N}(x,x))$ and $Q(\cdot/G_{D_N}(y,y))$. We can moreover assume that these polynomials belong to the basis $\{ \mathbf{L}_n^{(\theta^*-1)}, n \geq 0 \}$, i.e. that $P = \mathbf{L}_n^{(\theta^*-1)}$ and $Q = \mathbf{L}_m^{(\theta^*-1)}$ for some $n, m \geq 0$. The right hand side of \eqref{E:duality_critical} can then be computed directly thanks to the study of the renormalised local time of the loop soup with intensity $\theta^*$ (see \cite{LeJan2011Loops})
\[
\E \Big[ \mathbf{L}_n^{(\theta^*-1)} \Big( \frac{\ell_x(\Lc_{D_N}^{\theta^*})}{G_{D_N}(x,x)} \Big) \mathbf{L}_m^{(\theta^*-1)} \Big( \frac{\ell_y(\Lc_{D_N}^{\theta^*})}{G_{D_N}(y,y)} \Big) \Big]
= \indic{n=m} \frac{\Gamma(\theta^*+n)n!}{\Gamma(\theta^*)} \frac{G_{D_N}(x,y)^{2n}}{G_{D_N}(x,x)G_{D_N}(y,y)}.
\]
Concerning the left hand side term in \eqref{E:duality_critical}, we use the fact that $\ell_x(\Lc_{D_N}^{\theta}) = h_{\theta,N}(x)^2/2$ and the following identity between odd Hermite polynomials and Laguerre polynomials \cite[(22.5.41)]{special}
\begin{equation}
\label{E:Laguerre_Hermite}
\frac{1}{2^n} G^{\frac{2n+1}{2}} H_{2n+1}\left( \frac{h}{\sqrt{G}} \right)
= h G^n \mathbf{L}_n^{(\theta^*-1)} \left( \frac{h^2}{2G} \right), \quad \quad n\geq 0, h \in \R, G>0.
\end{equation}
Combining these two ingredients gives
\begin{align*}
& \E \Big[ h_{\theta,N}(x) h_{\theta,N}(y) \mathbf{L}_n^{(\theta^*-1)} \Big( \frac{\ell_x(\Lc_{D_N}^{\theta})}{G_{D_N}(x,x)} \Big) \mathbf{L}_m^{(\theta^*-1)} \Big( \frac{\ell_y(\Lc_{D_N}^{\theta})}{G_{D_N}(y,y)} \Big) \Big] \\
& = \frac{1}{2^{n+m}} G_{D_N}(x,x)^{1/2} G_{D_N}(y,y)^{1/2} \E \Big[ H_{2n+1} \Big( \frac{h_{\theta,N}(x)}{G_{D_N}(x,x)^{1/2}} \Big) H_{2m+1} \Big( \frac{h_{\theta,N}(y)}{G_{D_N}(y,y)^{1/2}} \Big) \Big] \\
& = \indic{n =m} \frac{(2n+1)!}{2^{2n}} \frac{G_{D_N}(x,y)^{2n+1}}{G_{D_N}(x,x)^n G_{D_N}(y,y)^n}
\end{align*}
where the last equality comes from the study of the Wick powers of the GFF (see \cite{LeJan2011Loops}).
Recalling that $\theta^* = 3/2$, one can check that $\frac{\Gamma(\theta^*+n)n!}{\Gamma(\theta^*)} = \frac{(2n+1)!}{2^{2n}}$ and we obtain that both sides of \eqref{E:duality_critical} are equal when $F(s,t) = \mathbf{L}_n^{(\theta^*-1)}(s / G_{D_N}(x,x)) \mathbf{L}_m^{(\theta^*-1)}(t / G_{D_N}(y,y))$. This concludes the proof.
\end{proof}


Let $\theta \in (0,1/2]$.
Lemmas \ref{L:2point1D}, \ref{L:1D_martingale2} and \ref{L:duality_criticality} suggest to define the Wick renormalisation of $h_{\theta,N}(x) \ell_x^n$ by
\begin{equation}
\label{E:Wick_def_conjecture}
:h_{\theta,N}(x) \ell_x^n: \quad = \quad h_{\theta,N}(x) G(x,x)^n \mathbf{L}_n^{(\theta^*-1)}(\ell_x / G(x,x))
\end{equation}
where $\theta^* = 2-\theta$. The relation \eqref{E:Laguerre_Hermite} between odd Hermite polynomials and Laguerre polynomials $\mathbf{L}_n^{(1/2)}$ guarantees that this renormalisation of $h_{\theta,N}(x) \ell_x^n$ is consistent with the usual renormalisation when $\theta=1/2$:
\[
:h_{\theta=1/2,N}(x) \ell_x^n:
\quad = \quad \frac{1}{ 2^n} G(x,x)^{\frac{2n+1}{2}} H_{2n+1} \left( \frac{h_{\theta=1/2,N}(x)}{\sqrt{G(x,x)}} \right).
\]
We make the following conjecture:

\begin{conjecture}\label{Conjecture1}
Let $\theta \in (0,1/2)$.
The Wick powers $:h_{\theta,N}(x) \ell_x^n:$ defined in \eqref{E:Wick_def_conjecture} have nondegenerate scaling limits. More precisely, for any $n_0 \geq 1$,
\[
\left( h_{\theta,N}, (:h_{\theta,N} \ell^n:)_{n=1 \dots n_0}, \Lc_{D_N}^\theta \right)
\xrightarrow[N \to \infty]{\mathrm{(d)}} \left(h_\theta^{\mathrm{conj}}, (:h_\theta^{\mathrm{conj}} L^n:)_{n =1 \dots n_0}, \Lc_D^\theta \right)
\]
where the right hand side term is defined by this limit. The convergence holds in the space $(H^{-\eps})^{n_0} \times \mathfrak{L}$ for any $\eps >0$. Moreover, $h_\theta^{\mathrm{conj}}$ and  $(:h_\theta^{\mathrm{conj}} L^n:)_{n =1 \dots n_0}$ are measurable w.r.t. $\Lc_D^\theta$.
\end{conjecture}

Let us stress that this conjecture is known when $\theta = 1/2$; see Theorem \ref{T:Wick_convergence}.
This conjecture is particularly appealing to us since:

\begin{theorem}\label{T:expansion_signed_discrete}
Let $\theta \in (0,1/2]$ and $\gamma \in (0,\sqrt{2})$. Define
\begin{equation}
\label{E:def_expansion_discrete_signed}
m_{\gamma,N}(x) = 
\sum_{k \geq 0} \frac{\gamma^{2k}}{2^k} \frac{\Gamma(\theta)}{k! \Gamma(k+\theta)} (2\pi)^k:\ell_x^k:
+ \gamma^{2(1-\theta)} \sum_{k \geq 0} \frac{\gamma^{2k}}{2^k} \frac{\Gamma(\theta^*)}{k! \Gamma(k+\theta^*)} (2\pi)^k :h_{\theta,N}(x) \ell_x^k:
\end{equation}
where the Wick powers $:h_{\theta,N}(x) \ell_x^k:$ are defined in \eqref{E:Wick_def_conjecture}.
For any bounded smooth test function $f$,
\begin{equation}
\frac{1}{N^2} \sum_{x \in D_N} f(x) m_{\gamma,N}(x) \xrightarrow[N \to \infty]{\mathrm{(d)}} \scalar{\Mc_\gamma^+,f}
\end{equation}
jointly with $\Lc_{D_N}^\theta \to \Lc_D^\theta$.
\end{theorem}

Let us emphasise that Theorem \ref{T:expansion_signed_discrete} is not conditionally on Conjecture \ref{Conjecture1}. This result is another strong indication that Conjecture \ref{Conjecture1} should hold.

\begin{proof}[Proof of Theorem \ref{T:expansion_signed_discrete}]
Let $m_{\gamma,N}^\mathrm{even}(x)$ and $m_{\gamma,N}^\mathrm{odd}(x)$ be respectively the first and second term on the right hand side of \eqref{E:def_expansion_discrete_signed}.
Recall that, as a consequence of Lemma \ref{L:Laguerre_Bessel}, we obtained that (see \eqref{E:expansion_unsigned_discrete})
\begin{align*}
m_{\gamma,N}^\mathrm{even}(x)
= 
\Gamma(\theta) \left( \frac{\gamma^2}{2} 2\pi\ell_x \right)^{\frac{1}{2} - \frac{\theta}{2}} e^{-\frac{\gamma^2}{2} G(x,x)} I_{\theta -1} ( \gamma \sqrt{2\times 2\pi \ell_x} ).
\end{align*}
Similarly, Lemma \ref{L:Laguerre_Bessel} applied to $\theta^*$ instead of $\theta$ yields
\begin{align*}
m_{\gamma,N}^\mathrm{odd}(x)
& = \gamma^{2(1-\theta)} h_{\theta,N}(x) \Gamma(\theta^*) 
\left( \frac{\gamma^2}{2} 2\pi\ell_x \right)^{\frac{1}{2} - \frac{\theta^*}{2}} e^{-\frac{\gamma^2}{2} G(x,x)} I_{\theta^* -1} ( \gamma \sqrt{2\times 2\pi\ell_x} ) \\
& = 2^{1-\theta} \Gamma(\theta^*) \left( \frac{\gamma^2}{2} \right)^{\frac{1}{2} - \frac{\theta}{2}} h_{\theta,N}(x) (2\pi\ell_x)^{\frac{1}{2} - \frac{\theta^*}{2}} e^{-\frac{\gamma^2}{2} G(x,x)} I_{\theta^* -1} ( \gamma \sqrt{2\times 2\pi \ell_x} ).
\end{align*}
Recall the definition \eqref{E:def_htheta_discrete} of $h_{\theta,N}$: $h_{\theta,N}(x) = c_\theta \sigma_x (2\pi\ell_x)^{1-\theta}$ where $c_\theta = 2^{\theta-1} \Gamma(\theta) / \Gamma(\theta^*)$. We can rewrite
$
h_{\theta,N}(x) (2\pi\ell_x)^{\frac{1}{2} - \frac{\theta^*}{2}} = c_\theta \sigma_x (2\pi\ell_x)^{\frac{1}{2} - \frac{\theta}{2}}
$
and we overall find that $m_{\gamma,N}(x)$ is equal to
\begin{align*}
\left( \frac{\gamma^2}{2} 2\pi \ell_x \right)^{\frac{1}{2} - \frac{\theta}{2}} e^{-\frac{\gamma^2}{2} G(x,x)} \left\{ \Gamma(\theta) I_{\theta -1} ( \gamma \sqrt{2\times 2\pi \ell_x} ) + 2^{1-\theta} \Gamma(\theta^*) c_\theta \sigma_x I_{\theta^* -1} ( \gamma \sqrt{2\times 2\pi \ell_x} ) \right\}.
\end{align*}
The constant $c_\theta$ has been chosen so that the two constants in front of the modified Bessel functions match (which is particularly important since they have the same asymptotic behaviour at infinity)
and
\begin{align*}
m_{\gamma,N}(x) = \Gamma(\theta) \left( \frac{\gamma^2}{2} 2\pi \ell_x \right)^{\frac{1}{2} - \frac{\theta}{2}} e^{-\frac{\gamma^2}{2} G(x,x)} \left\{  I_{\theta -1} ( \gamma \sqrt{2\times 2\pi \ell_x} ) + \sigma_x I_{\theta^* -1} ( \gamma \sqrt{2\times 2\pi \ell_x} ) \right\}.
\end{align*}
In the special case $\theta = 1/2$, we have
\[
I_{-1/2}(z) = \sqrt{\frac{2}{\pi z}} \cosh(z)
\quad \text{and} \quad
I_{1/2}(z) = \sqrt{\frac{2}{\pi z}} \sinh(z)
\]
and we do recover that
\[
m_{\gamma,N}(x) = \Gamma(1/2) \frac{1}{\sqrt{\pi}} e^{-\frac{\gamma^2}{2} G(x,x)} e^{\sigma_x \gamma \sqrt{2\times 2\pi \ell_x} } = e^{-\frac{\gamma^2}{2} G(x,x)} e^{\sigma_x \gamma \sqrt{2\times 2\pi\ell_x} }
\]
which converges to $:e^{\gamma h}:$ as $N \to \infty$. In general ($\theta \in (0,1/2]$), if $\sigma_x= -1$, the leading order terms of the two Bessel functions will cancel each other. Since the normalisation factor has been tuned to normalise these leading order terms, the subleading order terms will vanish in the scaling limit and the measure will concentrate on points with a positive spin. One can therefore use a similar reasoning as in the proof of Theorem \ref{T:expansion_unsigned} and compare $m_{\gamma,N}(x)$ with $\Mc_{a,N}(\d x) \indic{\sigma_x = 1}$. In Corollary \ref{C:discrete_ma+} we showed that this latter measure converges to $\Mc_\gamma^+$, so this argument shows that $m_{\gamma,N}(x)$ also converges to $\Mc_\gamma^+$.
\end{proof}


\paragraph*{Consequences of Conjecture \ref{Conjecture1}}
Let us now assume that Conjecture \ref{Conjecture1} holds and discuss the implications it would have. In the course of proving Conjecture \ref{Conjecture1}, it is likely that one would obtain a control on the growth of the correlation of $:h_{\theta,N}(x) \ell_x^n:$ and $:h_{\theta,N}(y) \ell_y^m:$ of a similar type as \eqref{E:covariance_Wick}. This control would ensure that most of the mass of $m_{\gamma,N}$ is carried by the first hundred terms say in the two sums in \eqref{E:def_expansion_discrete_signed}. This would then allow us to take the scaling limit of these sums (exactly like in the proof of Theorem \ref{T:expansion_unsigned}) and we would obtain, in conjunction with Theorem \ref{T:expansion_signed_discrete}, that
\begin{equation}
\label{E:conj_expansion}
\Mc_\gamma^+ = \sum_{k \geq 0} \frac{\gamma^{2k}}{2^k} \frac{\Gamma(\theta)}{k! \Gamma(k+\theta)} (2\pi)^k :L_x^k:
+ \gamma^{2(1-\theta)} \frac{\gamma^{2k}}{2^k} \frac{\Gamma(\theta^*)}{k! \Gamma(k+\theta^*)} (2\pi)^k :h_\theta^\mathrm{conj}(x) L_x^k:.
\end{equation}
In particular, this shows that the second order term in the expansion of $\Mc_\gamma^+$ is of order $\gamma^{2(1-\theta)}$ which would imply that the limit
\begin{equation}
\label{E:conj_crossing_probability}
c_{\mathrm{conj}} := \lim_{\gamma \to 0} \frac{Z_\gamma}{\gamma^{2(1-\theta)}} \in (0,\infty)
\end{equation}
exists and is nondegenerate. This would also identify $h_\theta^\mathrm{conj}$ with $c_\mathrm{conj} h_\theta$. Finally, with the help of a Tauberian theorem, it may be the case that the above convergence \eqref{E:conj_crossing_probability} implies the convergence of the crossing probability
\begin{equation}
\lim_{r \to 0} | \log r |^{1-\theta} \P \Big( e^{-1} \partial \D \overset{\Lc_\D^\theta}{\longleftrightarrow} r \D \Big) \in (0,\infty).
\end{equation}
This would be a considerable strengthening of the main result of \cite{JLQ23a} (see Theorem \ref{T:large_crossing}).


%
%Defining the Wick powers $:h_\theta(x) L_x^k:$ by $\frac{1}{c_\mathrm{conj}} :h_\theta^\mathrm{conj}(x) L_x^k:$, we would then obtain
%for all $\gamma \in (0,\sqrt{2})$, 
%\begin{equation}
%\label{E:conj_expansion}
%\Mc_\gamma^+ = \sum_{k \geq 0} \frac{\gamma^{2k}}{2^k} \frac{\Gamma(\theta)}{k! \Gamma(k+\theta)} (2\pi)^k :L_x^k:
%+ c_\mathrm{conj} \gamma^{2(1-\theta)} \frac{\gamma^{2k}}{2^k} \frac{\Gamma(\theta^*)}{k! \Gamma(k+\theta^*)} (2\pi)^k :h_\theta(x) L_x^k:.
%\end{equation}





\begin{comment}
\begin{remark}
\red{(Do we keep this remark?)} Let us notice that the hypergeometric function $s^{-\alpha} {}_2 F_1(\alpha+\theta,\alpha,1+\alpha+\theta,1-1/s)$, $\alpha \leq 1-\theta$, that naturally appeared in the proof of Lemma \ref{L:fixed-points} (see \eqref{E:Pfaff}), has an expansion of a very similar form as $s \to \infty$. Indeed, by using \eqref{E:Hypergeometric_01}, we have for all $s > 1$,
\begin{align*}
& s^{-\alpha} {}_2 F_1 \Big( \alpha+\theta,\alpha,1+\alpha+\theta,1-\frac{1}{s} \Big) \\
& = - \frac{\alpha+\theta}{1-\alpha} \frac1s ~{}_2 F_1 \Big( 1,1+\theta,2-\alpha,\frac{1}{s} \Big)
+ \frac{\Gamma(1+\alpha+\theta) \Gamma(1-\alpha)}{\Gamma(\theta+1)} \Big( \frac1s \Big)^\alpha {}_2 F_1 \Big( \alpha+\theta, \alpha, \alpha, \frac{1}{s} \Big)
\\
& = \sum_{k \geq 0} a_k \Big( \frac{1}{s} \Big)^{k+1} + b_k \Big( \frac1s \Big)^{\alpha +k}
\end{align*}
for some coefficients $a_k, b_k$. In particular, in the limiting case $\alpha = 1-\theta$, the expansion takes a similar form as the one in \eqref{E:conj_expansion}. At this stage, we do not know whether this is just a mere coincidence or not.
\end{remark}
\end{comment}



==> subfiles/app_sum.tex <==
\begin{lemma}\label{L:sum_elementary}
Let $(a_n)_{n \geq 1}$ be a sequence of non zero real numbers and let $(\sigma_n)_{n \geq 1}$ be i.i.d. spins taking values in $\{\pm 1\}$ with equal probability 1/2. Assume that $\sum_n \sigma_n a_n$ converges almost surely. Then the distribution of $\sum_n \sigma_n a_n$ is non-atomic.
\end{lemma}

\begin{proof}
Let $x \in \R$. We are going to show that $\sum_n \sigma_n a_n \neq x$ a.s. which will conclude the proof. The conditional probability $\Prob{ \sum_n \sigma_n a_n = x \vert \sigma_1, \dots, \sigma_{k-1} }$ converges a.s. to $\indic{\sum_n \sigma_n a_n = x}$ as $k \to \infty$. But, by flipping the $k$-th spin and using the fact that $a_k \neq 0$, we see that
\begin{align*}
\P \Big( \sum_n \sigma_n a_n = x \big\vert \{\sigma_i\}_{i=1}^{k-1} \Big)
& \leq \P \Big( \sum_{n \neq k} \sigma_n a_n -\sigma_k a_k \neq x \big\vert \{\sigma_i\}_{i=1}^{k-1}  \Big)  = \P \Big( \sum_n \sigma_n a_n \neq x \big\vert \{\sigma_i\}_{i=1}^{k-1}  \Big).
\end{align*}
Rearranging, this shows that  $\Prob{ \sum_n \sigma_n a_n = x \vert \sigma_1, \dots, \sigma_{k-1} } \leq 1/2$ a.s. Therefore, $\indic{\sum_n \sigma_n a_n = x}$ is at most $1/2$ a.s., meaning that  $\sum_n \sigma_n a_n \neq x$ a.s.
\end{proof}

==> subfiles/crossing.tex <==
\subsection{Decay rate of \texorpdfstring{$Z_\gamma$}{Z gamma}}


In this section, we apply Theorem \ref{T:large_crossing} to prove that, as stated in Theorem \ref{T:convergenceL2}, the normalising constant $Z_\gamma$ defined in \eqref{E:Zgamma} decays like $Z_\gamma = \gamma^{2(1-\theta)+o(1)}$ as $\gamma \to 0$. 

\begin{proof}[Proof of Theorem \ref{T:convergenceL2} -- Decay rate of $Z_\gamma$]
We start with the upper bound.
If the origin is connected to the circle $e^{-1} \partial \D$ by a cluster of $\Xi_a^{0,\D} \wedge \Lc_\D^\theta$, there must be a cluster of $\Lc_\D^\theta$ which intersects both $r \partial \D$ and $e^{-1} \partial \D$ where $r = \norme{ \Xi_a^{0,\D} }_\infty$.
By independence of $\Xi_a^{0,\D}$ and $\Lc_\D^\theta$ this gives
\begin{align*}
Z_\gamma & \leq \Prob{\norme{ \Xi_a^{0,\D} }_\infty \geq e^{-1} } + \int_0^{e^{-1}}  \Prob{\norme{ \Xi_a^{0,\D} }_\infty \in \d r} \Prob{ r \partial \D \overset{\Lc_\D^\theta}{\longleftrightarrow} e^{-1} \partial \D }.
\end{align*}
Let $\eps >0$. By Theorem \ref{T:large_crossing}, there exists $C_\eps >0$ such that the last probability in the above display is at most $C_\eps |\log r|^{-1+\theta+\eps}$ for all $r \in (0,e^{-1})$. Together with Lemma \ref{L:diameter_thick}, we obtain that
\[
Z_\gamma
\leq 1 - e^{-a} + \int_0^{e^{-1}} a r^{a-1} C_\eps |\log r|^{-1+\theta +\eps} \d r \sim C_\eps \Gamma(\theta + \eps) a^{1-\theta - \eps}
\]
as $a \to 0$. Since $a = \gamma^2/2$, this proves the desired upper bound: $Z_\gamma \leq \gamma^{2(1-\theta)+o(1)}$.

We now turn to the lower bound. The event $\{ 0 \overset{\Lc_\D^\theta \wedge \Xi_a^{0,\D}}{\longleftrightarrow} e^{-1} \partial \D \}$ occurs as soon as
1) $\Xi_a^{0,\D}$ reaches $e^{-1/a} \partial \D$,
2) a cluster of $\Lc_\D^\theta$ intersects the circles $e^{-2/a} \partial \D$ and $e^{-1} \partial \D$ and
3) there is a loop in $\Lc_\D^\theta$ surrounding $e^{-2/a} \D$ while staying in $e^{-1/a} \D$.
By independence of $\Xi_a^{0,\D}$ and $\Lc_\D^\theta$ and by FKG, the probability of the intersection of these three events is at least the product of each probability. By Lemma \ref{L:diameter_thick}, the probability of the first event is $1 - e^{-1}$. By Theorem \ref{T:large_crossing}, the probability of the second event is $a^{1-\theta + o(1)}$. By ***, the probability of the last event is $1 + o(1)$. Overall, we conclude that $Z_\gamma \geq a^{1-\theta + o(1)} = \gamma^{2(1-\theta)+o(1)}$.
\end{proof}

==> subfiles/field.tex <==
We start by stating without proof key results needed in order to prove Theorems \ref{T:convergenceL2}, \ref{T:cluster2point} and \ref{T:cluster_xy_doob}. We will then show how these theorems are deduced. The rest of the section will then consist of the proofs of these intermediate results.
We start with a lemma that shows that computing the second moment of $h_\gamma$ boils down to computing crossing probabilities between $x$ and $y$ in a soup whose loops come from
1) an unconditioned Brownian loop soup $\Lc_D^\theta$,
2) a thick loop $\Xi_a^x$ at $x$ and
3) a thick loop $\Xi_a^y$ at $y$.


\begin{lemma}\label{L:second_moment_to_crossing_proba}
Let $\eps >0$ and $F : D \times D \times \mathfrak{L} \to \R$ be a bounded measurable admissible function such that for all $x,y \in D$, $F(x,y, \cdot)$ does not depend on loops with diameter smaller than $\eps$. For all $\gamma, \gamma' \in (0,\sqrt{2})$,
\begin{align}
\label{E:L_second_moment_to_crossing_proba}
& \Expect{ \int_{D \times D} F(x,y,\Lc_D^\theta) h_{\gamma}(x) h_{\gamma'}(y) \d x \d y } \\
& = \frac{1}{Z_{\gamma} Z_{\gamma'}} \int_{D \times D} \E \Big[ F(x,y,\Lc_D^\theta \cup \{\Xi_{a_i}^x \}_{i \geq 1} \cup \{\Xi_{a_i'}^y \}_{i \geq 1}) \mathbf{1} \Big\{ x \overset{\Lc_D^\theta \cup \{\Xi_{a_i}^x \}_{i \geq 1} \cup \{\Xi_{a_i'}^y \}_{i \geq 1}}{\longleftrightarrow} y \Big\} \Big] \d x \d y 
+ O(1) \frac{\gamma^2 {\gamma'}^2}{Z_{\gamma} Z_{\gamma'}}
\nonumber
\end{align}
where the three collections of loops $\Lc_D^\theta$, $\{\Xi_{a_i}^x \}_{i \geq 1}$ and $\{ \Xi_{a_i'}^y \}_{i \geq 1}$ are independent and distributed as in Lemma \ref{L:moment_measure}.
The $O(1)$ above is bounded uniformly in $\gamma, \gamma'$ in compact subsets of $[0,\sqrt{2})$.
\end{lemma}


The next two results are then dedicated to estimating the crossing probability appearing in  Lemma \ref{L:second_moment_to_crossing_proba}. The first result has a very similar flavour as \cite[Proposition 4.1]{JLQ23a}. On the other hand, the second result is novel and crucially relies on Theorem \ref{T:ratio_general}.


\begin{lemma}\label{L:crossing_upper}
For any $\eta >0$, there exists $C>0$ such that for all $\gamma \in (0,1]$ and $x, y \in D$,
\begin{equation}
\label{E:P_crossing_bound}
\frac{1}{Z_\gamma^2} \Prob{ x \overset{\Lc_D^\theta \cup \Xi_a^x \cup \Xi_a^y}{\longleftrightarrow} y } \leq C |\log |x-y||^{2(1-\theta) + \eta}.
\end{equation}
\end{lemma}

\begin{proposition}\label{P:crossing}
For any distinct points $x, y \in D$, the limit
\begin{equation}
\label{E:P_crossing_limit}
C_\theta(x,y) := \lim_{\gamma \to 0}
\frac{1}{Z_\gamma^2} \P \Big( x \overset{\Lc_D^\theta \cup \Xi_a^x \cup \Xi_a^y}{\longleftrightarrow} y \Big)
\end{equation}
exists and
\begin{equation}
\label{E:P_crossing_limit2}
C_\theta(x,y) \leq \liminf_{\gamma_1, \gamma_2 \to 0}
\frac{1}{Z_{\gamma_1} Z_{\gamma_2}} \P \Big( x \overset{\Lc_D^\theta \cup \Xi_{a_1}^x \cup \Xi_{a_2}^y}{\longleftrightarrow} y \Big).
\end{equation}
Moreover,
\begin{equation}
C_\theta(x,y) = \left( \log \frac{1}{|x-y|} \right)^{2(1-\theta)+o(1)}
\quad \quad \text{as} \quad x-y \to 0.
\end{equation}
More generally, let $\eps >0$ and $F: \mathfrak{L} \to \R$ be a bounded measurable function that does not depend on loops with diameter smaller than $\eps>0$. Then the following two limits exist and are identical
\begin{equation}
\label{E:P_law}
\lim_{r \to 0}
\frac{1}{Z_r^2}
\Expect{ F(\Lc_D^\theta) \mathbf{1}\Big\{ D(x,r) \overset{\Lc_D^\theta}{\longleftrightarrow} D(y,r) \Big\} }
=
\lim_{a \to 0}
\frac{1}{Z_\gamma^2}
\Expect{ F(\Lc_D^\theta) \mathbf{1}\Big\{x \overset{\Lc_D^\theta \cup \Xi_{a}^x \cup \Xi_{a}^y}{\longleftrightarrow} y \Big\} }.
\end{equation}
\end{proposition}

We can now show Theorems \ref{T:convergenceL2}, \ref{T:cluster2point} and \ref{T:cluster_xy_doob}.

\begin{proof}[Proof of Theorem \ref{T:cluster2point}]
It follows directly from \eqref{E:P_law}. Indeed,
let $x, y \in D$ be two distinct points.
By a density-type argument, to prove Theorem \ref{T:cluster2point}, it is enough to show that for any $\eps >0$ and any bounded measurable function $F: \mathfrak{L} \to \R$ which does not depend on loops with diameter smaller than $\eps$,
$
\EXPECT{x \leftrightarrow y,r}{F(\Lc_\D^\theta)}
$
converges as $r \to 0$. This is a mere restatement of the convergence \eqref{E:P_law}.
\end{proof}

\begin{proof}[Proof of Theorem \ref{T:convergenceL2}]
Let $f:D \to \R$ be a bounded measurable function. By decomposing $f$ into its positive and negative parts, we can assume without loss of generality that $f$ is nonnegative. We want to show that $((h_\gamma,f), \gamma \in (0,\sqrt{2})$ is Cauchy in $L^2$, i.e. that
$
\Expect{ | (h_{\gamma_1},f) - (h_{\gamma_2},f) |^2 } \to 0
$
as $\gamma_1, \gamma_2 \to 0$.
By Lemma \ref{L:second_moment_to_crossing_proba}, this second moment is equal to
\[
o(1) + \int_{D \times D} f(x) f(y) \Bigg( \frac{\P \Big( x \overset{\Lc_D^\theta \cup \Xi_{a_1}^x \cup \Xi_{a_1}^y}{\longleftrightarrow} y \Big)}{Z_{\gamma_1}^2} + \frac{\P \Big( x \overset{\Lc_D^\theta \cup \Xi_{a_2}^x \cup \Xi_{a_2}^y}{\longleftrightarrow} y \Big)}{Z_{\gamma_2}^2} - 2 \frac{\P \Big( x \overset{\Lc_D^\theta \cup \Xi_{a_1}^x \cup \Xi_{a_2}^y}{\longleftrightarrow} y \Big)}{Z_{\gamma_1} Z_{\gamma_2}} \Bigg).
\]
Proposition \ref{P:crossing} together with dominated convergence theorem (and Fatou's lemma for the crossed term involving both $a_1$ and $a_2$) then shows that
$
\limsup_{\gamma_1, \gamma_2 \to 0} \Expect{ | (h_{\gamma_1},f) - (h_{\gamma_2},f) |^2 } \leq 0
$.
This concludes the $L^2$ convergence of $(h_\gamma,f)$.

We now explain how one can lift this convergence to a convergence in the Sobolev space $H^{-\eps}(\C)$, where $\eps \in (0,1)$ is arbitrary small. Recall that $H^{-\eps}(\C)$ is the set of tempered distribution $f$ such that
\begin{equation}
\label{E:Sobolev}
\norme{f}_{H^{-\eps}(\C)}^2 := \int_\C (1+|\xi|^2)^{-\eps} |\hat{f}(\xi)|^2 \d \xi < \infty.
\end{equation}
Let $\gamma_1, \gamma_2 \in (0,\sqrt{2})$. Denoting $C_{\gamma_1,\gamma_2}(x,y) = \Expect{ (h_{\gamma_1}(x) - h_{\gamma_2}(x))(h_{\gamma_1}(y) - h_{\gamma_2}(y)) }$, we have
\begin{align}
\label{E:Sobolev2}
\E \norme{h_{\gamma_1}-h_{\gamma_2}}_{H^{-\eps}(\C)}^2 & = \int_{\R^2} \frac{\E \abs{\hat{h}_{\gamma_1}(\xi) - \hat{h}_{\gamma_2}(\xi)}^2}{(1+\abs{\xi}^2)^\eps} \d \xi
\leq \int_{\R^2} \frac{\E \abs{\hat{h}_{\gamma_1}(\xi) - \hat{h}_{\gamma_2}(\xi)}^2}{\abs{\xi}^{2\eps}} \d \xi \\
& = \int_{D \times D} \d x \d y ~C_{\gamma_1,\gamma_2}(x,y) \int \d \xi ~\frac{e^{2\pi i \xi \cdot (x-y)}}{\abs{\xi}^{2\eps}}
= C_\eps \int_{D \times D} \d x \d y ~\frac{C_{\gamma_1,\gamma_2}(x,y)}{|x-y|^{2-2\eps}}
\nonumber
\end{align}
where we used the fact that the Fourier transform of $|\cdot|^{-2\eps}$ is $C_\eps |\cdot|^{-2+2\eps}$ for some constant $C_\eps$ depending on $\eps$.
We can then conclude as before using Proposition \ref{P:crossing} that $h_\gamma$ is Cauchy in $L^2(H^{-\eps}(\C), \P)$.

Finally, the fact that $Z_\gamma = \gamma^{2(1-\theta)+o(1)}$ was proved in Section \ref{SS:thick_loop}.
\end{proof}

\begin{proof}[Proof of Theorem \ref{T:cluster_xy_doob}]
By a simple density-type argument, it is enough to check the identity statement in Theorem \ref{T:cluster_xy_doob} for a function $F: \mathfrak{L} \to \R$ depending only on loops with diameter larger than a given threshold. For such functions, it then follows from Lemma \ref{L:second_moment_to_crossing_proba}, Theorem \ref{T:cluster2point} and \eqref{E:P_law}.
\end{proof}


\subsection{Proof of Lemma \ref{L:second_moment_to_crossing_proba}}


\begin{proof}[Proof of Lemma \ref{L:second_moment_to_crossing_proba}]
By definition of $h_\gamma$, the left hand side of \eqref{E:L_second_moment_to_crossing_proba} is equal to
\begin{align*}
\frac{1}{Z_\gamma Z_{\gamma'}} \int_{D \times D}
\Expect{ F(x,y,\Lc_D^\theta) (\Mc_a^+(\d x) \Mc_{a'}^+(\d y) - \Mc_a^+(\d x) \d y - \d x \Mc_{a'}^+(\d y) + \d x \d y) }.
\end{align*}
By \eqref{E:first_moment_measure},
\[
\Expect{ F(x,y,\Lc_D^\theta) \Mc_a^+(\d x)} = \Expect{F(x,y,\Lc_D^\theta \cup \{\Xi_{a_i}^x \}_{i \geq 1})} \d x
\]
where the loops $\{\Xi_{a_i}^x \}_{i \geq 1}$ are as defined above Lemma \ref{L:moment_measure}. A similar result holds at $y$.
To handle the term $\Expect{ F(x,y,\Lc_D^\theta) (\Mc_a^+(\d x) \Mc_{a'}^+(\d y)}$, we first control the contribution of soups containing at least one loop which visits both $x$ and $y$. By triangle inequality and then by
\eqref{E:second_moment_measure1} and \eqref{E:second_moment_measure2} applied to $F \equiv 1$, we have
\begin{align*}
& \abs{ \Expect{F(x,y,\Lc_D^\theta) \Mc_a^+(\d x) \Mc_{a'}^+(\d y) \indic{\exists \wp \in \Lc_D^\theta: x,y \in \wp}} }
\leq \norme{F}_\infty \Expect{ \Mc_a(\d x) \Mc_{a'}(\d y) \indic{\exists \wp \in \Lc_D^\theta: x,y \in \wp}} \\
& = 4 \norme{F}_\infty \left( \left( 2 \pi \sqrt{aa'} G_D(x,y) \right)^{1-\theta} \Gamma(\theta) I_{\theta-1} \left(4\pi \sqrt{aa'} G_D(x,y) \right) - 1 \right) \d x \d y
= O(\gamma^2 {\gamma'}^2).
\end{align*}
On the other hand, by the Girsanov-type transform \eqref{E:second_moment_measure2}, the contribution with no such loop is equal to
\begin{align*}
& \Expect{F(x,y,\Lc_D^\theta) \Mc_a^+(\d x) \Mc_a^+(\d y) \indic{\nexists \wp \in \Lc_D^\theta: x,y \in \wp}} \\
& = 4 \E \Big[ F(x,y,\Lc_D^\theta \cup \{\Xi_{a_i}^x \}_{i \geq 1} \cup \{\Xi_{a_i'}^y \}_{i \geq 1}) \mathbf{1} \{ \Cf^+ (\Lc_D^\theta \cup \{\Xi_{a_i}^x \}_{i \geq 1} \cup \{\Xi_{a_i'}^y \}_{i \geq 1}) \} \Big] \d x \d y.
\end{align*}
We then notice that, conditionally on $\Lc_D^\theta \cup \{\Xi_{a_i}^x \}_{i \geq 1} \cup \{\Xi_{a_i'}^y \}_{i \geq 1}$, the probability that both $x$ and $y$ belong to positive clusters of $\Lc_D^\theta \cup \{\Xi_{a_i}^x \}_{i \geq 1} \cup \{\Xi_{a_i'}^y \}_{i \geq 1}$ is equal to
\begin{align*}
\frac14 \Big(1- \mathbf{1} \Big\{ x \overset{\Lc_D^\theta \cup \{\Xi_{a_i}^x \}_{i \geq 1} \cup \{\Xi_{a_i'}^y \}_{i \geq 1}}{\longleftrightarrow} y \Big\} \Big) + \frac12 \mathbf{1} \Big\{ x \overset{\Lc_D^\theta \cup \{\Xi_{a_i}^x \}_{i \geq 1} \cup \{\Xi_{a_i'}^y \}_{i \geq 1}}{\longleftrightarrow} y \Big\}
= \frac{1}{4} + \frac{1}{4} \mathbf{1} \Big\{ x \overset{\Lc_D^\theta \cup \{\Xi_{a_i}^x \}_{i \geq 1} \cup \{\Xi_{a_i'}^y \}_{i \geq 1}}{\longleftrightarrow} y \Big\}.
\end{align*}
Putting everything together, we have obtained that the left hand side of \eqref{E:L_second_moment_to_crossing_proba} is equal to
\begin{align*}
& \frac{1}{Z_\gamma Z_{\gamma'}} \int_{D \times D} \Expect{ F(x,y,\Lc_D^\theta \cup \{\Xi_{a_i}^x \}_{i \geq 1} \cup \{\Xi_{a_i'}^y \}_{i \geq 1}) \mathbf{1} \Big\{ x \overset{\Lc_D^\theta \cup \{\Xi_{a_i}^x \}_{i \geq 1} \cup \{\Xi_{a_i'}^y \}_{i \geq 1}}{\longleftrightarrow} y \Big\} } \d x \d y + O(1) \frac{\gamma^2 {\gamma'}^2}{Z_\gamma Z_{\gamma'}} \\
& + \frac{1}{Z_\gamma Z_{\gamma'}} \int_{D \times D} \E [ F(x,y,\Lc_D^\theta \cup \{\Xi_{a_i}^x \}_{i \geq 1} \cup \{\Xi_{a_i'}^y \}_{i \geq 1}) - F(x,y,\Lc_D^\theta \cup \{\Xi_{a_i}^x \}_{i \geq 1}) \\
& ~~~~~~~~~~~~~~~~~~~~~~~~~~ - F(x,y,\Lc_D^\theta \cup \{\Xi_{a_i'}^y \}_{i \geq 1}) + F(x,y,\Lc_D^\theta) ] \d x \d y.
\end{align*}
To bound the last integral above, we need to recall that $F$ does not depend on loops with diameter smaller than a given threshold $\eps$. Hence, if $\wedge_{i \geq 1} \Xi_{a_i}^x$ or $\wedge_{i \geq 1} \Xi_{a_i'}^y$ has diameter smaller than $\eps$, then
\[
F(x,y,\Lc_D^\theta \cup \{\Xi_{a_i}^x \}_{i \geq 1} \cup \{\Xi_{a_i'}^y \}_{i \geq 1}) - F(x,y,\Lc_D^\theta \cup \{\Xi_{a_i}^x \}_{i \geq 1}) - F(x,y,\Lc_D^\theta \cup \{\Xi_{a_i'}^y \}_{i \geq 1}) + F(x,y,\Lc_D^\theta) = 0.
\]
The probability that both $\wedge_{i \geq 1} \Xi_{a_i}^x$ and $\wedge_{i \geq 1} \Xi_{a_i'}^y$ have diameter at least $\eps$ is of order $\gamma^2 {\gamma'}^2$ (Lemma \ref{L:diameter_thick}) concluding the proof.
\end{proof}


\subsection{Proof of Lemma \ref{L:crossing_upper} and Proposition \ref{P:crossing}}

We start by proving Lemma \ref{L:crossing_upper}.

\begin{proof}
Let $\eta >0$ be small and $x,y \in D$. If $|x-y| \leq e^{-a^{-1+\eta}}$, we simply bound the probability in  \eqref{E:P_crossing_bound} by 1 and using that $Z_\gamma = \gamma^{2(1-\theta)+o(1)} = a^{1-\theta + o(1)}$, we obtain that the left hand side of \eqref{E:P_crossing_bound} is at most
\[
a^{-2(1-\theta) + o(1)} \leq C |\log |x-y||^{2(1-\theta)/(1-2\eta)}.
\]
We therefore only need to consider the case where $x$ and $y$ are not too close to each other, i.e. $|x-y| \geq e^{-a^{-1+\eta}}$. 
For $z \in \{x,y\}$, we will denote by $D_z = D(z, |x-y|/2)$.
By Lemma \ref{L:diameter_thick}, the minimal disc centred at $x$ containing $\Xi_a^x$ has typically a radius of order $e^{- O(1) /a}$. It is therefore very unlikely that $\Xi_a^x$ exits $D_x$. We are first going to show that this is still the case conditionally on the existence of a cluster joining $x$ and $y$:
\begin{equation}
\label{E:exitDx}
\frac{1}{Z_\gamma^2} \Prob{ x \overset{\Lc_D^\theta \cup \Xi_a^x \cup \Xi_a^y}{\longleftrightarrow} y, \exists z \in \{x,y\}: \Xi_a^z \not\subset D_z } \to 0 
\quad \quad \text{as~} \gamma \to 0
\end{equation}
and also that the left hand side can be bounded by $C |\log |x-y||^{\frac{2(1-\theta)}{1-2\eta}}$, uniformly in $\gamma$.
With some abuse of notation, we will view $\Xi_a^x$ both as the collection of excursions in a Poisson point process with intensity $a \mu_D^{x,x}$ and as the loop formed by the concatenation of all these excursions. 
Let $E_x^1$ (resp. $E_x^2$) be the event that there is a unique excursion (resp. at least two distinct excursions) of $\Xi_a^x$ that exits $D_x$.
By Lemma \ref{L:diameter_thick},
$
\mu_D^{z,z}( \{ \wp \not\subset D_x \} ) = \log \frac{2 \CR(x,D)}{|x-y|}.
$
So
\[
\Prob{E_x^2} \leq
\E \Big[ \sum_{\wp \neq \wp' \in \Xi_a^x} \indic{\wp \not\subset D_x, \wp' \not\subset D_x } \Big]
= a^2 \mu_D^{z,z}( \{ \wp \not\subset D_x \} )^2 \leq C a^2 |\log |x-y||^2.
\]
In that case, we simply bound
\[
\frac{1}{Z_\gamma^2} \Prob{ x \overset{\Lc_D^\theta \cup \Xi_a^x \cup \Xi_a^y}{\longleftrightarrow} y, E_x^2 }
\leq a^{-2(1-\theta)+o(1)} \Prob{E_x^2} \leq C a^{2\theta+o(1)} |\log |x-y||^2
\leq C |\log |x-y||^{\frac{2(1-\theta)}{1-2\eta}}.
\]
The probability of the event $E_x^1$ is at most $C a |\log |x-y||$. On that event, let $r_x$ be the minimal distance between $y$ and the unique excursion of $\Xi_a^x$ that exists $D_x$. Let also $r_y$ be the maximal $r>0$ such that there exists a cluster of loops of $\Lc_D^\theta \cup \Xi_a^y$ that connect $y$ to $\partial D(y,r)$.
On the event $E_1^x$, in order to have a cluster joining $x$ and $y$, we need to have $r_x \leq r_y$.
For all $k \geq 0$, the probability that $r_x$ is smaller than $e^{-k} |x-y|/2$ can be compared with the probability that a Brownian path starting on the circle $\partial D_x$ hits $D(y,e^{-k} |x-y|/2)$ before exiting the domain $D$. Hence for all $k \geq 0$,
\[
\Prob{ r_x \leq e^{-k} \frac{|x-y|}{2} \Big\vert E_x^1} \leq C \frac{|\log|x-y||}{|\log|x-y|| + k}.
\]
On the other hand, using that
\[
Z_\gamma \geq c \Prob{ y \overset{\Lc_D^\theta \cup \Xi_a^y}{\longleftrightarrow} \partial D(y,e^{-1}) }
\]
and using FKG inequality, we have
\begin{align*}
\frac{1}{Z_\gamma} \Prob{ r_y \geq e^{-k} \frac{|x-y|}{2} }
& \leq C \Prob{ y \overset{\Lc_D^\theta \cup \Xi_a^y}{\longleftrightarrow} \partial D(y,e^{-1}) \vert y \overset{\Lc_D^\theta \cup \Xi_a^y}{\longleftrightarrow} \partial D(y,e^{-k} \frac{|x-y|}{2}) }^{-1} \\
& \leq C \Prob{ \partial D(y,e^{-k} \frac{|x-y|}{2}) \overset{\Lc_D^\theta}{\longleftrightarrow} \partial D(y,e^{-1}) }^{-1} \leq C (|\log |x-y|| + k)^{1-\theta+\eta}.
\end{align*}
Hence, 
\begin{align*}
\frac{1}{Z_\gamma^2} \Prob{ x \overset{\Lc_D^\theta \cup \Xi_a^x \cup \Xi_a^y}{\longleftrightarrow} y, E_x^1 }
\leq C \frac{a}{Z_\gamma^2} \sum_{k \geq 0} \Prob{ r_x \leq e^{-k} \frac{|x-y|}{2} \Big\vert E_1^x } \Prob{ \frac{2r_y}{|x-y|} \in [e^{-k-1},e^{-k})} \\
\leq C \frac{a}{Z_\gamma^2} \sum_{k \geq 0} \frac{|\log|x-y||}{|\log|x-y|| + k} \Prob{ \frac{2r_y}{|x-y|} \in [e^{-k-1},e^{-k})}.
\end{align*}
We perform a discrete integration by parts, ``differentiating'' $\frac{|\log|x-y||}{|\log|x-y|| + k}$:
\[
\frac{|\log|x-y||}{|\log|x-y|| + k-1} - \frac{|\log|x-y||}{|\log|x-y|| + k} \leq C \frac{|\log|x-y||}{(|\log|x-y|| + k)^2}.
\]
This leads to 
\begin{align*}
\frac{1}{Z_\gamma^2} \Prob{ x \overset{\Lc_D^\theta \cup \Xi_a^x \cup \Xi_a^y}{\longleftrightarrow} y, E_x^1 }
& \leq C \frac{a}{Z_\gamma^2} \sum_{k \geq 0} \frac{|\log|x-y||}{(|\log|x-y|| + k)^2} 
\Prob{ \frac{2r_y}{|x-y|} \geq e^{-k} } \\
& \leq C \frac{a}{Z_\gamma} \sum_{k \geq 0} \frac{|\log|x-y||}{(|\log|x-y|| + k)^{1+\theta-\eta}} 
\leq C a^{\theta+o(1)} |\log |x-y||^{1-\theta+\eta}.
\end{align*}
This concludes the proof of \eqref{E:exitDx}.

We can now work on the event $\Xi_a^z \subset D_z$ for $z=x,y$.
Let $\Lc_{D,x,y}^\theta$ be the subset of $\Lc_D^\theta$ consisting of the loops that are not included in $D_x \cup D_y$. Let
\[
r_z = \inf\{ r>0: \exists \wp \in \Lc_{D,x,y}^\theta: \wp \cap D(z,r) \neq \varnothing \},
\quad \quad z=x,y.
\]
By the restriction property of $\Xi_a^x$ (see Lemma \ref{L:restriction_thick_loop}),
\begin{align*}
& \frac{1}{Z_\gamma^2} \Prob{ x \overset{\Lc_D^\theta \cup \Xi_a^x \cup \Xi_a^y}{\longleftrightarrow} y, \forall z=x,y, \Xi_a^z \subset D_z}
\leq \frac{1}{Z_\gamma^2} \Prob{ \forall z=x,y, z \overset{\Lc_D^\theta \cup \Xi_a^z}{\longleftrightarrow} \partial D(z,r_z), \Xi_a^z \subset D_z } \\
& = \frac{1}{Z_\gamma^2} \frac{\CR(x,D_x)^a \CR(y,D_y)^a}{\CR(x,D)^a \CR(y,D)^a} \Prob{ \forall z=x,y, z \overset{\Lc_D^\theta \cup \Xi_a^{z,D_z}}{\longleftrightarrow} \partial D(z,r_z)}.
\end{align*}
In what follows, we will simply bound the ratio of conformal radii by 1 (which is also a good approximation since $a \to 0$).
Now by scale invariance of $\Lc_D^\theta$ and $\Xi_a^z$,
\begin{align*}
& Z_\gamma \Big/ \Prob{ z \overset{\Lc_{D_z}^\theta \cup \Xi_a^{z,D_z}}{\longleftrightarrow} \partial D(z,r_z) \Big\vert r_z }
= Z_\gamma \Big/ \Prob{ 0 \overset{\Lc_{\D}^\theta \cup \Xi_a^{0,\D}}{\longleftrightarrow} \frac{2r_z}{|x-y|} \partial \D \Big\vert r_z } \\
& = \Prob{ 0 \overset{\Lc_{\D}^\theta \cup \Xi_a^{0,\D}}{\longleftrightarrow} e^{-1} \partial \D \Big\vert r_z, 0 \overset{\Lc_{\D}^\theta \cup \Xi_a^{0,\D}}{\longleftrightarrow} \frac{2r_z}{|x-y|} \partial \D }.
\end{align*}
Conditionally on the origin being linked to $\frac{2r_z}{|x-y|} \partial \D$, the origin will be linked to $e^{-1} \partial \D$ provided the following events hold:
\begin{itemize}
\item
There is a cluster of $\Lc_\D^\theta$ crossing $e^{-1} \D \setminus \frac{r_z}{|x-y|} \D$;
\item
There is a loop in $\Lc_\D^\theta$ surrounding $\frac{r_z}{|x-y|} \D$ while staying in $\frac{2r_z}{|x-y|} \D$.
\end{itemize}
By FKG inequality, the conditional probability of the intersection of these two events is at least the product of the two unconditioned probabilities. The probability of the first event is at least $\left( \log \frac{|x-y|}{2r_z} \right)^{-1+\theta-\eta}$ by Theorem \ref{T:large_crossing}. By Lemma \ref{L:surround}, the probability of the second event is at least some constant showing that
\[
Z_\gamma \Big/ \Prob{ z \overset{\Lc_{D_z}^\theta \cup \Xi_a^{z,D_z}}{\longleftrightarrow} \partial D(z,r_z) \Big\vert r_z } \geq c \left( \log \frac{|x-y|}{2r_z} \right)^{-1+\theta-\eta}.
\]
Wrapping things up,
\begin{align*}
\frac{1}{Z_\gamma^2} \Prob{ x \overset{\Lc_D^\theta \cup \Xi_a^x \cup \Xi_a^y}{\longleftrightarrow} y, \forall z=x,y, \Xi_a^z \subset D_z}
\leq C \Expect{ \prod_{z=x,y} \left( \log \frac{|x-y|}{2r_z} \right)^{1-\theta+\eta} }.
\end{align*}
In \cite{JLQ23a}, we show that the above quantity is upper bounded by $C|\log |x-y||^{2(1-\theta)+2\eta}$ (see (4.16) in Remark 4.5 therein) concluding the proof of Lemma \ref{L:crossing_upper}.
%We also show in that paper that for $A>0$ large,
%\[
%\Expect{ \prod_{z=x,y} \left( \log \frac{|x-y|}{2r_z} \right)^{1-\theta+\eta} \indic{\exists z \in \{x,y\}, r_z \geq A|\log |x-y||} } \leq o(1) |\log |x-y||^{2(1-\theta)+2\eta}
%\]
%where $o(1) \to 0$ as $A \to \infty$, uniformly in $x, y$; see (4.17) in \cite[Remark 4.5]{JLQ23a}.
%In particular, if $x$ and $y$ are at a macroscopic distance to each other and if $r_0 >0$ is small, then
%\begin{equation}
%\label{E:proof_P_crossing3}
%\frac{1}{Z_\gamma^2} \Prob{ x \overset{\Lc_D^\theta \cup \Xi_a^x \cup \Xi_a^y}{\longleftrightarrow} y, \forall z = x,y, \Xi_a^z \subset D_z, \min(r_x,r_y) \leq r_0 } \leq o_{r_0 \to 0}(1)
%\end{equation}
%where $o_{r_0 \to 0}(1)$ goes to zero as $r_0 \to 0$ and does not depend on $\gamma$. This estimate will be needed in the proof Proposition \ref{P:crossing}.
\end{proof}



We can now prove Proposition \ref{P:crossing}.

\begin{proof}[Proof of Proposition \ref{P:crossing}]
Let $x$ and $y$ be two distinct points in $D$. Compare to the upper bound, the two points $x$ and $y$ are fixed and we wish to take the limit as $\gamma_1, \gamma_2 \to 0$. It is therefore important for the proof to keep in mind that $x$ and $y$ are at macroscopic distance to each other and that we can assume $\gamma_1$ and $\gamma_2$ to be as small as desired. We start by proving \eqref{E:P_crossing_limit}. We will explain at the end of the proof what needs to be changed in order to get \eqref{E:P_crossing_limit2} and \eqref{E:P_law}.

Let $\eta >0$ be small and let $D_x = D(x,\eta|x-y|/2)$ and $D_y = D(y,\eta|x-y|/2)$. By taking $\eta >0$ small enough, we can ensure that $D_x$ and $D_y$ are subsets of $D$. We will denote $\Lc_{D,x,y}^\theta = \Lc_D^\theta \setminus (\Lc_{D_x}^\theta \cup \Lc_{D_y}^\theta)$ the collection of loops which are not included in $D_x$ or $D_y$.
We now introduce the following events:
\begin{itemize}
\item $E_1$: there is a loop in $\Lc_{D,x,y}^\theta$ that disconnects $D_x$ from $D_y$;
\item $E_2$: for $z = x,y$, $\Xi_a^z \subset D_z$.
%\item $E_3$: $\Lc_{D,x,y}^\theta$ does not intersect $D(x,r_0) \cup D(y, r_0)$.
\end{itemize}
We first claim that we can work on $E_1 \cap E_2$. Indeed, by Lemma \ref{L:surround} $\Prob{E_1^c} \to 0$ as $\eta \to 0$ and, by FKG inequality,
\[
\limsup_{\gamma \to 0} \frac{1}{Z_{\gamma}^2}
\Prob{ x \overset{\Lc_D^\theta \cup \Xi_{a}^x \cup \Xi_{a}^y}{\longleftrightarrow} y, E_1^c } \to 0 \quad \quad \text{as} \quad \eta \to 0.
\]
Moreover, in the proof of the upper bound, we showed that
\[
\lim_{\gamma \to 0} \frac{1}{Z_{\gamma}^2}
\Prob{ x \overset{\Lc_D^\theta \cup \Xi_{a}^x \cup \Xi_{a}^y}{\longleftrightarrow} y, E_2^c } = 0.
\]
%and that
%\[
%\limsup_{\gamma \to 0} \frac{1}{Z_{\gamma}^2}
%\Prob{ x \overset{\Lc_D^\theta \cup \Xi_{a}^x \cup \Xi_{a}^y}{\longleftrightarrow} y, E_2, E_3^c } \to 0 \quad \quad \text{as} \quad r_0 \to 0.
%\]
See \eqref{E:exitDx}.
% and \eqref{E:proof_P_crossing3} respectively.
We can therefore work on the event $E_1 \cap E_2$. On the event $E_1$, there is at most one cluster $\Cc_{x,y}$ of loops in $\Lc_{D,x,y}^\theta$ that intersects both $D_x$ and $D_y$ (we set $\Cc_{x,y} = \varnothing$ if there is no such cluster).
By the restriction property \eqref{E:restriction_thick_loop} of $\Xi_a^z$, we have
\begin{align*}
& \Prob{ x \overset{\Lc_D^\theta \cup \Xi_a^x \cup \Xi_a^y}{\longleftrightarrow} y, E_1\cap E_2}
 = \frac{\CR(x,D_x)^a \CR(y,D_y)^a}{\CR(x,D)^a \CR(y,D)^a} \Expect{ \mathbf{1}_{E_1} \prod_{z=x,y} \Prob{z \overset{\Lc_{D_z}^\theta \cup \Xi_a^{z,D_z}}{\longleftrightarrow} \Cc_{x,y} \Big\vert \Cc_{x,y} }  }.
\end{align*}
The ratio of conformal radii converges to 1. Moreover, for $z = x$ or $y$, we can rewrite
\[
\frac{1}{Z_\gamma}
\P \Big( z \overset{\Lc_{D_z}^\theta \cup \Xi_a^{z,D_z}}{\longleftrightarrow} \Cc_{x,y} \vert \Cc_{x,y} \Big)
=
\P \Big( z \overset{\Lc_{D_z}^\theta \cup \Xi_a^{z,D_z}}{\longleftrightarrow} \Cc_{x,y} \vert \Cc_{x,y} \Big)
\Big/ \P \Big( z \overset{\Lc_{D_z}^\theta \cup \Xi_a^{z,D_z}}{\longleftrightarrow} \partial D(z, e^{-1}\eta |x-y|/2) \Big)
\]
and we can replace
% For $z = x$ or $y$, and on the event $E_3$, we can rewrite
%\begin{align*}
%\frac{1}{Z_\gamma}
%\P \Big( z \overset{\Lc_{D_z}^\theta \cup \Xi_a^{z,D_z}}{\longleftrightarrow} \Cc_{x,y} \vert \Cc_{x,y} \Big)
%& = \P \Big( z \overset{\Lc_{D_z}^\theta \cup \Xi_a^{z,D_z}}{\longleftrightarrow} \Cc_{x,y} \Big\vert \Cc_{x,y}, z \overset{\Lc_{D_z}^\theta \cup \Xi_a^{z,D_z}}{\longleftrightarrow} \partial D(z,r_0) \Big) \\
%& \times \P \Big( z \overset{\Lc_{D_z}^\theta \cup \Xi_a^{z,D_z}}{\longleftrightarrow} \partial D(z,r_0) \Big\vert z \overset{\Lc_{D_z}^\theta \cup \Xi_a^{z,D_z}}{\longleftrightarrow} \partial D(z,|x-y|/4) \Big).
%\end{align*}
%In the first probability on the right hand side, we can replace
$\Cc_{x,y}$ by the closure of $(\Cc_{x,y} \cap D_z) \cup \partial D_z$ which is a.s. a connected compact subset of $\overline{D_z} \setminus \{z\}$. We are now in the setting of Theorem \ref{T:ratio_general} which shows that the above ratio converges as $a \to 0$, a.s. with respect to $\Cc_{x,y}$.
The upper bound \eqref{E:P_crossing_bound} provides the bound necessary to apply dominated convergence in order to exchange the expectation w.r.t. $\Cc_{x,y}$ and the limit. We have proved that
\begin{equation}
\label{E:proof_P_crossing4}
\lim_{\gamma \to 0} \frac{1}{Z_\gamma^2} \Prob{ x \overset{\Lc_D^\theta \cup \Xi_a^x \cup \Xi_a^y}{\longleftrightarrow} y, E_1 \cap E_2}
\end{equation}
exists and that
$
\frac{1}{Z_\gamma^2} \P \Big( x \overset{\Lc_D^\theta \cup \Xi_a^x \cup \Xi_a^y}{\longleftrightarrow} y \Big)
$
converges as $\gamma \to 0$ towards the nondecreasing limit of \eqref{E:proof_P_crossing4} as $\eta \to 0$. This shows \eqref{E:P_crossing_limit}.

The proof of \eqref{E:P_crossing_limit2} concerning the mixed case $(a_1,a_2)$ follows along the same lines. The main difference comes from the fact that we only need a lower bound, so we can add for free the extra events $E_1$ and $E_2$.
The proof of \eqref{E:P_law} is obtained similarly. Indeed, because the function $F$ does not depend on loops that have diameter smaller than a given threshold $\eps$, $F$ does not depend on loops included in $D_x$ and $D_y$ provided $\eta$ is small enough. We then repeat the above procedure and use Theorem \ref{T:ratio_general}.

Finally, the upper bound of \eqref{E:P_crossing_bound} follows from Lemma \ref{L:crossing_upper}. The lower bound is much easier to prove and follows from Theorem \ref{T:large_crossing} and FKG inequality. We omit the details.
\end{proof}

==> subfiles/intro.tex <==
The continuum Gaussian free field (GFF), also known as the Euclidean bosonic free field, is an ubiquitous object both in Quantum Field Theory, where it represents, up to a Wick rotation, a gas of non-interacting bosons, and in Statistical Physics, where it appears in the scaling limit of different discrete models [cite dimers, Ginzburg-Landau, random matrices other]. The 2D GFF in particular is conformally invariant and logarithmically correlated. Together with its multiplicative chaos, it has been at the heart of some extraordinary developments in the past few years in probability theory, in particular in connection with Liouville quantum gravity *** and the mathematical construction of Liouville conformal field theory ***.
%The ubiquity of the GFF can be explained by the fact that it is the only conformal invariant generalised function satisfying a certain domain Markov property *** (plus some moment condition).

Le Jan \cite{LeJan2010LoopsRenorm, LeJan2011Loops} offered another remarkable perspective on the Gaussian free field by relating it to the local time of the Brownian loop soup. The latter is a random collection of infinitely many Brownian-type loops in a given domain $D$ of the plane, sampled according to a Poisson point process with intensity $\theta \loopmeasure_D$. $\theta >0$ is a positive real parameter and $\loopmeasure_D$ is a measure on loops defined by:
\begin{equation}
\label{Eq loop meas}
\loopmeasure_{D}(d\wp)=
\int_{D}\int_{0}^{+\infty}
\P_{D,t}^{z,z}(d\wp)
p_D(t, z, z)\dfrac{\d t}{t} \d z,
\end{equation}
where $p_D(t, z, z)$ is the heat kernel in $D$ and $\P_{D,t}^{z,z}$ is a Brownian bridge law (see Section \ref{SS:preliminaries_paths} for details).
It has been introduced by Lawler and Werner \cite{Lawler04} and is related to other important objects of 2D random conformal geometry. Le Jan's isomorphism states that when $\theta =1/2$ the (centred) occupation field of the loop soup has the same distribution as half of the (Wick) square of the GFF. This result is part of the random walk/Brownian motion
representations of the GFF, 
also known as \textbf{isomorphism theorems}
\cite{Symanzik65Scalar,Symanzik66Scalar,Symanzik1969QFT,
BFS82Loop,Dynkin1984Isomorphism,
Dynkin1984IsomorphismPresentation,
Wolpert2,
EKMRS2000,
MarcusRosen2006MarkovGaussianLocTime,
Sznitman2012LectureIso}.

Now, the 2D Brownian loop soups are interesting at all intensity parameters,
not just at $\theta=1/2$, and not just because of the relation to the GFF.
Indeed, the Brownian loop soups satisfy a conformal invariance property for all values of $\theta$, and therefore are related to other conformally invariant stochastic processes such as Schramm-Loewner Evolutions (SLE) and Conformal Loop Ensembles (CLE).
In \cite{LSW03Restriction}, 
Lawler, Schramm and Werner show that one can construct the chordal conformal restriction measures with exponent $\alpha>5/8$ by attaching to an 
SLE$_{\kappa}$ path (with $\kappa = \kappa(\alpha)\in (0,8/3)$) the Brownian loops
from an independent Brownian loop soup (with $\theta=\theta(\alpha)>0$) that are intersected by the path
\cite[Theorem 7.3]{LSW03Restriction}.
Further, in their seminal work \cite{SheffieldWernerCLE}, Sheffield and Werner study the clusters of loops (chains of intersecting loops) in Brownian loop soups and show the following phase transition:
\begin{itemize}
\item
Supercritical:
when $\theta>1/2$, there is a.s. only one cluster of loops;
\item
Critical and subcritical:
when $\theta \leq 1/2$, there are a.s. infinitely many clusters. In this case, the outermost boundaries of the outermost clusters are distributed according to a (non-nested) CLE$_\kappa$ where $\kappa = \kappa(\theta) \in (8/3, 4]$.
\end{itemize}
Remarkably, the parameter $\theta=1/2$ appears also in this context of phase transition.

Motivated by this particular case of the GFF and the Brownian loop soup at 
$\theta=1/2$, 
we want to address in this paper the following more general question:
\begin{center}
\emph{What is the natural field associated to the Brownian loop soup when $\theta \neq 1/2$?}
\end{center}
Due to the percolation properties of the loop soup, we will be able to build and study the properties of such a field only when $\theta \leq 1/2$. Surprisingly, the relevant field will not correspond to a signed version of the square root of the local time of the loop soup, as for $\theta = 1/2$, but instead to a signed version of the local time to the power $1-\theta$.

\medskip

Our approach relies on two key inputs, 
\titus{both inspired by the GFF setting ($\theta=1/2$).
The first idea is to give signs to clusters of loops.
This is where the constraint $\theta \leq 1/2$ comes from,
since for $\theta>1/2$ there is a.s. only one cluster.
In \cite{LupuIsomorphism} it is explained how to recover from the loop soup 
(with $\theta =1/2$) not only the square of the GFF but also its signs.
One assigns to each cluster independent spins taking values in $\{\pm 1\}$ with equal probability.
\cite{LupuIsomorphism} shows that, to recover the GFF from this loop soup at 
$\theta=1/2$, one has to take the square root of twice the local time and then multiply this value by the spin of the relevant cluster.
This construction works precisely on the so called \textit{metric graphs},
where the local times of a loop soup are defined pointwise.
To do this in 2D continuum requires a renormalisation procedure.
Indeed, in this setting the local times are not defined pointwise and even diverge everywhere because of the contribution of the multitude of small loops.
So it is not even immediately clear what the square root of the local time means.
Yet, the article \cite{ALS4} gives the precise analogue of this procedure in the 2D continuum.}
See also Section *** for more about this.

The second key input that we use in this paper is the construction in \cite{ABJL21} of a multiplicative chaos associated to the Brownian loop soup with any intensity $\theta >0$.
Gaussian multiplicative chaos (GMC), initially introduced by Kahane \cite{kahane} in the eighties and extensively studied in the past decade \cite{RobertVargas2010, DuplantierSheffield, RhodesVargasGMC, ShamovGMC, BerestyckiGMC}, is a theory that defines and studies properties of random measures informally defined as the exponential of a real parameter $\gamma \in \R$ times a Gaussian logarithmically-correlated field. The two-dimensional GFF is an archetypal example of such a field and its GMC measure is sometimes called Liouville measure. Because log-correlated fields are not defined pointwise but are only generalised functions, making sense of such a measure requires a non trivial work and induces the requirement that $\gamma \in (-2,2)$ in dimension 2 ($\gamma = \pm 2$ is a critical case where a nondegenerate measure can still be made sense of).
GMC appears to be a universal feature of log-correlated fields going beyond the Gaussian setting: \cite{Junnila18} studies fields defined as random Fourier series with i.i.d. coefficients and \cite{jegoBMC, jegoCritical} makes sense of the exponential of the square root of the local time of planar Brownian motion.
The article \cite{ABJL21} provides a third example of a non-Gaussian multiplicative chaos and defines what can be thought of as the exponential of $\gamma$ times the square root of twice the local time of the Brownian loop soup, for any intensity $\theta$. In view of Le Jan's isomorphism, it is natural to expect, and has been proven in \cite{ABJL21}, that when $\theta=1/2$ the resulting measure agrees with an unsigned version of Liouville measure: $e^{\gamma |\text{GFF}|} \d x = e^{\gamma \text{GFF}} \d x+ e^{-\gamma \text{GFF}} \d x$, i.e. a sum of two \emph{correlated} Liouville measures.


Combining these two inputs, our approach consists in considering the multiplicative chaos $\Mc_\gamma$ of the loop soup and restricting it to clusters with a positive spin (the rest of the discussion is restricted to the case $\theta \leq 1/2$). We prove that when $\theta = 1/2$ the resulting measure $\Mc_\gamma^+$ agrees with $e^{\gamma \text{GFF}} \d x$. The GFF can therefore be recovered from the loop soup, together with the independent spins, by differentiating $\Mc_\gamma^+$ at 
$\gamma = 0$.
\titus{This idea is used for instance in \cite{ALS1}.}
When $\theta < 1/2$, we show that the same procedure yields a nondegenerate conformally invariant field with the surprising and important difference that one has to take a \emph{fractional derivative} of $\Mc_\gamma^+$ at $\gamma=0$.

\titus{Part of our motivation for introducing these fields is that they may posses ``level lines'' that could be SLE$_{\kappa}$-type curves with $\theta$ and $\kappa$ related as in Sheffield-Werner \cite{SheffieldWernerCLE},
spanning in this way all the range $(8/3,4]$ for $\kappa$.
This would be analogous to the GFF case ($\theta = 1/2$),
where SLE$_{4}$-type curves appear as level lines of the free field [CITE SCHRAMM-SHEFFIELD] (these are really rather cliffs of constant height between two different values on either side).
Already, \cite{SheffieldWernerCLE} tells us that the (non-nested) 
CLE$_{\kappa(\theta)}$ loops should correspond to interfaces in our fields.
We intend to investigate this hypothetical relation to SLE$_{\kappa}$-type curves
in the future.}


==> subfiles/intro_crossing.tex <==


For us it is particularly important to understand the decay rate of these crossing probabilities since this is what drives the blow-up of the correlations of $h_\theta$. The decay of the normalising constant $Z_\gamma$ in Theorem \ref{T:convergenceL2} is also obtained from the asymptotic behaviour of these crossing probabilities.


\begin{notation}
For any family $\Lc$ of loops and any sets $A, B \subset D$, we will denote by $\{ A \overset{\Lc}{\leftrightarrow} B \}$ the event that there is a cluster of loops in $\Lc$ that intersects both $A$ and $B$. If $x$ and $y$ are points, we will simply write $\{ x \overset{\Lc}{\leftrightarrow} A \}$ and $\{ x \overset{\Lc}{\leftrightarrow} y \}$ instead of $\{ \{x\} \overset{\Lc}{\leftrightarrow} A \}$ and $\{ \{x\} \overset{\Lc}{\leftrightarrow} \{y\} \}$.
\end{notation}


Let $D$ be a bounded simply connected domain and $x \in D$.
In ***, we define an infinite measure on excursions from $x$ to $x$ that stay inside $D$. For $a>0$, we let $\Xi_a^{x,D}$ be the loop which is the concatenation at $x$ of all the excursions in a Poisson point process with intensity $a \mu_D^{x,x}$. The normalising constant $Z_\gamma$ is then defined by
\begin{equation}
\label{E:Zgamma}
Z_\gamma := \Prob{ 0 \overset{\Lc_\D^\theta \wedge \Xi_a^{0,\D}}{\longleftrightarrow} e^{-1} \partial \D }.
\end{equation}
In words, $Z_\gamma$ is the probability that the origin is connected to the circle $e^{-1} \partial \D$ in a soup composed of a loop soup $\Lc_\D^\theta$ with intensity $\theta$ and an $a$-thick loop $\Xi_a^{0,\D}$ at the origin.





\begin{theorem}\label{T:large_crossing}
Let $\theta \in (0,1/2]$.
The probability that a cluster in a Brownian loop soup $\Lc_\D^\theta$ intersects both the microscopic circle $r \partial \D$ and the macroscopic circle $e^{-1} \partial \D$ decays like
\[
\Prob{ r \partial \D \overset{\Lc_\D^\theta}{\longleftrightarrow} e^{-1} \partial \D } = |\log r|^{-1+ \theta +o(1)}
\quad \quad \text{as~} \quad r \to 0.
\]
\end{theorem}



Theorem \ref{T:large_crossing} can be seen as an interpolation of the two known cases $\theta =1/2$ and $\theta \to 0^+$. Indeed, when the intensity $\theta = 1/2$, the connection with the Gaussian free field allows one to show the crossing probability is of order $|\log r|^{-1/2}$.
\red{More details.}
When $\theta \to 0^+$, the crossing probability can be informally compared with the probability that a Brownian path starting somewhere in the unit disc (not at the origin), and killed at the boundary of the unit disc, hits the disc $r \partial \D$. This probability is of order $|\log r|^{-1}$.




==> subfiles/intro_discrete.tex <==
Let $D_N \subset \frac1N \Z^2 \cap D$ be a subset of the square lattice with mesh size $\frac1N$ which approximates the continuous domain $D$. See \eqref{eq:DN} for a precise definition.
Fix $\theta \in (0,1/2]$ and let $\Lc_{D_N}^\theta$ be a random walk loop soup in the metric graph $\widetilde{D}_N$ and $\Cf_N = \{ \Cc \}_{\Cc \in \Cf_N}$ be the collection of clusters $\Cc$ of $\Lc_{D_N}^\theta$. Conditionally on $\Cf_N$, let $\sigma_\Cc$, $\Cc \in \Cf_N$, be i.i.d. spins taking values in $\{\pm 1\}$ with equal probability.
For all $x \in \widetilde{D}_N$, let $\ell_x(\Lc_{D_N}^\theta)$ be the total local time accumulated by all loops at $x$, i.e.
\[
\ell_x(\Lc_{D_N}^\theta)
= \sum_{ \wp \in \Lc_{D_N}^\theta } N^2 \int_0^{T(\wp)} \indic{ \wp(t) = x } \d t.
\]
For orientation, we recall that for all $x$, $\ell_x(\Lc_{D_N}^\theta)$ is distributed according to Gamma$(\theta,G_{D_N}(x,x))$ where $G_{D_N}(x,x)$ is the discrete Green function which behaves, with our normalisation, like $G_{D_N}(x,x) \sim \frac{1}{2\pi} \log N$ as $N \to \infty$.
We can now define what we conjecture being the analogue of $h_\theta$ in the discrete:
\begin{equation}
\label{E:def_htheta_discrete}
h_{\theta,N}(x) := \frac{\Gamma(\theta)}{2^{1-\theta} \Gamma(2-\theta)} \sigma_{\Cc_x} \{ 2\pi \ell_x(\Lc_{D_N}^\theta) \}^{1-\theta},
\end{equation}
where $\Cc_x$ denotes the cluster containing $x$.


\begin{conjecture}\label{Conj:intro}
Let $\theta \in (0,1/2]$. There exists $c_{\mathrm{conj}} = c_{\mathrm{conj}}(\theta) >0$ such that for all bounded smooth test function $f$,
\begin{equation}
\frac{1}{N^2} \sum_{x \in D_N} f(x) h_{\theta,N}(x)
\xrightarrow[N \to \infty]{\mathrm{(d)}} c_{\mathrm{conj}} \int_D f(x) h_\theta(x) \d x.
\end{equation}
\end{conjecture}



In Section \ref{S:2D_Wick}, we considerably elaborate on this conjecture and address the question of defining the renormalised powers of $h_\theta$. The powers of $h_\theta$ that reduce to integer powers $:L_x^n:$ of the local time $:L_x:$ have already been defined by Le Jan \cite{LeJan2011Loops}. In order to define the remaining powers (the ``odd'' powers of $h_\theta$), we give a specific approximation scheme from the discrete and we conjecture that it possesses a nondegenerate scaling limit (Conjecture \ref{Conjecture1}). This is based on a connection with the one-dimensional Brownian loop soup (first revealed in \cite{JLQ23a}) and reveals a surprising notion of duality between the intensities $\theta$ and $\theta^* = 2-\theta$. If this conjecture held true, we would obtain the following expansion for $\Mc_\gamma^+$ around $\gamma =0$:
\[
\Mc_\gamma^+(\d x) = \Big( \sum_{k \geq 0} \frac{\gamma^{2k}}{2^k} \frac{\Gamma(\theta)}{k! \Gamma(k+\theta)} (2\pi)^k :L_x^k:
+ c_\mathrm{conj} \gamma^{2(1-\theta)} \frac{\gamma^{2k}}{2^k} \frac{\Gamma(\theta^*)}{k! \Gamma(k+\theta^*)} (2\pi)^k :h_\theta(x) L_x^k: \Big) \d x.
\]
See Section \ref{S:expansion_signed} for the definition of the different terms appearing in the above display.




==> subfiles/intro_field.tex <==
Let $D \subset \C$ be a bounded simply connected domain and $\theta \in (0,1/2]$. Consider a Brownian loop soup $\Lc_D^\theta$ in $D$ with intensity $\theta$.
Let us denote by $\Cf$ the collection of all clusters $\Cc$ of $\Lc_D^\theta$. Conditionally on $\Cf$, let $(\sigma_\Cc)_{\Cc \in \Cf}$ be i.i.d. signs taking values in $\{ \pm 1 \}$ with equal probability 1/2. If a point $x \in D$ belongs to some cluster $\Cc$, we will write $\sigma_x$ for the sign $\sigma_\Cc$ of that cluster.


Let $\gamma \in (0,2)$ and let $\Mc_\gamma$ be the multiplicative chaos of the Brownian loop soup $\Lc_D^\theta$ constructed in \cite{ABJL21}, normalised so that $\Expect{ \Mc_\gamma(\d x)} = 2\d x$; see Section \ref{S:multiplicative_chaos} for details. Let $\Mc_\gamma^+ (\d x) = \indic{\sigma_x = +1} \Mc_\gamma (\d x)$ be the multiplicative chaos of $\Lc_D^\theta$ restricted to positive clusters. Note that this definition is meaningful since every $\Mc_\gamma$--typical point is visited by a loop (actually by infinitely many loops, see \cite[Theorem 1.8]{ABJL21}).
Let $h_\gamma$ be the field obtained from $\Mc_\gamma^+$ by
\begin{equation}
(h_\gamma,f) := \frac{1}{Z_\gamma} \int_D f(x) (\Mc_\gamma^+(\d x) - \d x),
\end{equation}
for any bounded measurable function $f: \C \to \R$. Here $Z_\gamma$ is a normalising constant defined in \eqref{E:Zgamma} below in terms of some crossing probability.
With some abuse of notation, we will often write $(h_\gamma,f) = \int h_\gamma(x) f(x) \d x$. Note that $h_\gamma$ is defined as a random generalised function on the whole complex plane, vanishing outside of $D$.


To define the normalising constants we will use in this article, we first introduce the following notations:

\begin{notation}
For any family $\Lc$ of loops and any sets $A, B \subset D$, we will denote by $\{ A \overset{\Lc}{\leftrightarrow} B \}$ the event that there is a cluster of loops in $\Lc$ that intersects both $A$ and $B$. If $x$ and $y$ are points, we will simply write $\{ x \overset{\Lc}{\leftrightarrow} A \}$ and $\{ x \overset{\Lc}{\leftrightarrow} y \}$ instead of $\{ \{x\} \overset{\Lc}{\leftrightarrow} A \}$ and $\{ \{x\} \overset{\Lc}{\leftrightarrow} \{y\} \}$.
\end{notation}

We will then use two normalising constants $Z_r$ and $Z_\gamma$ defined by
\begin{equation}
\label{E:Zgamma}
Z_r := \P \Big( e^{-1} \partial \D \overset{\Lc_\D^\theta}{\longleftrightarrow} r \D \Big)
\quad \quad \text{and} \quad \quad
Z_\gamma := \P \Big( e^{-1} \partial \D \overset{\Lc_\D^\theta \cup \Xi_a^{0,\D}}{\longleftrightarrow} 0 \Big)
\end{equation}
where $\Xi_a^{0,\D}$ is an $a$-thick loop ($a = \gamma^2/2$) at the origin defined in Section \ref{SS:preliminaries_paths} that is independent from $\Lc_\D^\theta$.




\begin{theorem}\label{T:convergenceL2}
Let $\theta \in (0,1/2]$.
For any bounded measurable function $f : \C \to \R$, $(h_\gamma, f)$ converges in $L^2$ as $\gamma \to 0$.
Moreover, for any $\eps >0$, $h_\gamma$ converges in $L^2$ as $\gamma \to 0$ in the Sobolev space $H^{-\eps}(\C)$ \eqref{E:Sobolev} to some random field $h_\theta \in H^{-\eps}(\C)$.

Furthermore, the normalising constant $Z_\gamma$ satisfies $Z_\gamma = \gamma^{2(1-\theta) + o(1)}$.
\end{theorem}


\begin{theorem}[Properties of $h_\theta$]\label{T:prop}
Let $\theta \in (0,1/2]$.
\begin{enumerate}
\item
\label{I:covariance}
Covariance:
There exists a measurable function $C_\theta : D \times D \to [0,\infty]$ such that for all test functions $f$,
\[
\Expect{ (h_\theta,f)^2 } = \int_{D \times D} f(x) C_\theta(x,y) f(y) \d x \d y.
\]
The blow-up of $C_\theta$ on the diagonal is given by
\[
C_\theta(x,y) = | \log |x-y||^{2(1-\theta) + o(1)}
\quad \quad \text{as} \quad x-y \to 0.
\]
\item
\label{I:conformal_invariance}
Conformal invariance: Let $\psi : D \to \titus{\widetilde{D}}$ be a conformal map between two bounded simply connected domains and let $h_{\theta, D}$ and 
$h_{\theta, \titus{\widetilde{D}}}$ denote the fields from Theorem \ref{T:convergenceL2} in the domains $D$ and $\titus{\widetilde{D}}$. 
Then\footnote{Recall that by definition $(h_{\theta, D} \circ \psi^{-1}, \tilde{f}) = (h_{\theta,D}, \tilde{f} \circ \psi^{-1})$ for any test function $\tilde{f}$.}
$h_{\theta, D} \circ \psi^{-1}$ and $h_{\theta, \titus{\widetilde{D}}}$ 
have the same law.
\item
\label{I:symmetry}
Symmetry: Let $h_\theta^-$ denote the field obtained in a similar way as $h_\theta$ with negative clusters instead of positive ones. Then $h_\theta^- = - h_\theta$ a.s. In particular, $h_\theta \overset{\mathrm{(d)}}{=} - h_\theta$.
\item
\label{I:nondegenerate}
Nondegeneracy: Let $f : D \to \R$ be a smooth test function, non identically zero. Then the law of $(h_\theta,f)$ is nonatomic. In particular, $(h_\theta,f) \neq 0$ a.s.
\end{enumerate}
\end{theorem}


As already mentioned, when $\theta = 1/2$, $\Mc_\gamma$ agrees with the hyperbolic cosine $:e^{\gamma h}: \d x$ $+ :e^{-\gamma h}:\d x$ of the GFF $h$ with Dirichlet boundary condition. Here $h$ is normalised so that $\Expect{h(x) h(y)} \sim -\log|x-y|$ as $x-y \to 0$ and $:e^{\pm \gamma h}: \d x$ are GMC measures normalised so that $\Expect{:e^{\pm \gamma h}: \d x} = \d x$. See \cite[Theorem 1.5]{ABJL21}. Because the isomorphism relating the local time to the GFF is much stronger in the discrete, the proof of this result was obtained by first proving a discrete approximation of $\Mc_\gamma$. In Theorem \ref{T:one_cluster}, we show a stronger version of this convergence by showing that the discrete approximation holds cluster by cluster, for any $\theta \in (0,1/2]$. It implies that, when $\theta =1/2$, the measure $\Mc_\gamma^+(\d x) = \indic{\sigma_x = +1} \Mc_\gamma(\d x)$ agrees with $:e^{\gamma h}: \d x$. As a corollary,

\begin{theorem}\label{T:identification_field1/2}
When $\theta = 1/2$, $h_\theta$ has the law of a multiple of the GFF in $D$.
More precisely, there is a (deterministic) constant $c_{1/2}$ and a coupling between a critical loop soup $\Lc_D^{1/2}$ together with i.i.d. spins $(\sigma_\Cc)_{\Cc \in \Cf}$ and a Gaussian free field $h$ in $D$ such that almost surely,
\begin{itemize}
\item
$\Mc_\gamma^+ = :e^{\gamma h}: \d x$ and $\Mc_\gamma = 2:\cosh (\gamma h): \d x$ for all $\gamma \in (0,2)$;
\item
$h_{1/2} = c_{1/2} h$ and $:L: = \frac12 :h^2:$.
\end{itemize}
\end{theorem}

The appearance of the constant $c_{1/2}$ comes from the fact that we do not renormalise $\Mc_{\gamma}^+(\d x) - \d x$ by $\gamma$, but by a normalising constant $Z_\gamma$ that behaves asymptotically like a multiple of $\gamma$ (see \cite[Lemma 2.6]{JLQ23a} for a similar result where the $a$-thick loop is replaced by a small disc).





\begin{remark}
We warn the reader that, when $\theta \neq 1/2$, the field that we build is different from the CLE nesting field built in \cite{miller2015conformal} whose correlation blows up logarithmically on the diagonal; see \cite[Theorem 1.3]{miller2015conformal}.
\end{remark}


==> subfiles/intro_minkowski.tex <==
We now give another description of $h_\theta$, somewhat more geometric. We will show that the field $h_{\theta}$ is a limit of random signed Radon measures supported on the topological closures of clusters of 
$\Lc^{\theta}_{D}$,
and give an expression for these measures.
This description is greatly inspired by \cite{ALS1,ALS4},
where the authors deal with the more tractable case of the free field 
($\theta = 1/2$).


We start by defining a nondegenerate measure supported on the closure of a given cluster of $\Lc_D^\theta$.
Given a closed (fractal) set $A \subset \C$, it is a classical problem (that can be highly non-trivial) to define a nondegenerate measure supported on $A$. One possibility is to try to renormalise the Lebesgue measure of the $r$-neighbourhood of $A$ and take the limit as $r \to 0^+$. More precisely, one seeks an appropriate gauge function $\phi : (0,\infty) \to (0,\infty)$ such that the measure
$
r^{-2} \phi(r) \indic{\mathrm{dist}(x,A)<r} \d x
$
converges weakly as $r \to 0^+$. If such a function can be found, the resulting measure is then called the Minkowski content of $A$ in the gauge $\phi$.
It is a well known fact that the Minkowski content of a single planar Brownian trajectory is well defined and nondegenerate in the gauge $r \mapsto r^2 |\log r|$. In this case, it coincides with the occupation measure of the path.
Because the non-renormalised local time of a given cluster of $\Lc_D^\theta$ (i.e. the sum of the local times of all the trajectories of a given cluster) is infinite, the Brownian gauge function $r \mapsto r^2 |\log r|$ is not appropriate for the clusters of $\Lc_D^\theta$. And indeed, \cite{ALS1} showed that, when $\theta = 1/2$, the Minkowski content of a given cluster of $\Lc_D^\theta$ is well-defined and nondegenerate in the gauge $r \mapsto r^2 |\log r|^{1/2}$.
In Theorem \ref{T:measure_cluster} below, we resolve the analogous problem when $\theta \in (0,1/2)$ by showing that the Minkowski content of a given cluster of $\Lc_D^\theta$ is well-defined and nondegenerate in some non-explicit gauge function $r \mapsto r^2 / Z_r$ that behaves like $r^2 |\log r|^{1-\theta + o(1)}$ as $r \to 0$.

We order the clusters of $\Lc^{\theta}_{D}$ as follows.
Let $(x_{k})_{k\geq 1}$ be a dense sequence in $D$.
We will denote by $\Cc_{k}$ the outermost cluster of $\Lc^{\theta}_{D}$
surrounding $x_{k}$, among the clusters different from
$\Cc_{1},\dots,\Cc_{k-1}$.
By construction, the clusters $(\Cc_{k})_{k\geq 1}$ are two by two distinct.
It is also easy to see that a.s. this is an enumeration of the clusters of
$\Lc^{\theta}_{D}$.
For $k \geq 1$, let $\mu_{k,r}$ and $\mu_{k, \gamma}$ be the random Radon measures defined by
\[
\mu_{k, r}(B) =
\dfrac{1}{Z_{r}} \int_B \indic{\mathrm{dist}(x,\Cc_{k})<r} \,\d x,
\quad
\mu_{k, \gamma}(B) =
\dfrac{1}{Z_{\gamma}}\int_B \indic{\mathrm{dist}(x,\Cc_{k})<1} (1-\mathrm{dist}(x,\Cc_{k})^{\gamma^{2}/2}) \,\d x,
\]
for all Borel set $B \subset D$. 
Recall that the normalising constants $Z_r$ and $Z_\gamma$ are defined in \eqref{E:Zgamma}.

\begin{theorem}\label{T:measure_cluster}
Let $\theta \in (0,1/2]$. For all $k\geq 1$, $\mu_{k,r}$ and $\mu_{k,\gamma}$ converge in probability w.r.t. the topology of weak convergence as $r \to 0$ and $\gamma \to 0$ to the same random Radon measure $\mu_k$. Moreover, $\mu_k$ is a.s. a non-negative finite measure supported on $\overline{\Cc}_{k}$ and $\mu_k(\overline{\Cc}_k) > 0$ a.s.
\end{theorem}

Recall that we denote by $\sigma_{\Cc_k}$ the spin associated to the $k$-th cluster $\Cc_k$.
The field $h_\theta$ is then obtained by:

\begin{theorem}\label{T:h_and_minkowski}
Let $\theta \in (0,1/2]$. For all $\eps >0$ and all bounded measurable function $f: \C \to \R$, the following convergences hold a.s. and in $L^2$:
\[
\sum_{j=1}^k \sigma_{\Cc_j} \mu_j \xrightarrow[k \to \infty]{} h_\theta
\quad \quad \text{and} \quad \quad \sum_{j=1}^k \sigma_{\Cc_j} (\mu_j,f) \xrightarrow[k \to \infty]{} (h_\theta,f)
\]
in the spaces $H^{-\eps}(\C)$ and $\R$ respectively.
\end{theorem}

In other words, the ``restriction of $|h_\theta|$'' to $\Cc_k$ is a well-defined Radon measure that agrees with $\mu_k$.
\titus{Note however that this does not at all mean that the field $h_\theta$ is a signed measure.
Most likely, the associated total variation measures 
\begin{displaymath}
\sum_{j=1}^k \mu_j
\end{displaymath}
diverge, as $k\to +\infty$, in every open subset of $D$;
so the compensations induced by the signs are necessary for the convergence.
This is known to happen for $\theta=1/2$.
}

==> subfiles/law_cluster.tex <==
\antoine{I don't think we need this section  any more.}

Let $x, y \in D$ be two distinct points and $\eps>0$ be smaller than $|x-y|/2$. On the event that there is a cluster intersecting both $D(x,\eps)$ and $D(y,\eps)$, let $\Cc_{x \leftrightarrow y,\eps}$ be any such cluster (with a deterministic rule to choose one if it is not unique; it is unique with probability tending to 1 as $\eps \to 0$). We view $\Cc_{x \leftrightarrow y,\eps}$ as a random element of $\mathfrak{L}$ equipped with the metric \eqref{metric}. Let $\mu_{x \leftrightarrow y,\eps}$ be the law of $\Cc_{x \leftrightarrow y,\eps}$ conditionally on the event that $D(x,\eps)$ and $D(y,\eps)$ are connected by a cluster.

\begin{theorem}
The probability measure $\mu_{x \leftrightarrow y,\eps}$ converges weakly as $\eps \to 0$ to some probability measure $\mu_{x \leftrightarrow y}$.
\end{theorem}

We define the law $\P_{x \leftrightarrow y}$ (with expectation $\E_{x \leftrightarrow y}$) of the loop soup conditioned on having a cluster that visits both $x$ and $y$. First we sample such a cluster $\Cc$ according to $\mu_{x \leftrightarrow y}$. Then, conditionally on $\Cc$, we sample an unconditioned loop soup $\Lc_{D \setminus \Cc}^\theta$ in (each connected component of) $D \setminus \Cc$. That is,
\[
\EXPECT{x \leftrightarrow y}{F(\Lc)} := \int  \Expect{ F( \Lc_{D \setminus \Cc}^\theta \cup \Cc ) } \d \mu_{x \leftrightarrow y}(\Cc).
\]

\subsection{Cluster conditioned to visit a point}

The main goal of this section is to prove Theorem \ref{T:cluster2point}. Its proof relies on a one-point version that we state now.
For $x \in D$, let $\Cc_{x,\eps}$ be the cluster with the largest diameter that intersects $D(x,\eps)$ and let $\mu_{x,\eps}$ be the probability law of $\Cc_{x,\eps}$.
For any $r>0$, let $p(x,\eps, r)$ be the probability that $\Cc_{x,\eps} \cap \partial D(x,r)\not=\emptyset$.

\begin{theorem}\label{thm:cluster_measure}
Let $x \in D$ and $r_0 >0$ be such that $\overline{D}(x,r_0) \subset D$.
The sequence of measures $p(x,\eps, r_0)^{-1} \mu_{x,\eps}$ converges vaguely w.r.t.\ the metric \eqref{metric} to an infinite measure $\mu_x$ supported on clusters that contain $x$ in its closure.
\end{theorem}

The measure $\mu_x$ should be thought of as the (infinite) measure on the cluster in $\Lc_D^\theta$ conditioned to visit $x$. It becomes finite if one restricts it to macroscopic clusters (clusters with a diameter larger than a given threshold for instance). It is supported on  collections of parametrized loops. In defining the metric \eqref{metric}, we have assigned a root to each loop for convenience, but we can also regard the loops as unrooted loops by forgetting their roots.


We start by proving a weaker notion of convergence which follows immediately from Theorem \ref{T:ratio_general}: we will first view a cluster as a random element of $(\Kc,\d_\Kc)$ \eqref{E:Hausdorff_distance}, i.e. as a random compact set (instead of a collection of loops). In this section, we fix a point $x \in D$ and $r_0 >0$ such that $\overline{D}(x,r_0) \subset D$. Because $x$ is fixed, we will omit the dependence in $x$ in our notations. We will need to keep track of the domain $D$ in the proof and will denote by $\Cc_{D,\eps}$ (instead of $\Cc_{x,\eps}$ as above) the cluster with the largest diameter intersecting the disc $D(x,\eps)$. We will also denote by $p(\eps,r)$ the probability that $\Cc_{D,\eps}$ intersects $\partial D(x,r)$.

\begin{lemma}
Let $K_{D,\eps}$ be the closure of $\Cc_{D,\eps}$ and $\nu_{D,\eps}$ be its law. Then $p(\eps, r_0)^{-1} \nu_{D,\eps}$ converges vaguely in the space $(\mathcal{K}, \d_\Kc)$ to an infinite distribution $\nu_{D}$.
\end{lemma}

\begin{proof}
Let $r \in (0,r_0)$. We claim that following weak convergence of probability measures in $(\Kc, \d_\Kc)$ holds:
\[
p(\eps, r)^{-1} \one_{K \cap \partial D(x,r)\not=\emptyset} \d\nu_{D,\eps}(K) \underset{\eps\to 0}{\longrightarrow} \Qb_r.
\]
Indeed, this follows from the convergence of the probabilities
\[
\Prob{ K_{D,\eps} \cap A \cap \partial D(x,r) \neq \varnothing \vert K_{D,\eps} \cap \partial D(x,r) \neq \varnothing }, \quad \quad A \in \Kc, \quad \quad \text{as} \quad \eps \to 0.
\]
See e.g. \cite[Theorem 6.5]{molchanov2005theory} (since $\overline D$ is compact, the Fell topology on closed subsets of $\overline{D}$ agrees with the Hausdorff topology on compact subsets of $\overline{D}$, see \cite[Appendix C]{molchanov2005theory}).


Because for $r\in(0,r_0)$,
\begin{align}\label{eq:pp}
p(\eps, r)^{-1} p(\eps, r_0)= p(\eps, r)^{-1} \nu_{D,\eps} (K \cap \partial D(x,r_0)\not=\emptyset ) \underset{\eps\to 0}{\longrightarrow} \Qb_r (K \cap  \partial D(x,r_0)\not=\emptyset) =: c(r),
\end{align}
we have that for $r\in (0,r_0)$,
\begin{align*}
p(\eps, r_0)^{-1} \one_{K \cap \partial D(x,r)\not=\emptyset} \d\nu_{D,\eps}(K)
\underset{\eps\to 0}{\longrightarrow} c(r)^{-1} \Qb_r.
\end{align*}
Since the measure $p(\eps, r_0)^{-1} \d\nu_{D,\eps}(K)$ restricted to the event $\{K \cap \partial D(x,r)\not=\emptyset\}$ converges for all $r\in(0,r_0)$, and the event $\{K \cap \partial D(x,r)\not=\emptyset\}$ increases to the whole space as $r\to 0$, we deduce that $p(\eps, r_0)^{-1} \nu_{D,\eps}$ converges to some limiting measure $\nu_{D}$.
\end{proof}

Let $A\subset \overline D$ be a closed set which does not contain $x$. Let $\Lc_{D\setminus A}$ denote the set of loops in $\Lc_D^\theta$ that stay in $D\setminus A$, and let $\Lc^A$ denote the set of loops in $\Lc_D^\theta$ that touch $A$. 
Let $\Cc_{D\setminus A,\eps}$ be the  the cluster in $\Lc_{D\setminus A}$ with the largest diameter that intersects $D(x,\eps)$, and let $K_{D\setminus A,\eps}$ be its closure. Let us consider the probability measure $\Pb_\eps$ on the triple $(K, L, M)$ defined as follows:
\begin{itemize}
\item $K$ is a random set distributed as $K_{D\setminus A,\eps}$
\item $L$ is a set of loops distributed as $\Lc_{D\setminus A} \setminus \Cc_{D\setminus A,\eps}$
\item $M$ is a set of loops distributed as $\Lc^A$.
\end{itemize}
The triple  $(K, L, M)$ lives in the product of three spaces, where the first space is endowed with the Hausdorff metric and the other two spaces are endowed with the metric \eqref{metric}.

\begin{lemma}\label{lem:conv}
The measures $p(\eps, r_0)^{-1} \Pb_\eps$ converge vaguely as $\eps\to 0$ to a limiting measure $\sigma_A$. If $(K, L, M)$ is distributed according to $\sigma_A$, then
\begin{enumerate}
\item there exists a constant $c_A$ such that $K$ is distributed according to $c(A) \nu_{D\setminus A}$;
\item given $K$, the set $L$ is distributed as an independent loop soup in $D \setminus (A \cup K)$;
\item $M$ is distributed as an independent loop soup in $D$ restricted to the loops that intersect $A$.
\end{enumerate}
\end{lemma}

Note that the laws of $L$ and $M$ given $K$ are probability laws, while the marginal distribution on $K$ carries infinite total mass.

\begin{proof}
Let $p_{D\setminus A} (\eps, r_0)$ be the probability that $K_{D\setminus A,\eps}$ intersects $D(x,r_0)$. In order to prove the lemma, it suffices to prove that there exists $c_A>0$ such that
\begin{align}\label{eq:ratio}
p_{D\setminus A} (\eps, r_0)/p_D(\eps,r_0)  \to  c_A \text{ as } \eps\to 0.
\end{align}
Let $(K_\eps, L_\eps, M_\eps)$ be a triple under the law $\Pb_\eps$, then the marginal distribution of $M_\eps$ does not depend on $\eps$, and is equal to an independent loop soup in $D$ restricted to the loops that intersect $A$. We therefore drop the subscript and denote $M=M_\eps$.
Let $\wt A$ be the union of $D\setminus D(x,r_0)$ and $M$. Then
$
p_D(\eps, r_0) = \nu_{D\setminus A,\eps} (K \cap \wt A \not=\emptyset).
$
For $r\in(0,r_0)$, similarly to \eqref{eq:pp}, we have 
$$\nu_{D\setminus A,\eps} (K \cap \wt A \not=\emptyset)/ p_{D\setminus A} (\eps, r)\to c(r, \wt A, D\setminus A).$$
For similar reasons, $p_{D\setminus A} (\eps, r_0)/p_{D\setminus A} (\eps, r)$ also converges to some constant $c$ as $\eps\to 0$. Combined, we have proved \eqref{eq:ratio}.

Given $K_\eps$, the set $L_\eps$ is distributed as an independent loop soup in  $D \setminus (A \cup K_\eps)$. Therefore, the conditional law of $L_\eps$ given $K_\eps$ converges to that of an independent loop soup in $D\setminus (A\cup K)$. We have already argued that the law of $M_\eps$ does not depend on $\eps$. This completes the proof of the lemma.
\end{proof}


We are now ready to prove Theorem~\ref{thm:cluster_measure}.

\begin{proof}[Proof of Theorem~\ref{thm:cluster_measure}]
Suppose that $(K, L, M)$ is distributed according to $\sigma_A$. Let $\psi_A(K, L, M)$ be the set of loops in $M$ which belong to the clusters in $L\cup M$ that intersect $K$. Let $\mu_{D, A}$ be the distribution of $\psi_A(K, L, M)$, restricted to the event that $\psi_A(K, L, M)\not=\emptyset$. 
Let $\Cc_{D,\eps}(A)$ be the set of loops in $\Cc_{D,\eps}$ that intersect $A$. Let $\mu_{D, A,\eps}$ be the law of $\Cc_{D,\eps}(A)$ restricted on the event that $\Cc_{D,\eps} \cap A\not=\emptyset$. Let us prove the following vague convergence
\begin{align}\label{eq:cvg_measure}
p(\eps, r_0)^{-1} \mu_{D, A,\eps} \to \mu_{D, A}.
\end{align}
Let $E_\eps$ be the event that among the clusters formed by the loops in $\Cc_{D,\eps}$ that stay in $D\setminus A$, the one with the largest diameter which intersects $D(x,\eps)$ is equal to $\Cc_{D\setminus A,\eps}$.
Let $F_\eps$ be the event that there exists a cluster in $\Lc$ that intersects both $D(x,\eps)$ and $A$.
We need to prove that
\begin{align}\label{eq:decay}
\nu_{D,\eps} (E_\eps^c \cap F_\eps) / p(\eps, r_0) \to 0.
\end{align}
On the event $E_\eps^c \cap F_\eps$, the cluster in $\Lc$ which intersects both $D(x,\eps)$ and $A$ must not encircle $D(x,\eps)$. This means that the outer boundary of this cluster (which is a CLE loop) goes through $D(x,\eps)$, which is an event  with probability $\eps$ to some power. This probability decays much faster than $p(\eps,r_0)$, hence we have proved \eqref{eq:decay}.

On the event $E_\eps \cap F_\eps$, $\Cc_{D,\eps}(A)$ is non empty and is equal to $\psi_A(K_\eps, L_\eps, M_\eps)$, where $(K_\eps, L_\eps, M_\eps)$ is distributed according to $\Pb_\eps$.
Let $\wt\mu_{D, A,\eps}$ be the law of $\psi_A(K_\eps, L_\eps, M_\eps)$ restricted to the event $\psi_A(K_\eps, L_\eps, M_\eps)\not=\emptyset$.
 By Lemma~\ref{lem:conv}, we know that $p(\eps, r_0)^{-1}\wt\mu_{D, A,\eps}\to \mu_{D,A}$ as $\eps\to 0$.
 Noting \eqref{eq:decay} and that $\{\psi_A(K_\eps, L_\eps, M_\eps)\not=\emptyset\} \subset F_\eps$, we have
 \begin{align*}
p(\eps, r_0)^{-1}\wt\mu_{D, A,\eps} \one_{E_\eps \cap F_\eps}\to \mu_{D,A} \text{ as } \eps\to 0.
\end{align*}
Noting that $\wt\mu_{D, A,\eps} \one_{E_\eps \cap F_\eps}=\mu_{D, A,\eps} \one_{E_\eps \cap F_\eps}$, we have
 \begin{align*}
p(\eps, r_0)^{-1}\mu_{D, A,\eps} \one_{E_\eps \cap F_\eps}\to \mu_{D,A} \text{ as } \eps\to 0.
\end{align*}
By \eqref{eq:decay}, we further have
$$
p(\eps, r_0)^{-1}\mu_{D, A,\eps}\one_{F_\eps} \to \mu_{D,A} \text{ as } \eps\to 0.
$$
Noting that $\{\Cc_{D,\eps}(A)\not=\emptyset\} \subset F_\eps$, we have $p(\eps, r_0)^{-1}\mu_{D, A,\eps}\one_{F_\eps}= p(\eps, r_0)^{-1}\mu_{D, A,\eps}$, hence we get \eqref{eq:cvg_measure}.

We point out that the distributions $\mu_{D, A}$ for different $A$ are compatible : If $A_1\subseteq A_2$,  and $N_2$ is distributed under $\mu_{D,A_2}$, then the set $N_1$ of loops in $N_2$ that intersect $A_1$ (restricted to the event that $N_1\not=\emptyset$) is distributed according to $\mu_{D, A_1}$. Indeed, we can naturally couple two triples $(K^1_\eps, L^1_\eps, M^1_\eps)$ and $(K^2_\eps, L^2_\eps, M^2_\eps)$ distributed respectively according to $\Pb_{\eps, A_1}$ and $\Pb_{\eps, A_2}$ in a way that the set of loops in $\psi_{A_2} (K^2_\eps, L^2_\eps, M^2_\eps)$ that intersect $A_1$ is equal to $\psi_{A_1} (K^1_\eps, L^1_\eps, M^1_\eps)$. This coupling is realized by defining these sets out of the same loop soup $\Lc$.
Taking the $\eps\to 0$ limit proves the compatibility of the distributions $\mu_{D, A}$ for different $A$.

Let $A_\delta:=D\setminus B(0,\delta)$. Let $\mu_D$ be the limit of $\mu_{D,A_\delta}$ as $\delta$ tends to $0$. Since the measures $\mu_{D, A}$ for different $A$ are compatible, $\mu_D$ is well defined. 
Moreover, if $\Cc$ is a set distributed according to $\mu_D$, then the set of loops in $\Cc$ that intersect $A_\delta$ (restricted to the event that this set is non empty) is distributed according to $\mu_{D, A_\delta}$.
This completes the proof of Theorem~\ref{thm:cluster_measure}.
\end{proof}

We finish this section with:

\begin{proof}[Proof of Theorem \ref{T:cluster2point}]
Using a similar procedure as in the proof of Proposition \ref{P:crossing}, one can obtain the convergence of $\mu_{x \leftrightarrow y, \eps}$ from Theorem \ref{thm:cluster_measure}. We omit the details.
\end{proof}


==> subfiles/minkowski.tex <==
This section is devoted to the proofs of Theorems \ref{T:measure_cluster} and \ref{T:h_and_minkowski}. We start by proving Theorem \ref{T:measure_cluster}. Recall the notations introduced above Theorem \ref{T:measure_cluster}.

\begin{proof}[Proof of Theorem \ref{T:measure_cluster}]
Let $k \geq 1$.
Let $B \subset D$ be some Borel set. It is enough to show that $(\mu_{k,r}(B))_{r >0}$ and $(\mu_{k,\gamma}(B))_{\gamma >0}$ are Cauchy in $L^2$ and that $\mu_{k,r}(B) - \mu_{k,\gamma}(B)$ converges to 0 in $L^2$ as $\gamma, r \to 0$. We already have all the ingredients to prove this. Indeed,
\begin{align*}
& \limsup_{r,r' \to 0}
\Expect{ (\mu_{k,r}(B) - \mu_{k,r'}(B))^2 }
= \limsup_{r,r' \to 0} \frac{1}{Z_r Z_{r'}} \int_{B \times B} \Big( \Prob{ \Cc_k \cap D(x,r) \neq \varnothing, \Cc_k \cap D(y,r) \neq \varnothing } \\
&~~~ + \Prob{ \Cc_k \cap D(x,r') \neq \varnothing, \Cc_k \cap D(y,r') \neq \varnothing } - 2 \Prob{ \Cc_k \cap D(x,r) \neq \varnothing, \Cc_k \cap D(y,r') \neq \varnothing }\Big) \d x \d y.
\end{align*}
The analogue of Lemma \ref{L:crossing_upper} with small discs instead of thick loops (and Fatou's lemma to deal with the mixed term $r$-$r'$) provides the necessary domination to exchange limit and integral. To show that the integrand converges pointwise to zero, we then use the same approach as in the proof of Proposition \ref{P:crossing}. Eventually, the proof of Theorem \ref{T:measure_cluster} boils down to Theorem \ref{T:ratio_general}. We omit the details.

The above line of argument also shows that the second moment of $\mu_k(D)$ is positive. In particular, the probability that $\mu_k(D)>0$ is positive. We are going to show that this probability is actually equal to 1.
Without loss of generality assume that $D = [0,1]^2$. 
Let $\wp$ be some fixed macroscopic loop of $\Lc_D^\theta$, e.g. the loop with the largest diameter. Let $n \geq 1$ be a large integer and divide $D$ into disjoint squares $Q_i$, $i = 1, \dots, 4^n$, of side length $2^{-n}$. For each $i=1, \dots, 4^n$, let $\Lc_i$ be the set of loops included in $Q_i$. Conditionally on $\{ \text{diam}(\wp) > \sqrt{2} 2^{-n} \}$, the collections $\Lc_i$, $i=1, \dots, 4^n$, are independent from $\wp$ and independent loop soups in $D_i$.
For $i=1, \dots, 4^n$, let $Q_i'$ be the square with side length $2^{-n-1}$ with the same centre as $Q_i$ and let $E_i$ be the event that there is a cluster $\Cc_i$ of $\Lc_i$ with non-zero Minkowski content and such that $\Cc_i$ disconnects $Q_i'$ from $\partial Q_i$. By scale invariance, $p = \P(E_i)$ is positive and independent of $n$ and $i$.
Let $I = \{ i=1, \dots, 4^n: \wp \cap Q_i' \neq \varnothing \}$. On the event $E_i \cap \{i \in I\}$, the cluster of $\wp$ contains $\Cc_i$. Hence, the probability that the Minkowski content of the cluster of $\wp$ vanishes is at most
\[
\Prob{ \text{diam}(\wp) \leq \sqrt{2} 2^{-n} } + \Expect{(1-p)^{\# I} }
\xrightarrow[n \to \infty]{} 0.
\]
This concludes the proof.
\end{proof}

The main item that remains to be checked is that, as stated in Theorem \ref{T:h_and_minkowski}, $\mu_k$ corresponds to the restriction of $|h_\theta|$ to $\Cc_k$. The rest of this section is dedicated to this.

As usually, we will denote by $\overline{\Cc}_{k}$ the topological closure of
$\Cc_{k}$, seen as a compact subset of $D$.
We will denote
\begin{displaymath}
D_{k} = D\setminus\bigcup_{1\leq j\leq k}\overline{\Cc}_{j}.
\end{displaymath}
Then $D_{k}$ is an open subset of $D$ that has infinitely many connected components,
among which finitely many (at most $k$) are multiply connected and the rest are simply connected, the total number of holes being $k$.
We will denote by
\begin{displaymath}
\Lc^{\theta}_{D,k} = \{\wp\in \Lc^{\theta}_{D}: \wp \subset D_{k}\}.
\end{displaymath}
We will denote by $\sigma_{k}$ the sign $\sigma_{\Cc_{k}}$ of the cluster
$\Cc_{k}$.
We will denote by $\Fc_{k}$ the $\sigma$-algebra generated by the loops contained in
$\Cc_{1},\dots,\Cc_{k}$ (including their time parametrization)
and the signs $\sigma_{1},\dots, \sigma_{k}$.

\begin{lemma}
\label{Lem cond loop soup D k}
Fix $k\geq 1$.
Let $O_{i}$, $i\geq 0$ be the connected components of $D_{k}$.
Conditionally on $\Fc_{k}$, we have:
\begin{itemize}
\item
The collections of loops $\{ \wp \in \Lc_D^\theta: \wp \subset O_i \}, i \geq 0$, are independent;
\item
For all $i \geq 0$ such that $O_{i}$ is simply connected, 
$\{ \wp \in \Lc_D^\theta: \wp \subset O_i \}$ has the law of a Brownian loop soup in $O_i$ with intensity $\theta$;
\item
For all $i \geq 0$ such that $O_{i}$ is not simply connected, 
$\{ \wp \in \Lc_D^\theta: \wp \subset O_i \}$ has the law of a Brownian loop soup in $O_i$ with intensity $\theta$ conditioned on not having clusters surrounding an inner hole of $O_i$.
\end{itemize}
\end{lemma}

\begin{proof}
\titus{Titus: This is very similar to Lemma \ref{L:condition_cluster} and the two could perhaps be somehow merged.}
\end{proof}

In particular, the collection of loops $\Lc^{\theta}_{D,k}$ is a Brownian loop soup in
$D_{k}$ conditioned on an event that has a positive probability.
So for $\gamma\in (0,2)$, one can define a multiplicative chaos measure associated to
$\Lc^{\theta}_{D,k}$. 
The fact that $D_k$ is not simply connected is non essential: see Remark \ref{rmk:multiplicative_chaos}.
The multiplicative chaos measure associated to $\Lc^{\theta}_{D,k}$
is nothing else than
\begin{displaymath}
\indic{x\in D_{k}}e^{\gamma^{2}\pi(G_{D}(x,x)-G_{D_{k}}(x,x))}\Mc_\gamma(dx),
\end{displaymath}
where $G_{D}$ is the Dirichlet Green's function on $D$ 
and $G_{D_{k}}$ is the Dirichlet Green's function on $D_{k}$.
Note that $G_{D}(x,x)-G_{D_{k}}(x,x)<+\infty$.
We get a density and not just a restriction to $D_{k}$ because our convention
$\E[\Mc_\gamma(dx)] = 2 dx$ makes the normalization for the multiplicative chaos domain-dependent: how we normalize around a point $x$ depends also on the global shape of the domain and not just the Brownian loops we see around $x$. With the normalisation used in \cite{ABJL21}, we would not get this extra density: see \eqref{E:difference_normalisation} for the relation between these two normalisations.
One can further consider the measure $\Mc_\gamma^{+}\mathbf{1}_{D_{k}}$
and the field
\begin{displaymath}
h_{\theta, k}
= \lim_{\gamma\to 0^{+}}
\dfrac{1}{Z_{\gamma}}\indic{x\in D_{k}}(e^{\gamma^{2}\pi(G_{D}(x,x)-G_{D_{k}}(x,x))}
\Mc_\gamma^{+}(dx) - dx),
\end{displaymath}
which is a well defined random element of $H^{-\varepsilon}(\C)$
for $\varepsilon>0$ (simply by working in the domain $D_k$).

Further, one can consider the conditional expectation
$\mathbb{E}[h_{\theta}\vert \Fc_{k}]$.
Since $\mathbb{E}[\Vert h_{\theta}\Vert^{2}_{H^{-\varepsilon}(\C)}] <+\infty$
for $\varepsilon>0$,
the conditional expectation $\mathbb{E}[h_{\theta}\vert \Fc_{k}]$
is a well defined random element of $H^{-\varepsilon}(\C)$,
with
\begin{displaymath}
\Vert \mathbb{E}[h_{\theta}\vert \Fc_{k}]\Vert^{2}_{H^{-\varepsilon}(\C)}
\leq 
\mathbb{E}[\Vert h_{\theta}\Vert^{2}_{H^{-\varepsilon}(\C)}\vert \Fc_{k}]
< +\infty ~~\text{a.s.}
\end{displaymath}
See \cite[Section 2.6]{hytonen2016analysis} for a reference on conditional expectation of random variables in a Banach space.
We define $\nu_{1} = \sigma_{1}\mathbb{E}[h_{\theta}\vert \Fc_{1}]$,
and for $k\geq 2$,
\begin{displaymath}
\nu_{k} = \sigma_{k}(\mathbb{E}[h_{\theta}\vert \Fc_{k}]
-\mathbb{E}[h_{\theta}\vert \Fc_{k-1}]),
\quad \quad \text{so~that} \quad \quad
\mathbb{E}[h_{\theta}\vert \Fc_{k}] = 
\sum_{j=1}^{k}\sigma_{j}\nu_{j}.
\end{displaymath}


\begin{lemma}
The following holds.
\begin{enumerate}
\item For every $k\geq 1$,
conditionally on $\Fc_{k}$, $h_{\theta,k}$ has the same law as $-h_{\theta,k}$,
and in particular
$\mathbb{E}[h_{\theta, k}\vert \Fc_{k}] = 0$.
\item A.s., for every $k\geq 1$
and every $f\in\Cc^{\infty}_{c}(\C)$, such that
$\operatorname{Supp}(f)\cap (D\setminus D_{k}) = \emptyset$,
$(h_{\theta},f) = (h_{\theta,k},f)$.
\item For every $k\geq 1$, 
$h_{\theta} = \mathbb{E}[h_{\theta}\vert \Fc_{k}] + h_{\theta, k}$ a.s.
\item For every $\varepsilon>0$, as $k\to +\infty$,
$\Vert h_{\theta}-\mathbb{E}[h_{\theta}\vert \Fc_{k}]\Vert_{H^{-\varepsilon}(\C)}
\to 0$ a.s. and in $L^2$.
%\begin{displaymath}
%\lim_{k\to +\infty}
%\mathbb{E}[\Vert h_{\theta}-\mathbb{E}[h_{\theta}\vert \Fc_{k}]
%\Vert^{2}_{H^{-\varepsilon}(\C)}] = 0.
%\end{displaymath}
\item For every $k\geq 2$,
$h_{\theta, k-1} = \sigma_{k}\nu_{k} + h_{\theta, k}$ a.s. and
\begin{displaymath}
\nu_{k} = \sigma_{k}\mathbb{E}[h_{\theta, k-1}\vert \Fc_{k}]~~\text{a.s.}
\end{displaymath}
\item $\nu_{1}$ and $\sigma_{1}$ are independent,
and for every $k\geq 2$,
$\nu_{k}$ and $\sigma_{k}$ are independent conditionally on $\Fc_{k-1}$.
\item A.s., for every $k\geq 1$
and every $f\in\Cc^{\infty}_{c}(\C)$ such that
$\operatorname{Supp}(f)\cap \overline{\Cc}_{k} = \emptyset$,
$(\nu_{k},f) = 0$,
that is to say $\nu_{k}$ is supported on $\overline{\Cc}_{k}$.
\end{enumerate}
\end{lemma}

\begin{proof}
1. The proof is the same as for $h_{\theta}$ (see Section \ref{SS:properties_field}).

2. Let $k\geq 1$ and $n\geq 1$. 
Let $\C_{k,n}$ be the open subset of $\C$
formed by points $x\in \C$ such that
$d(x,D\setminus D_{k})>1/n$.
By construction, for every $f\in\Cc^{\infty}_{c}(\C_{k,n})$,
\begin{displaymath}
(h_{\theta},f) = 
\lim_{\gamma\to 0^{+}}
\dfrac{1}{Z_{\gamma}}\int_{D_{k}}f(x)(\Mc_\gamma^{+}(dx) - dx),
\end{displaymath}
where the convergence holds in $L^2$ for a given Sobolev norm
$H^{-\varepsilon}(\C)$
(and thus for all test functions simultaneously).
Further, since $G_{D}(x,x)-G_{D_{k}}(x,x)$ is bounded on $\C_{k,n}$,
the convergence and the limit do no change if we replace $\Mc_\gamma^{+}$
by
\begin{displaymath}
e^{\gamma^{2}\pi(G_{D}(x,x)-G_{D_{k}}(x,x))}
\Mc_\gamma^{+}(dx).
\end{displaymath}

\medskip

3. \titus{Titus: Please, check if the proof of 3. is correct and convincing.} By 1., we only need to show that $h_{\theta} - h_{\theta,k}$ is
measurable w.r.t. $\Fc_{k}$.
Actually will see that $h_{\theta} - h_{\theta,k}$ is
measurable w.r.t. the $\sigma$-algebra $\Fc_{k}$ augmented by the negligible events (i.e. with probability $0$),
which also implies the desired result.

Consider the sets $\C_{k,n}$ defined above. 
Let $\Fc_{k,n}$ be the $\sigma$-algebra generated by $\Fc_{k}$
as well as by the those loops of $\Lc^{\theta}_{D,k}$ that are in clusters at distance at most $1/n$ from $D\setminus D_{k}$, and the signs of these clusters.
By definition, $\Fc_{k}\subset \Fc_{k,n}$ and $\Fc_{k,n+1}\subset \Fc_{k,n}$.
Denote	
\begin{displaymath}
\Fc_{k,\infty} = \bigcap_{n\geq 1}\Fc_{k,n}.
\end{displaymath}
We have $\Fc_{k}\subset \Fc_{k,\infty}$.

For $k\geq 1$ and $n\geq 1$, let $\chi_{k,n}$ be a cutoff function
such that $\chi_{k,n}\in\Cc^{\infty}(\C)$, $\chi_{k,n}$ takes values in $[0,1]$,
$\chi_{k,n}$ equals $0$ on $\C_{k,n}$ and $1$ on $\C\setminus \C_{k,n+1}$.
We also want $\chi_{k,n}$ to be, as a random variable, measurable w.r.t.
$D_{k}$.
We omit the detailed construction of such a cutoff function, which is standard.
Fix $k\geq 1$ and $n\geq 1$. For $m\geq 1$ we have
$h_{\theta} = h_{\theta}\chi_{k,m}+h_{\theta}(1-\chi_{k,m})$,
and by 2., $h_{\theta}(1-\chi_{k,m}) = h_{\theta,k}(1-\chi_{k,m})$.
Moreover, for $m\geq n$, $h_{\theta}\chi_{k,m}$
is measurable w.r.t. $\Fc_{k,n}$.
Further, for $\varepsilon>0$,
\begin{displaymath}
\lim_{m\to +\infty}
\mathbb{E}[\Vert h_{\theta,k}\chi_{k,m}\Vert_{H^{-\varepsilon}(\C)}^{2}
\vert \Fc_{k}] = 0 ~~ \text{a.s.}
\end{displaymath}
by a computation similar to \eqref{E:Sobolev2}.
Therefore,
\begin{displaymath}
\lim_{m\to +\infty}
\mathbb{E}[\Vert(h_{\theta} - h_{\theta,k})- h_{\theta}\chi_{k,m}
\Vert_{H^{-\varepsilon}(\C)}^{2} \vert \Fc_{k}] = 0 ~~ \text{a.s.}
\end{displaymath}
So in particular, $h_{\theta} - h_{\theta,k}$ is the limit in
probability of $h_{\theta}\chi_{k,m}$ as $m\to +\infty$.
Therefore, $h_{\theta} - h_{\theta,k}$ is measurable w.r.t. $\Fc_{k,n}$.
By letting $n\to +\infty$, we get that
$h_{\theta} - h_{\theta,k}$ is measurable w.r.t. $\Fc_{k,\infty}$.

To conclude, it is enough to check that the $\sigma$-algebra $\Fc_{k,\infty}$
is the same as $\Fc_{k}$ up to negligible events.
This is what is sketched below, by omitting some details.
\begin{itemize}
\item Step 1: Let $\Fc'_{k,n}$ be the $\sigma$-algebra generated by $\Fc_{k}$
as well as by the those loops of $\Lc^{\theta}_{D,k}$ that are in clusters at distance at most $1/n$ from $D\setminus D_{k}$.
Contrary to $\Fc_{k,n}$, $\Fc'_{k,n}$ does not contain any information on the
sign of clusters of $\Lc^{\theta}_{D,k}$. Denote
\begin{displaymath}
\Fc'_{k,\infty} = \bigcap_{n\geq 1}\Fc'_{k,n}.
\end{displaymath}
By construction, $\Fc_{k}\subset \Fc'_{k,\infty}\subset \Fc_{k,\infty}$.
We further claim that $\Fc_{k,\infty}$ is the same as
$\Fc'_{k,\infty}$ up to negligible events.
Indeed, the signs of clusters are sampled independently
of the loops in $\Lc^{\theta}_{D,k}$ and are i.i.d.
Moreover, as $n$ increases, $\Fc_{k,n}$ contains information about less clusters and their signs, and in particular, $\Fc_{k,\infty}$ contains
information only on the tail of the sequence of signs.
So essentially this follows from the $0-1$ law of the tails of sequences of 
independent r.v.s.
\item Step 2: Let $\Fc''_{k,n}$ be the $\sigma$-algebra generated by $\Fc_{k}$
as well as by the loops of $\Lc^{\theta}_{D,k}$ that are at distance at most $1/n$ from $D\setminus D_{k}$.
So contrary to $\Fc'_{k,n}$, we look only at individual loops and do not consider how they are grouped into clusters.
By construction, $\Fc''_{k,n}\subset \Fc'_{k,n}$.
Denote
\begin{displaymath}
\Fc''_{k,\infty} = \bigcap_{n\geq 1}\Fc''_{k,n}.
\end{displaymath}
We claim that $\Fc'_{k,\infty}$ is the same as
$\Fc''_{k,\infty}$ up to negligible events. 
For $m>n\geq 1$, let $A_{k,m,n}$ be the event that all the clusters of
$\Lc^{\theta}_{D,k}$ that are at distance at most $1/m$ from $D\setminus D_{k}$,
are actually made of loops that stay in the $1/n$-neighborhood of
$D\setminus D_{k}$.
Then $A_{k,m,n}\in \Fc''_{k,n}$ and for every $A\in \Fc'_{k,m}$,
we have $A\cap A_{k,m,n}\in \Fc''_{k,n}$. Moreover,
\begin{displaymath}
\lim_{m\to +\infty}\mathbb{P}(A_{k,m,n}^{\rm c}) = 0.
\end{displaymath}
Thus, $\Fc'_{k,\infty}$ is contained in $\Fc''_{k,n}$ augmented by the negligible
events, whatever the value of $n$.
\item Step 3: We have that $\Fc_{k}\subset \Fc''_{k,\infty}$.
We claim that $\Fc''_{k,\infty}$ is the same as $\Fc_{k}$ up to negligible events.
If the conditional distribution of $\Lc^{\theta}_{D,k}$ given $\Fc_{k}$
were exactly Poisson, this would have been immediate by $0-1$ law.
However, by Lemma \ref{Lem cond loop soup D k},
this conditional distribution is Poisson conditioned on an event with positive probability, so the $0-1$ law still holds.
\end{itemize}

\medskip

4. This is simply due to the fact that the $\sigma$-algebra
$\vee_{k\geq 1}\Fc_{k}$ generated by the union of the $\Fc_{k}$
is the total $\sigma$-algebra generated by the loop soup
$\Lc^{\theta}_{D}$ and the signs clusters.

5. Since
\begin{displaymath}
\mathbb{E}[h_{\theta}\vert \Fc_{k-1}] + h_{\theta, k-1}
=\mathbb{E}[h_{\theta}\vert \Fc_{k-1}] + \sigma_{k}\nu_{k} + h_{\theta, k}
= h_{\theta},
\end{displaymath}
we get that $\sigma_{k}\nu_{k} = h_{\theta, k-1}-h_{\theta, k}$.
Since $\sigma_{k}\nu_{k}$ is $\Fc_{k}$-measurable
and $\mathbb{E}[h_{\theta, k}\vert \Fc_{k}] = 0$,
we conclude by taking the conditional expectation w.r.t. $\Fc_{k}$.

6. Since $-h_{\theta}$ has the same law as $h_{\theta}$, we have that
\begin{displaymath}
\nu_{1}\indic{\sigma_{1} = -1}
=
-\mathbb{E}[h_{\theta}\vert \Fc_{1}]\indic{\sigma_{1} = -1}
=\mathbb{E}[-h_{\theta}\vert \Fc_{1}]\indic{\sigma_{1} = -1}
\stackrel{\text{(d)}}{=}\mathbb{E}[h_{\theta}\vert \Fc_{1}]\indic{\sigma_{1} = 1}
=\nu_{1}\indic{\sigma_{1} = 1},
\end{displaymath}
which gives the independence between $\nu_{1}$ and $\sigma_{1}$.
For $k\geq 2$, we use the same reasoning, by relying on points 5. and 1.

7. From 3. and 2. follows that a.s. for every 
$f\in\Cc^{\infty}_{c}(\C\setminus\overline{\Cc}_{1})$,
$(\mathbb{E}[h_{\theta}\vert\Fc_{1}],f)=0$.
So this concludes in the case $k=1$.
Now take $k\geq 2$. By 5., for every 
$f\in\Cc^{\infty}_{c}(\C)$, 
\begin{displaymath}
\sigma_{k}(\nu_{k},f) = (h_{\theta, k-1}-h_{\theta, k},f).
\end{displaymath}
Then, similarly to 2., we get that
$(h_{\theta, k-1},f) = (h_{\theta, k},f)$
for every $f\in \Cc^{\infty}_{c}(\C\setminus\overline{\Cc}_{k})$.
\end{proof}

By convention, we set $D_{0}=D$.
Let $D_{k}^{\ast}$ be the open subset of $D_{k}$ obtained as the union of the
non-simply connected components of $D_{k}$, which are finitely many.

%\begin{lemma}
%\label{Lem int to 0 dim}
%A.s., as $\gamma\to 0$, the measure
%\begin{displaymath}
%\dfrac{1}{Z_{\gamma}}\indic{x\in D_{k}^{\ast}}
%(1-e^{\gamma^{2}\pi(G_{D_{k}}(x,x)-G_{D_{k-1}}(x,x))}) dx
%\end{displaymath}
%converges to $0$ for the weak topology of measures on
%$\overline{D_{k}^{\ast}}$.
%\end{lemma}


\begin{lemma}
\label{Lem remove multiply}
The measure
\begin{equation}
\label{Eq cond measure multiply}
\dfrac{1}{Z_{\gamma}}
(\indic{x\in D_{k}^{\ast}}dx-
\mathbb{E}[\mathbf{1}_{x\in D_{k}^{\ast}}e^{\gamma^{2}\pi (G_{D}(x,x) - G_{D_{k-1}}(x,x))}\Mc_{\gamma}^{+}(dx))\vert \Fc_{k}]) 
\end{equation}
is a.s. a positive finite measure that converges a.s. to $0$ for the weak topology of measures on
$\overline{D_{k}^{\ast}}$ as $\gamma \to 0$.
\end{lemma}

\begin{proof}
We start by proving that \eqref{Eq cond measure multiply} is a positive measure.
Let $\Lc^{\theta}_{D_{k}^{\ast}}$ be the collection of Brownian loops,
distributed conditionally on $D_{k}$,
as the Brownian loop soup in $D_{k}^{\ast}$ with intensity $\theta$
(that is without any topological conditioning).
Let $\Mc_{D_{k}^{\ast},\gamma}$ denote the multiplicative chaos
of $\Lc^{\theta}_{D_{k}^{\ast}}$, normalized by
$\mathbb{E}[\Mc_{D_{k}^{\ast},\gamma}\vert D_{k}]
= \indic{x\in D_{k}^{\ast}} 2 dx$.
Let $E_{k}$ be the event that no cluster of loops in $\Lc^{\theta}_{D_{k}^{\ast}}$
surrounds an inner hole of $D_{k}^{\ast}$,
which is an event with positive probability.
Then
\begin{displaymath}
\mathbb{E}[\mathbf{1}_{x\in D_{k}^{\ast}}
e^{\gamma^{2}\pi (G_{D}(x,x) - G_{D_{k-1}}(x,x))}\Mc_{\gamma}^{+}(dx))\vert \Fc_{k}]
=\dfrac{1}{2}
\mathbb{E}\Big[
e^{\gamma^{2}\pi(G_{D_{k}}(x,x)-G_{D_{k-1}}(x,x))}
\Mc_{D_{k}^{\ast},\gamma}(dx)
\Big\vert D_{k}^{\ast}, E_{k}\Big].
\end{displaymath}
Note that the Dirichlet Green's function on $D_{k}^{\ast}$
is the restriction of $G_{D_{k}}$ to
$D_{k}^{\ast}\times D_{k}^{\ast}$.
The event $E_{k}$ is a decreasing event.
Therefore, by FKG inequality for Poisson point processes, a.s.
\begin{multline*}
\mathbb{E}[\mathbf{1}_{x\in D_{k}^{\ast}}
e^{\gamma^{2}\pi (G_{D}(x,x) - G_{D_{k-1}}(x,x))}\Mc_{\gamma}^{+}(dx))\vert \Fc_{k}]
\\
\leq 
\dfrac{1}{2}
\mathbb{E}\Big[
e^{\gamma^{2}\pi(G_{D_{k}}(x,x)-G_{D_{k-1}}(x,x))}
\Mc_{D_{k}^{\ast},\gamma}(dx)
\Big\vert D_{k}^{\ast}\Big]
=
\indic{x\in D_{k}^{\ast}}
e^{\gamma^{2}\pi(G_{D_{k}}(x,x)-G_{D_{k-1}}(x,x))} dx .
\end{multline*}
Thus, for every $\gamma\in (0,2)$, 
\eqref{Eq cond measure multiply} is a positive finite measure.

The rest of the proof is then dedicated to showing that \eqref{Eq cond measure multiply} goes to zero as $\gamma \to 0$. Define $f(x) = e^{2\pi(G_{D_{k}}(x,x)-G_{D_{k-1}}(x,x))}$.
We can write the total mass of \eqref{Eq cond measure multiply} as
\begin{equation}
\label{Eq cond measure multiply1}
\dfrac{1}{Z_{\gamma}} \int_{D_{k}^{\ast}}
(1-e^{\gamma^{2}\pi(G_{D_{k}}(x,x)-G_{D_{k-1}}(x,x))}) dx
-
\dfrac{1}{2 Z_{\gamma} \mathbb{P}(E_{k})}
\mathbb{E}\Big[\Big((\Mc_{D_{k}^{\ast},\gamma},f^{\gamma^{2}/2})
-2\int_{D_{k}^{\ast}}f^{\gamma^{2}/2}\Big) \mathbf{1}_{E_k}
\Big\vert D_{k}^{\ast}\Big].
\end{equation}
We are going to show separately that each of these two terms vanishes as $\gamma \to 0$. By Cauchy--Schwarz and then by \eqref{E:second_moment_measure1}, the absolute value of the second term is at most
\begin{align*}
& \dfrac{1}{2 Z_{\gamma} \mathbb{P}(E_{k})^{1/2}}
\mathbb{E}\Big[\Big((\Mc_{D_{k}^{\ast},\gamma},f^{\gamma^{2}/2})
-2\int_{D_{k}^{\ast}}f^{\gamma^{2}/2}\Big)^{2}
\Big\vert D_{k}^{\ast}\Big]^{1/2} \\
& = \frac{2}{Z_\gamma \P(E_k)^{1/2}} \left( \int_{D_{k}^{\ast}\times D_{k}^{\ast}}
\big((\gamma^{2}\pi G_{D_{k}^{\ast}}(x,y))^{1-\theta}
\Gamma(\theta)I_{\theta -1}(2\gamma^{2}\pi G_{D_{k}^{\ast}}(x,y))
-1\big) f(x)^{\gamma^{2}/2} f(y)^{\gamma^{2}/2}\,dx\,dy \right)^{1/2} \\
& = O(\gamma^2 / Z_\gamma).
\end{align*}
The last estimate can be obtained by expanding $I_{\theta -1}$ (see \eqref{E:BesselI}).
Hence the second term of \eqref{Eq cond measure multiply1} vanishes as $\gamma \to 0$. 

%
%Since $f\leq 1$ and $u^{1-\theta}\Gamma(\theta)I_{\theta -1}(2u) - 1\geq 0$
%for $u>0$, we get
%\begin{displaymath}
%\mathbb{E}\Big[\Big((\Mc_{D_{k}^{\ast},\gamma},f^{\gamma^{2}/2})
%-2\int_{D_{k}^{\ast}}f^{\gamma^{2}/2}\Big)^{2}
%\Big\vert D_{k}^{\ast}\Big]
%\leq
%\mathbb{E}\Big[\Big((\Mc_{D_{k}^{\ast},\gamma},1)
%-2\int_{D_{k}^{\ast}} dx\Big)^{2}
%\Big\vert D_{k}^{\ast}\Big].
%\end{displaymath}
%
%Since we have Lemma \ref{Lem int to 0 dim},
%to conclude it is enough to show that a.s.,
%\begin{displaymath}
%\mathbb{E}\Big[\Big((\Mc_{D_{k}^{\ast},\gamma},1)
%-2\int_{D_{k}^{\ast}} dx\Big)^{2}
%\Big\vert D_{k}^{\ast}\Big]
%= o(Z_{\gamma}^{2}).
%\end{displaymath}
%But actually,
%\begin{displaymath}
%\mathbb{E}\Big[\Big((\Mc_{D_{k}^{\ast},\gamma},1)
%-2\int_{D_{k}^{\ast}} dx\Big)^{2}
%\Big\vert D_{k}^{\ast}\Big]
%\sim 
%4\pi^{2}\gamma^{4}
%\dfrac{1}{\theta}
%\int_{D_{k}^{\ast}\times D_{k}^{\ast}} G_{D_{k}}(x,y)^{2}\,dx\,dy,
%\end{displaymath}
%which concludes.
%\titus{Titus: Maybe explain why. Do not use Wick expansion, keep things elementary.
%The expansion of $I_{\theta -1}$ near $0$ is not enough because of the blow-up of the two-point correlation function near the diagonal.}

To conclude the proof, it remains to show that
\begin{equation}
\label{Eq int to 0 dim}
\dfrac{1}{Z_{\gamma}} \int_{D_{k}^{\ast}}
(1-e^{\gamma^{2}\pi(G_{D_{k}}(x,x)-G_{D_{k-1}}(x,x))}) dx
\to 0
\quad \quad \text{as} \quad \gamma \to 0.
\end{equation}
For fixed $x\in D_{k}^{\ast}$, the density
$
1-e^{\gamma^{2}\pi(G_{D_{k}}(x,x)-G_{D_{k-1}}(x,x))})
$
is of order $\gamma^{2}$.
Since $Z_{\gamma}\gg \gamma^{2}$, the density converges to $0$,
actually uniformly on compact subsets of $D_{k}^{\ast}$.
However, this is not enough for our purpose and we need to control what happens
near the boundary $\partial D_{k}^{\ast}$.

The boundary $\partial D_{k}^{\ast}$ has exactly $k+1$ connected components,
one of them being $\partial D$, and the $k$ others being the
outer boundaries of $\Cc_{1},\dots,\Cc_{k}$.
$\partial D$ and $\Cc_1, \dots, \Cc_{k-1}$ lie outside both $D_{k-1}$ and $D_k$. Thus $G_{D_{k-1}}(x,x)-G_{D_{k}}(x,x)$ stays bounded in a neighborhood of
$\partial D \cup \Cc_{1} \cup \dots \cup \Cc_{k-1}$. Therefore,
the uniform convergence of the density to $0$
is also true on compact neighborhoods of these $k$ boundary components of
$\partial D_{k}^{\ast}$.
On the other hand, $\Cc_k$ is contained in $D_{k-1}$ and lies outside of $D_k$. We will therefore have to treat this case separately.

Let us denote by $\partial_{o}\Cc_{k}$ the outer boundary of $\Cc_k$.
Near $\partial_{o}\Cc_{k}$, $G_{D_{k-1}}(x,x)- G_{D_{k}}(x,x)$ explodes to $+\infty$.
But there is a constant $c(D_{k-1})\in (0,1)$, depending on $D_{k-1}$, 
such that for every $x\in D_{k}^{\ast}$,
\begin{displaymath}
e^{2\pi(G_{D_{k}}(x,x)-G_{D_{k-1}}(x,x))}\geq 
c(D_{k-1})\dfrac{d(x,\partial D_{k}^{\ast})}{d(x,\partial D_{k-1})}.
\end{displaymath}
This is in a way a generalization of Koebe quarter theorem to domains with holes; see \cite[Lemma 5.13]{ALS1}.
Fix $\varepsilon_{0}\in 
(0, d(\partial_{o}\Cc_{k},\partial D_{k}^{\ast}\setminus\partial_{o}\Cc_{k}))$.
Then for every $x\in D_{k}^{\ast}$ such that
$d(x,\partial_{o}\Cc_{k})<1\wedge(\varepsilon_{0}/2)$, we have
\begin{multline*}
\dfrac{1}{Z_{\gamma}}(1-e^{\gamma^{2}\pi(G_{D_{k}}(x,x)-G_{D_{k-1}}(x,x))})
\leq 
\dfrac{1}{Z_{\gamma}}\Big(
1
-c(D_{k-1})^{\gamma^{2}/2}
\dfrac{d(x,\partial D_{k}^{\ast})^{\gamma^{2}/2}}{d(x,\partial D_{k-1})^{\gamma^{2}/2}}
\Big)
\\\leq
\dfrac{1}{Z_{\gamma}}\Big(
1
-
c(D_{k-1})^{\gamma^{2}/2}
\dfrac{d(x,\partial_{o}\Cc_{k})^{\gamma^{2}/2}}{\diam(D)^{\gamma^{2}/2}}
\Big)
=
\dfrac{1}{Z_{\gamma}}(
1
-
d(x,\partial_{o}\Cc_{k})^{\gamma^{2}/2}
)
+
\dfrac{1}{Z_{\gamma}}\Big(
1- \dfrac{c(D_{k-1})^{\gamma^{2}/2}}{\diam(D)^{\gamma^{2}/2}}
\Big)
d(x,\partial_{o}\Cc_{k})^{\gamma^{2}/2}
\end{multline*}
Since
\begin{displaymath}
\lim_{\gamma\to 0} \dfrac{1}{Z_{\gamma}}\Big(
1- \dfrac{c(D_{k-1})^{\gamma^{2}/2}}{\diam(D)^{\gamma^{2}/2}}
\Big) = 0,
\end{displaymath}
we only need to consider the term
$(1-d(x,\partial_{o}\Cc_{k})^{\gamma^{2}/2})/Z_{\gamma}$.
Further,
\begin{equation}
\label{Eq Mink bound 1}
\dfrac{1}{Z_{\gamma}}\int_{d(x,\partial_{o}\Cc_{k})<1}
(1-d(x,\partial_{o}\Cc_{k})^{\gamma^{2}/2})\,dx
=
\dfrac{\gamma^{2}}{2Z_{\gamma}}\int_{0}^{1} dr\,
r^{\gamma^{2}/2-1}
\int_{d(x,\partial_{o}\Cc_{k})<r}dx
\end{equation}
Since $\partial_{o}\Cc_{k}$ is an SLE$_{\kappa(\theta)}$ type curve,
it is of dimension $1+\kappa(\theta)/8\leq 3/2<2$ \cite{BeffaradimSLE}.
In particular, for $\beta\in (0,1/2)$, there is a.s. a (random) constant
$c(\beta)>0$ such that for every $r\in (0,1)$,
\begin{displaymath}
\int_{d(x,\partial_{o}\Cc_{k})<r}dx \leq c(\beta)r^{\beta}.
\end{displaymath}
Thus, \eqref{Eq Mink bound 1} is bounded by
\begin{displaymath}
c(\beta)\dfrac{\gamma^{2}}{2Z_{\gamma}}\int_{0}^{1}
r^{\gamma^{2}/2 + \beta -1}\, dr,
\end{displaymath}
which tends to $0$ as $\gamma$ to $0$. This concludes.
\end{proof}


%
%Next we identify the distributions $\nu_{k}$ as random non-negative finite measures that agree with the measures $\mu_k$ from Theorem \ref{T:measure_cluster}.
%
%\begin{theorem}
%\label{Thm Minkowski}
%Let $k\geq 1$. 
%Then for every $f\in\Cc^{\infty}_{c}(\C)$,
%\begin{equation}
%\label{Eq nu k limit}
%(\nu_{k},f) = \lim_{\gamma \to 0}
%\dfrac{1}{Z_{\gamma}}\int_{d(x,\Cc_{k})<1}
%f(x) (1-d(x,\Cc_{k})^{\gamma^{2}/2}) \,dx
%,
%\end{equation}
%where the limit is in probability.
%In particular, $\nu_{k}$ is a.s. a non-negative finite measure
%supported on $\overline{\Cc}_{k}$ that agrees with $\mu_k$.
%\end{theorem}


We now have all the ingredients to prove Theorem \ref{T:h_and_minkowski}.

\begin{proof}[Proof of Theorem \ref{T:h_and_minkowski}]
The only thing that remains to be proved is that the random generalised function 
$\nu_{k}$ agrees a.s. with the measure $\mu_k$ from Theorem \ref{T:measure_cluster}. Let $f\in\Cc^{\infty}_{c}(\C)$. It is enough to show that
\begin{equation}
\label{Eq nu k limit}
(\nu_{k},f) = \lim_{\gamma \to 0}
\dfrac{1}{Z_{\gamma}}\int_{d(x,\Cc_{k})<1}
f(x) (1-d(x,\Cc_{k})^{\gamma^{2}/2}) \,dx
,
\end{equation}
in probability.
We have that
\begin{displaymath}
(\nu_{k},f) = \sigma_{k}\mathbb{E}[(h_{\theta, k-1},f)\vert\Fc_{k}],
\end{displaymath}
where by convention, $h_{\theta, 0} = h_{\theta}$.
Since $\nu_{k}$ and $\sigma_{k}$ are independent conditionally on $\Fc_{k}$,
we get that
\begin{equation}
\label{Eq nu k f}
(\nu_{k},f) = -\mathbb{E}[(h_{\theta, k-1},f)\vert\Fc_{k},\{\sigma_{k} = -1\}]
\end{equation}
Since
\begin{displaymath}
(h_{\theta, k-1},f) = 
\lim_{\gamma\to 0}
\dfrac{1}{Z_{\gamma}}
\int_{D_{k-1}}
f(x)(
e^{\gamma^{2}\pi (G_{D}(x,x) - G_{D_{k-1}}(x,x))}
\Mc^{+}_{\gamma}(dx) 
- dx),
\end{displaymath}
where the convergence is a.s. in $L^2$ conditionally on
$\Fc_{k-1}$
(that is to say $\lim_{\gamma\to 0}\mathbb{E}[(\cdot)^{2}\vert \Fc_{k-1}] =0$ a.s.).
Therefore, in \eqref{Eq nu k f} one can interchange the conditional expectation and the limit in $\gamma$ and get
\begin{displaymath}
(\nu_{k},f) = 
\lim_{\gamma\to 0}
\dfrac{1}{Z_{\gamma}}
\Big(\int_{D_{k-1}} f(x)\,dx
-\mathbb{E}\Big[
\int_{D_{k-1}}
 f(x)e^{\gamma^{2}\pi (G_{D}(x,x) - G_{D_{k-1}}(x,x))}
\Mc^{+}_{\gamma}(dx) 
\Big\vert
\Fc_{k},\{\sigma_{k} = -1\}
\Big]
\Big),
\end{displaymath}
where the convergence is a.s. in $L^2$ conditionally on $\Fc_{k-1}$.
By Theorem \ref{T:large_crossing}, $\overline{\Cc}_{k}$ has a.s. zero Lebesgue measure (the expectation of the Lebesgue measure of its $r$-neighbourhood vanishes as $r \to 0$). So $\int_{D_{k-1}} f(x)\,dx = \int_{D_k} f(x)\,dx$ a.s.
Moreover,
since on the event $\{\sigma_{k} = -1\}$,
$\indic{D_{k-1}}\Mc^{+}_{\gamma} = \indic{D_{k}}\Mc^{+}_{\gamma}$,
and since $\sigma_{k}$ is independent from $\indic{D_{k}}\Mc^{+}_{\gamma}$
conditionally on $\Fc_{k} $,
we get that
\begin{displaymath}
(\nu_{k},f) = 
\lim_{\gamma\to 0}
\dfrac{1}{Z_{\gamma}}
\Big(\int_{D_{k}} f(x)\,dx
-\mathbb{E}\Big[
\int_{D_{k}}
 f(x)e^{\gamma^{2}\pi (G_{D}(x,x) - G_{D_{k-1}}(x,x))}
\Mc^{+}_{\gamma}(dx) 
\Big\vert
\Fc_{k}
\Big]
\Big).
\end{displaymath}

Now we partition $D_{k} = D_{k}^{0} \cup D_{k}^{\ast}$,
where $D_{k}^{0}$ is the union of the simply connected components of
$D_{k}$ (there are infinitely many of them) and $D_{k}^{\ast}$
is the union of the multiply connected components of
$D_{k}$ (there are finitely many of them).
Then Lemma \ref{Lem remove multiply} ensures that
\begin{displaymath}
(\nu_{k},f) = 
\lim_{\gamma\to 0}
\dfrac{1}{Z_{\gamma}}
\Big(\int_{D_{k}^{0}} f(x)\,dx
-\mathbb{E}\Big[
\int_{D_{k}^{0}}
 f(x)e^{\gamma^{2}\pi (G_{D}(x,x) - G_{D_{k-1}}(x,x))}
\Mc^{+}_{\gamma}(dx) 
\Big\vert
\Fc_{k}
\Big]
\Big).
\end{displaymath}
Since conditionally on $\Fc_{k}$,
the loops in $D_{k}^{0}$ form a Poisson point process without conditioning,
we get that
\begin{displaymath}
\mathbb{E}\Big[
\int_{D_{k}^{0}}
 f(x)e^{\gamma^{2}\pi (G_{D}(x,x) - G_{D_{k-1}}(x,x))}
\Mc^{+}_{\gamma}(dx) 
\Big\vert
\Fc_{k}
\Big]
=
\int_{D_{k}^{0}}
f(x)e^{\gamma^{2}\pi (G_{D_{k}}(x,x) - G_{D_{k-1}}(x,x))}\,dx.
\end{displaymath}
The function $G_{D_{k-1}}(x,x)-G_{D_{k}}(x,x)$ is bounded for $x$
away from $\Cc_{k}$ and explodes when $x$ approaches $\partial\Cc_{k}$.
Further, \cite[Lemma 5.13]{ALS1} provides a comparison with the Euclidean
distance:
there is a constant $c(D_{k-1})\in (0,1)$
depending on $D_{k-1}$
such that for every $x\in D_{k}^{0}$,
\begin{displaymath}
c(D_{k-1})\dfrac{d(x,\partial D_{k}^{0})}{d(x,\partial D_{k-1})}
\leq e^{2\pi (G_{D_{k}}(x,x) - G_{D_{k-1}}(x,x))}
\leq 4 \dfrac{d(x,\partial D_{k}^{0})}{d(x,\partial D_{k-1})}.
\end{displaymath}
Then using these bounds,
similarly to the proof of \eqref{Eq int to 0 dim},
we get that
\begin{displaymath}
(\nu_{k},f) = 
\lim_{\gamma\to 0}
\dfrac{1}{Z_{\gamma}}
\int_{\substack{x\in D_{k}^{0}\\d(x,\Cc_{k})<1}}f(x)(1-d(x,\Cc_{k})^{\gamma^{2}/2})\,dx .
\end{displaymath}
Since the dimension of the outer boundary of
$\Cc_{k}$ is strictly smaller than $2$,
we get that (see the proof of \eqref{Eq int to 0 dim})
\begin{displaymath}
(\nu_{k},f) = 
\lim_{\gamma\to 0}
\dfrac{1}{Z_{\gamma}}
\int_{\substack{d(x,\Cc_{k})<1}}f(x)(1-d(x,\Cc_{k})^{\gamma^{2}/2})\,dx ,
\end{displaymath}
which concludes.
\end{proof}


\begin{comment}
\begin{remark}\label{rmk:Minkowski}
\antoine{delete this}
One may want to improve Theorem \ref{Thm Minkowski} into several directions.
All these improvements are available in the GFF case $\theta = 1/2$;
see \cite{ALS1}.
\begin{itemize}
\item First of all, one would like to replace the convergence in probability in
\eqref{Eq nu k limit} by an a.s. convergence.
\item Then, \eqref{Eq nu k limit} is not exactly the expression of a
Minkowski content measure.
A Minkowski content measure would be a renormalized area measure on an
$\varepsilon$-neighborhood of $\Cc_{k}$.
However, the two are related.
Indeed, for $\varepsilon\in (0,1)$, let $\gamma(\varepsilon)$ be given by
\begin{displaymath}
1 - \varepsilon^{\gamma(\varepsilon)^{2}/2} = \dfrac{1}{2},
\qquad \text{i.e.}
~~\gamma(\varepsilon) = \sqrt{\dfrac{2\log 2}{\log \varepsilon^{-1}}}.
\end{displaymath}
Then for every $r>0$,
\begin{displaymath}
\indic{r<\varepsilon}\leq 2 \indic{r<1} (1 - r^{\gamma(\varepsilon)^{2}/2}).
\end{displaymath}
Thus, Theorem \ref{Thm Minkowski} provides the tightness of measures
approximating the Minkowski content in the gauge
$\varepsilon^{2} Z_{\gamma(\varepsilon)}^{-1}$.
To identify $\nu_{k}$ with the Minkowski content measure in this gauge, one can use
that
\begin{displaymath}
\dfrac{1}{Z_{\gamma_{0}}} \indic{r<1} (1-r^{\gamma_{0}^{2}/2})
=\int_{0}^{1}\dfrac{1}{Z_{\gamma(\varepsilon^{2/\gamma_{0}^{2}})}}
\indic{r<\varepsilon^{2/\gamma_{0}^{2}}} 
\dfrac{Z_{\gamma(\varepsilon^{2/\gamma_{0}^{2}})}}{Z_{\gamma_{0}}}
d\varepsilon ,
\end{displaymath}
with $\gamma(\varepsilon^{2/\gamma_{0}^{2}})= \gamma_{0} \gamma(\varepsilon)$.
To conclude, we need the convergence, as $\gamma\to 0$,
of the ratio $Z_{c\gamma}/Z_{\gamma}$ for $c>0$ a constant.
We do not have this convergence in the case $\theta<1/2$.
However, we believe that
\begin{displaymath}
\lim_{\gamma\to 0} \dfrac{Z_{c\gamma}}{Z_{\gamma}} = c^{2(1-\theta)}.
\end{displaymath}
\item Finally, we believe that actually
$Z_{\gamma}\sim \text{cste } \gamma^{2(1-\theta)}$.
This would give the convergence of $Z_{c\gamma}/Z_{\gamma}$ and
explicitly identify the Minkowski gauge to
$\vert \log\varepsilon\vert^{1-\theta}\varepsilon^{2}$.
This is known so far only in the case $\theta = 1/2$; see \cite{ALS1}.
\end{itemize}
\end{remark}
\end{comment}



\subsection{Properties of \texorpdfstring{$h_\theta$}{h theta}: Proof of Theorem \ref{T:prop}}\label{SS:properties_field}

\begin{proof}
Point \ref{I:covariance}: See Lemma \ref{L:second_moment_to_crossing_proba} and Proposition \ref{P:crossing}.

Point \ref{I:conformal_invariance}: The conformal invariance of the field follows directly from the conformal covariance of the approximation procedure used to define it, together with the fact that the conformal anomaly disappears when $\gamma \to 0$ (derivative of the conformal map to the power $\gamma^2/2$). See \cite[Theorem 1.1]{ABJL21}.

Point \ref{I:symmetry}:
By definition,
$
h_\theta + h_\theta^- = \lim_{\gamma \to 0} \frac{1}{Z_\gamma} ( \Mc_\gamma - \E[\Mc_\gamma] ).
$
Because the second term in the expansion of $\Mc_\gamma$ is $\gamma^2$ times the occupation measure of $\Lc_D^\theta$ (see Theorem \ref{T:expansion_unsigned}) and because $Z_\gamma \geq \gamma^{2(1-\theta)+o(1)}$, this limit equals zero.

Point \ref{I:nondegenerate}: Let $f : D \to \R$ be a smooth test function, not identically zero. By Theorem \ref{T:h_and_minkowski},
\[
(h_\theta,f) = \sum_{k \geq 1} \sigma_k (\mu_k, f) \quad \quad \text{a.s.}
\]
Moreover, for all $k \geq 1$, the measure $\nu_k$ is not identically zero a.s. (see Theorem \ref{T:measure_cluster}). So for all $k \geq 1$ such that the closure of the cluster $\Cc_k$ is contained in $\{f \neq 0\}$, $(\mu_k, f) \neq 0$ a.s. There are almost surely infinitely many such $k$ and we can conclude with Lemma \ref{L:sum_elementary} below.
\end{proof}

\begin{lemma}\label{L:sum_elementary}
Let $(a_n)_{n \geq 1}$ be a sequence of non zero real numbers and let $(\sigma_n)_{n \geq 1}$ be i.i.d. spins taking values in $\{\pm 1\}$ with equal probability 1/2. Assume that $\sum_n \sigma_n a_n$ converges almost surely. Then the distribution of $\sum_n \sigma_n a_n$ is non-atomic.
\end{lemma}

\begin{proof}
Let $x \in \R$. We are going to show that $\sum_n \sigma_n a_n \neq x$ a.s. which will conclude the proof. The conditional probability $\Prob{ \sum_n \sigma_n a_n = x \vert \sigma_1, \dots, \sigma_{k-1} }$ converges a.s. to $\indic{\sum_n \sigma_n a_n = x}$ as $k \to \infty$. But, by flipping the $k$-th spin and using the fact that $a_k \neq 0$, we see that
\begin{align*}
\P \Big( \sum_n \sigma_n a_n = x \big\vert \{\sigma_i\}_{i=1}^{k-1} \Big)
& \leq \P \Big( \sum_{n \neq k} \sigma_n a_n -\sigma_k a_k \neq x \big\vert \{\sigma_i\}_{i=1}^{k-1}  \Big)  = \P \Big( \sum_n \sigma_n a_n \neq x \big\vert \{\sigma_i\}_{i=1}^{k-1}  \Big).
\end{align*}
Rearranging, this shows that  $\Prob{ \sum_n \sigma_n a_n = x \vert \sigma_1, \dots, \sigma_{k-1} } \leq 1/2$ a.s. Therefore, $\indic{\sum_n \sigma_n a_n = x}$ is at most $1/2$ a.s., meaning that  $\sum_n \sigma_n a_n \neq x$ a.s.
\end{proof}

==> subfiles/questions.tex <==
\begin{itemize}
\item
Construction of $h_\theta$ when $\theta \in (1/2,1)$ by erasing small loops? Find a procedure that would still give a conformally invariant field!
\item
\red{Measurability of the recentred local times w.r.t. $h_\theta$? One idea: show that the uniform measure on the set of thick points of $h_\theta$ regularised at scale $\eps$ converges as $\eps \to 0$ to $\Mc_\gamma^+$.}
\item
Is it true that $\{ :h_\theta(x) L_x^n:, :L_x^n: \}_{n \geq 0}$ is dense in the space of $L^2$ random variables measurable w.r.t. $h_\theta$?
\item
\red{Star-triangle}
\item
Is there a natural way of fixing the multiplicative constant in front of $h_\theta$? Related question: what is the value of the constant $c_\mathrm{conj}$ appearing in \eqref{E:conj_crossing_probability}?
\item
What happens when $\theta \to 0$? Can I renormalise $h_\theta$ and get something? Might be white noise (local time with signs $\to$ Gaussian, CLT)
\item
Show that $\pm L_x^{1-\theta}$ converges to $h_\theta$. (scaling limit)
Thanks to Theorem \ref{T:one_cluster}, it is sufficient to compare $\pm L_x^{1-\theta}$ with $\Mc_a^N \mathbf{1}_{\mathfrak{C}^+}$ to establish this convergence.
\item
Same thing as above but directly in the continuum. First restrict to a subset of loops so that the local time is well defined without recentering. Then take local time of small circle (or something else). sign and power $1-\theta$.
\item
Can we compute the moments of $h_\theta$ and express them as crossing probabilities? \cite{ABJL21} does not treat moments higher than two, so it might be painful...
\item
Domain Markov property? What would be the analogue of harmonic functions? Other description of this field? Characterisation?
\item
Explicit formula for the covariance of the field. Also true in the discrete??
\[
\Expect{ \sigma_x L_x^{1-\theta} \sigma_y L_y^{1-\theta} } \overset{??}{=} (1-\theta) \frac{\Gamma(1-\theta)}{\Gamma(\theta)} G_{D_N}(x,y)^{2(1-\theta)}
\]
\item
What can we say about the probabilistic properties of $(h_\theta,f)$? Existence of a smooth density w.r.t. Lebesgue measure? Is there an analogue of Malliavin calculus for Poisson point processes?
\end{itemize}


